Sublinear Time Low-Rank Approximation of Toeplitz Matrices

We present a sublinear time algorithm for computing a near optimal low-rank approximation to any positive semidefinite (PSD) Toeplitz matrix $T\in \mathbb{R}^{d\times d}$, given noisy access to its entries. In particular, given entrywise query access to $T+E$ for an arbitrary noise matrix $E\in \mathbb{R}^{d\times d}$, integer rank $k\leq d$, and error parameter $\delta>0$, our algorithm runs in time $\text{poly}(k,\log(d/\delta))$ and outputs (in factored form) a Toeplitz matrix $\widetilde{T} \in \mathbb{R}^{d \times d}$ with rank $\text{poly}(k,\log(d/\delta))$ satisfying, for some fixed constant $C$, \begin{equation*} \|T-\widetilde{T}\|_F \leq C \cdot \max\{\|E\|_F,\|T-T_k\|_F\} + \delta \cdot \|T\|_F. \end{equation*} Here $\|\cdot \|_F$ is the Frobenius norm and $T_k$ is the best (not necessarily Toeplitz) rank-$k$ approximation to $T$ in the Frobenius norm, given by projecting $T$ onto its top $k$ eigenvectors. Our result has the following applications. When $E = 0$, we obtain the first sublinear time near-relative-error low-rank approximation algorithm for PSD Toeplitz matrices, resolving the main open problem of Kapralov et al. SODA `23, whose algorithm had sublinear query complexity but exponential runtime. Our algorithm can also be applied to approximate the unknown Toeplitz covariance matrix of a multivariate Gaussian distribution, given sample access to this distribution, resolving an open question of Eldar et al. SODA `20. Our algorithm applies sparse Fourier transform techniques to recover a low-rank Toeplitz matrix using its Fourier structure. Our key technical contribution is the first polynomial time algorithm for \emph{discrete time off-grid} sparse Fourier recovery, which may be of independent interest.

==> approx_algorithm.tex <==
% !TEX root = ./main.tex

\section{Low-rank approximation with sublinear query complexity.}\label{algorithm}
%Now that we have established the existence of a good low rank approximation $\wt{T}$ which itself is Toeplitz, we present an alg orithm that constructs such a low rank approximation by only reading $poly(k)<<d$ entries of $T$. Note that we can trivially recover $T$ exactly by reading all the entries of the first column, that is the trivial sample complexity for this problem is $d$ samples. \\
In this section, we present our main algorithm, Algorithm \ref{sublinearqueryalgo} and prove the corresponding Theorem \ref{sublinearqueryalgo}, which shows that the algorithm outputs a near optimal low-rank approximation to $T$, while reading only sublinearly many entries. 
We treat $\wt{T}$, the low-rank Toeplitz approximation to $T$ (guaranteed to exist from Theorem \ref{frobeniusexistence}), as the true matrix, which we noisily access by reading entries of $T$.

\subsection{Reduction to weighted linear regression.}

%\hltodo{Need to double check the sparsity is updated throughout this section for the $1+\epsilon$ approximation: $\wt{O}(\frac{k}{\epsilon}\log(\frac{1}{\delta}))$} 
The near optimal Toeplitz low-rank approximation $\wt T \in \R^{d \times d}$ guaranteed to exist by Theorem \ref{frobeniusexistence} is of the form $\wt T =F_{\wt{S}}\wt{D}F_{\wt{S}}^{*}$, where $ F_{\wt{S}}\in \mathbb{C}^{d\times r}$ and $\wt{D}\in \mathbb{R}^{r\times r}$ are Fourier and diagonal matrices, respectively, and $r=\wt{O}((k/\epsilon)\log(1/\delta))$. Algorithm \ref{sublinearqueryalgo} uses brute force search to find the frequencies in $\wt{S}$. In particular, it uses an approximate regression oracle to test the quality of any guess for the frequencies in $\wt{S}$, without reading many entries of $T$.  

Recall from Theorem \ref{frobeniusexistence} that these frequencies lie in $r_1 = \tilde O(k/\epsilon)$  clusters of $r_2$ equispaced frequencies centered around points in $N =\{1/2d,3/2d,\ldots, 1-1/2d\}$. Thus, our search space will be all subsets of $r_1$ elements of $N$, of which there at at most $N^{r_1}$. Formally, the frequencies of our Toeplitz low-rank approximation will lie in the following set:
\begin{definition}[Frequency Search Space]\label{def:search}
	Consider any positive integers $d, r_1,r_2$ with $r_1,r_2 < d$ and $\gamma \in (0,1)$, 
	Let $N = \{1/2d,3/2d,\ldots,1-1/2d\}$. For any set of frequencies $B$, let $S(B) = \bigcup_{b \in B} \bigcup_{1 \le j \le r_2} \{ b + \gamma j, b - \gamma j\}$. Let $\mathcal{N}_{d,r_1,r_2,\gamma} = \{S(B): B \in N^{r_1}\}$. 
\end{definition}


Since the first column of $\wt{T}$ defines the full matrix, the approximate regression oracle will simply attempt to fit the first column of $\wt{T}$ to be close to that of $T$. However, since different entries in the first column appear with different frequencies in the matrix, we require the following weighting function to translate error bounds in the first column into error bounds for approximating the entire matrix ${T}$ in the Frobenius norm. 
\begin{definition}\label{weightingdef}
	Let $w\in \mathbb{R}^{d}$ be defined as follows:
	\begin{equation*}
		w_{i} =  \begin{cases} 
			\sqrt{d} & i = 1 \\
			\sqrt{2(d-i+1)} & i > 1 
		\end{cases}
	\end{equation*}
	Let $W = \diag(w)\in \mathbb{R}^{d\times d}$.
\end{definition}
We have the following immediate claim, which expresses the Frobenius norm difference between two symmetric Toeplitz matrices as the weighted $\ell_2$ norm difference of their first columns. 
\begin{claim}\label{frobtoeuclid}
	Let $T,  \wt T\in \mathbb{R}^{d\times d}$ be symmetric Toeplitz matrices with first columns $T_{1}, \wt T_1 \in \mathbb{R}^{d}$  respectively. Then letting $W \in \R^{d \times d}$ be as in Definition \ref{weightingdef},  $\|T -  \wt T\|_F = \|WT_1 - W \wt T_1\|_2$. 
\end{claim}

Now, for a Toeplitz matrix $T = F_S D F_S^*$, the first column can be expressed as $T_1 = F_S a$ where $a \in \R^{r}$ contains the diagonal entries of $D$. Further, if $T$ is real, $a$ must place equal weight on the conjugate frequencies in $F_S$. Thus, we can in fact write $T_1 = F_S R_S a$ where $a \in \R^{r/2}$ and $R_S \in \R^{r \times r/2}$ collapses the $2|S|=r$ conjugate pair columns of $F_S$ into $|S|=\frac{r}{2}$ real-valued columns, each corresponding to a degree of freedom of $a$. More formally:
\begin{definition}\label{def:RS} 
	Let $S \subset [0,\frac{1}{2})$ with $|S|=\frac{r}{2}$. % with $|S| = \frac{r}{2}$. 
	Then, define the matrix $R_S \in \mathbb{R}^{r \times \frac{r}{2}}$ by setting the $j^{th}$ column $(R_S)_{:,j}$ equal to $0$ everywhere except at $j$ and $|S|+j$, corresponding to the $j^{th}$ \emph{pair} of conjugate frequencies, where it is equal to $1$. 
\end{definition}

%Note in the above definition that if $r$, the rank of a Toeplitz matrix, is odd, then there exists some frequency in its Vandermonde decomposition which is its own conjugate. According to the convention of \ref{def:symmetric_fourier_matrix}, the frequency set $S$ is then of size $\frac{r}{2} \rceil$, where the column vector of $F_S$ corresponding to the self-conjugate frequency is repeated. This motivates the dimensionality of $R_S$ in the case when $r$ is odd. 

%It is trivial to check from this definition that $F_SR_S$ is always real-valued, so we can equivalently interpret $F_S$ applied to any $r$-length symmetric vector $x$ (which takes equal values on conjugate frequencies, ie. $x_j=x_{\frac{r}{2}+j}$ for $j\in[\frac{r}{2}]$) as $F_SR_S$ applied to the $\frac{r}{2}$-length scaled subset of $x$, $\frac{1}{2}R_S^Tx$. Therefore, we will apply leverage score sampling to the real-valued matrix $F_SR_S$, and optimize only over the desired $\frac{r}{2}$ degrees of freedom.

From Claim \ref{frobtoeuclid} and the existence proof of Theorem \ref{frobeniusexistence} we have the following lemma, which shows that fitting $\wt T$ can be reduced to a  real-valued linear regression problem:
\begin{lemma}[Toeplitz Approximation via Weighted Regression]\label{lem:regressionReduction}
	For any PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$ with first column $T_1$, $\eps,\delta \in (0,1)$, and integer $k\leq d$, let $\mathcal{N}_{d,r_1,r_2,\gamma}$ be as in Def. \ref{def:search}, where $r_1,r_2,\gamma$ are as in Theorem \ref{frobeniusexistence}. Let $W \in \R^{d\times d}$ be as in Def. \ref{weightingdef}. Then if $\wt S$ and $\wt a \in \R^{|\tilde S|}$ satisfy for some $\alpha \ge 1$:
	\begin{align*}
		\norm{WF_{\wt S} R_{\wt S} \wt a - WT_1}_2 \le \alpha \cdot \min_{S \in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{WF_SR_S a - WT_1}_2,
	\end{align*}
	letting $\wt T \in \R^{d \times d}$ be the symmetric Toeplitz matrix $\wt T = F_{\wt S} \diag(\wt a) F_{\wt S}^*$,
	$$\norm{T-\wt T}_F \le (1+\epsilon)\alpha \cdot \norm{T-T_k}_F + \alpha \delta \norm{T}_F.$$
\end{lemma}
\begin{proof}
	Letting $\wt T_1$ be the first column of $\wt T$, we have $\wt T_1 = F_{\wt S} R_{\wt S} \wt a$ where $R_{\wt S}$ is defined as in Def. \ref{def:RS}.
	%
	Thus, by Claim \ref{frobtoeuclid},
	\begin{align*}
		\|T -  \wt T\|_F = \|WT_1 - W F_{\wt S}R_{\wt S } \wt a\|_2 &\le  \alpha \cdot \min_{S \in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{WT_1 - WF_SR_S a}_2\\
		&\le (1+\epsilon) \alpha \cdot \norm{T-T_k}_F + \alpha \delta \norm{T}_F,
	\end{align*}
	where the last inequality follows from Theorem \ref{frobeniusexistence}, which shows that there is some Toeplitz matrix $\wt T$ with frequency set in $\mathcal{N}_{d,r_1,r_2,\gamma}$ satisfying $\norm{T-\wt T}_F \le (1+\epsilon) \norm{T-T_k}_F + \delta \norm{T}_F$.
	%The theorem then follows by noting that for $\epsilon \le 1$, $(1+\epsilon)^2 \le 1+3 \epsilon$ and $(1+\epsilon) \delta \le 2 \delta$.
\end{proof}

\subsection{Leverage score preliminaries.}
Our goal  is now  to find $\wt S \in \mathcal{N}_{d,r_1,r_2,\gamma}$ and $\wt a \in \R^{|\wt S|}$ satisfying the approximate regression guarantee of Lemma \ref{lem:regressionReduction} for $\alpha \le 1+\epsilon$. We do this using leverage score sampling. It is well known that leverage score sampling can be used to approximately solve linear regression problems in a sample-efficient manner \cite{Sarlos:2006vn,Woodruff:2014tg}. In our setting, an additional challenge arises in that to find $\wt S,\wt a$ satisfying the bound of Lemma \ref{lem:regressionReduction} we must solve many regression problems -- corresponding to all possible subsets $\wt S \in \mathcal{N}_{d,r_1,r_2,\gamma}$ -- and output one with near minimal error. This is challenging, since standard results on leverage score sampling for sample-efficient regression 1) typically do not succeed with very high probability, making it difficult to union bound over all possible $\wt S$, and 2) typically do not output an estimate of the actual regression error, making it impossible to chose a near optimal $\wt S,\wt a$ as needed in Lemma \ref{lem:regressionReduction}. We show how to overcome these issues in Sections \ref{sec:const} and \ref{sec:eps}.

Recall the notion of matrix leverage scores as defined in Definition \ref{leveragescoresdefn}. Our algorithm will sample rows of $WF_SR_S$ and $WT_1$ via approximations to the leverage scores of $WF_SR_S$ to solve the regression problem of Lemma \ref{lem:regressionReduction}. For technical reasons, we will sample with a mixture of a leverage score distribution and the uniform distribution, defined below:
\begin{definition}[Leverage score sampling; Def. 2.7 of \cite{musco2021active}]\label{def:levsampling}
	For any number of samples $m$ and a set of leverage score bounds $\{\tilde \tau_j \}_{j \in [n]}$ with $T = \sum_{j=1}^d \wt{\tau}_j$, let $\mathcal{S} \in \mathbb{R}^{m \times d}$ be a sampling matrix with each row set independently to the $i^{th}$ standard basis vector multiplied by $(m \cdot p_i)^{-1/2}$, with probability 
	\begin{align*}
		p_i &= \frac{1}{2} \Bigg( \frac{\wt{\tau}_i}{T} + \frac{1}{d} \Bigg).
	\end{align*}
\end{definition}
We also have the following unbiasedness property of the sampling matrix $\mcS$.
\begin{claim}\label{claim:unbiased}
	Let $\mcS$ be defined as in \ref{def:levsampling}. Then
	\begin{align*} 
		\E[\norm{\mcS x}_2^2] &= \norm{x}_2^2.
	\end{align*}
\end{claim}
Critically, we would like to take \emph{a single set} of samples and use them to approximately minimize $\norm{WT_1 - WF_SR_S a}_2$ for all $S \in \mathcal{N}_{d,r_1,r_2,\gamma}$ in order to solve the optimization problem of Lemma \ref{lem:regressionReduction}. We are able to do this due to the existence of \emph{universal} leverage score bounds on Fourier matrices \cite{Avron:2019tt,eldar2020toeplitz}, which are independent of the frequency subset $S$. We adapt these bounds to our  weighted setting. 
%To apply \ref{thm:updatedleveragesampling} in the proof of our approximate regression oracle, we therefore need good upper bounds on the leverage scores of $WF_SR_S$. We obtain such bounds in this section, which are in fact independent of the frequencies $S$. This is formalized in the following lemma.
\begin{lemma}[Fourier Matrix Leverage Score Bound]\label{leveragescorebound}
	Let $W$ be the weight matrix defined in \ref{weightingdef}. Then there exist non-negative numbers $\{\wt{\tau}_{j}\}_{j=1}^d$ such that the following hold for all frequency sets $S\subset [0,\frac{1}{2}), |S| = \frac{r}{2}\leq d$: 
	\begin{enumerate}
		\item $\tau_j(WF_SM_S) \leq \tau_j(WF_S) \leq \wt{\tau}_{j}$ for all $j\in [d]$.
		\item $\sum_{j=1}^{d} \wt{\tau}_{j} \leq O(r\log r \cdot \log d)$.
	\end{enumerate}
	Here, $F_S\in \mathbb{C}^{d\times r}$ is the symmetric Fourier matrix with frequency set $S$ as defined in \ref{def:symmetric_fourier_matrix}, and $M_S$ is any real-valued matrix with $r$ rows, which may depend on $S$. (For example, this includes the case $M_S=R_S$ as defined in Definition \ref{def:RS}.) Finally, $\tau_j(\cdot)$ is as defined in Def. \ref{leveragescoresdefn}.
\end{lemma}
\ref{leveragescorebound} is similar to Corollary C.2 of \cite{eldar2020toeplitz}, but applies to \emph{weighted} Fourier matrices. In \ref{subsec:weighted_fourier_lev_bounds} we restate Corollary C.2 of \cite{eldar2020toeplitz} as \ref{corr:C2_eldar}, and use it to prove  \ref{leveragescorebound}.

In our analysis, we will use the well known fact  that sampling $\tilde O(r)$ rows of $A \in \mathbb C^{d \times r}$ according to their leverage scores yields a \emph{subspace} embedding of $A$, which preserves the norms of all vectors in $A$'s column span to small relative error. In particular:
\begin{lemma}[Subspace Embedding \cite{Woodruff:2014tg}]\label{lem:subspace}
	Given $A \in \R^{d \times r}$, failure probability $\eta \in (0,1)$, and a set of leverage score upper bounds $\{\tilde \tau_j \}_{j \in [n]}$ satisfying $\tilde \tau_j \ge \tau_j(A)$ for all $j \in [d]$, let $\mathcal{S} \in \mathbb{R}^{m \times d}$ be a random sampling matrix drawn according to \ref{def:levsampling}, using the distribution $\wt{\tau}_j$ and $m=O\big(\frac{T \log(1/\eta)}{\beta^2}\big)$ samples. Then, with probability $\ge 1-\eta$, for all $x \in \R^r$, 
	$$(1-\beta) \norm{ Ax}_2 \le \norm{\mathcal{S}  Ax}_2 \le (1+\beta) \norm{ Ax}_2.$$
\end{lemma}

\subsection{Constant factor approximation.}\label{sec:const}
We now use the leverage score bounds of Lemma \ref{leveragescorebound} and the subspace embedding guarantee of Lemma \ref{lem:subspace} to show how to solve the optimization problem of Lemma \ref{lem:regressionReduction} for constant $\alpha$. We later show how to refine this to an $\alpha = 1+\epsilon$ approximation, achieving our final bound.

\begin{theorem}[Constant Factor Toeplitz Fitting]\label{thm:const}
	Consider the setting of Lemma \ref{lem:regressionReduction}. Let
	$\mathcal{S} \in \mathbb{R}^{m \times d}$ be a random sampling matrix drawn according to \ref{def:levsampling}, using the distribution $\wt{\tau}_j$ defined in Def. \ref{leveragescorebound} with $m = \tilde O \left( \frac{k^2\log(1/\delta)}{\epsilon^2} \right )$. Let
	\begin{align*}
		\tilde S, \tilde a = \argmin_{S \in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{\mathcal{S}WF_SR_S a - \mathcal{S}WT_1}_2.
	\end{align*}
	Then with probability at least $98/100$, $\tilde S$ and $\tilde a$ satisfy Lemma \ref{lem:regressionReduction} with $\alpha = 41$. In other words,
	\begin{align*}
		\norm{WF_{\wt S} R_{\wt S} \wt a - WT_1}_2 \le 41 \cdot \min_{S \in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{WF_SR_S a - WT_1}_2.
	\end{align*}
	%and so for $\wt T = F_{\wt S} \diag(\wt a) F_{\wt S}^*$,
	%$$\norm{T-\wt T}_F \le 200(1+\epsilon) \cdot \norm{T-T_k}_F + 200 \delta \norm{T}_F.$$
\end{theorem}
\begin{proof}
	%\Cam{Hannah can you do this proof?}
	Define the optimal frequency set and coefficients by $$S', a' = \text{argmin}_{S \in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{WF_SR_S a - WT_1}_2.$$ For any $S\in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}$ we can write $$\|WF_SR_Sa - WF_{S'}R_{S'}a'\|_2$$ as $$\|W[F_SR_S,F_{S'}R_{S'}][a;-a']\|_2 = \|W[F_S,F_{S'}][R_S;R_{S'}][a;-a']\|_2.$$ Here, $[F_S,F_{S'}]$ is a Fourier matrix, and $[R_S;R_{S'}]$ fits the criteria of the matrix $M_{S,S'}$ in \ref{leveragescorebound}. Therefore, by \ref{leveragescorebound} the leverage scores  of $W[F_S,F_{S'}][R_S;R_{S'}]$ are upper bounded by $\tilde{\tau}_j$ and sum to $O(r\log(d)\log(r))$. Applying \ref{lem:subspace} with $A=W[F_S,F_{S'}][R_S;R_{S'}]$, $\beta=\frac{1}{2}$, $\eta = 1/(100|N|^{r_1})$, and the upper bounds $\tilde{\tau}_j$, we obtain a sampling matrix $\mcS\in \mathbb{R}^{m\times d}$ that takes $m=\wt{O}(\frac{k^2\log(1/\delta)}{\epsilon^2})$ samples. By combining the probabilistic guarantee of \ref{lem:subspace} with a union bound over all $S \in \mathcal{N}_{d,r_1,r_2,\gamma}$, we get that the following holds with probability at least $1-|N|^{r_1}\eta = \frac{99}{100}$ over the choice of $\mcS$:
	\begin{align*}
		\|\mcS W [F_SR_S,F_{S'}R_{S'}] x \|_2 &\geq \frac{1}{2} \| W [F_SR_S,F_{S'}R_{S'}] x \|_2 \: \: \:  \forall S \in \mathcal{N}_{d,r_1,r_2,\gamma}, \: x \in \R^{r}.
	\end{align*} 
	This implies for the particular case of $S=\tilde{S}$ and $a=\tilde{a}$ that the following holds with probability at least $\frac{99}{100}$:
	\begin{align*}
%		\|WF_{\tilde{S}}R_{\tilde{S}}\tilde{a} - WF_{S'}R_{S'}a'\|_2 &= \|W[F_{\tilde{S}}R_{\tilde{S}},F_{S'}R_{S'}][\tilde{a};-a']\|_2    \\
		&\leq 2\|\mcS W [F_{\tilde{S}}R_{\tilde{S}},F_{S'}R_{S'}] [\ta;-a'] \|_2 \\
		&= 2\|\mcS WF_{\tilde{S}}R_{\tilde{S}}\tilde{a} - \mcS WF_{S'}R_{S'}a' \|_2  \\
		&\leq 2 (\|\mcS WF_{\tilde{S}}R_{\tilde{S}}\tilde{a} - \mcS WT_1 \|_2 + \|\mcS WT_1 - \mcS WF_{S'}R_{S'}a' \|_2  ) \\
		&\leq 2 (\| \mcS WF_{S'}R_{S'}a' - \mcS WT_1  \|_2 + \| \mcS WF_{S'}R_{S'}a' - \mcS WT_1  \|_2  ) \\
		&= 4 \| \mcS WF_{S'}R_{S'}a' - \mcS WT_1  \|_2.
	\end{align*}
	The last inequality above followed by the definition of $\tilde{S}$ and $\tilde{a}$ as minimizing $\norm{WF_SR_S a - WT_1}_2$ over all $S \in \mathcal{N}_{d,r_1,r_2,\gamma}, \: a \in \R^{r}$.  
	
	Moreover, by \ref{claim:unbiased}, $\E[\norm{\mcS WF_{S'}R_{S'}a' - \mcS WT_1}_2^2] = \norm{WF_{S'}R_{S'}a' - WT_1}_2^2$. Then by applying Markov's inequality, $\norm{\mcS WF_{S'}R_{S'}a' - \mcS WT_1}_2^2 \leq 100\norm{WF_{S'}R_{S'}a' - WT_1}_2^2$ with probability at least $\frac{99}{100}$. 
	Finally, we return to the quantity of interest, $\norm{WF_{\tilde{S}}R_{\tilde{S}}\tilde{a} - WT_1}_2$. By applying a union bound once more, the following then holds with probability at least $\frac{98}{100}$ over the choice of $\mcS$:
	\begin{align*}
		\norm{WF_{\tilde{S}}R_{\tilde{S}}\tilde{a} - WT_1}_2 &\leq \norm{WF_{S'}R_{S'}a' - WT_1}_2 + \norm{WF_{\tilde{S}}R_{\tilde{S}}\tilde{a} - WF_{S'}R_{S'}a'}_2  \\
		& \leq \norm{WF_{S'}R_{S'}a' - WT_1}_2 + 4 \| \mcS WF_{S'}R_{S'}a' - \mcS WT_1  \|_2  \\
		%&\leq \norm{WF_{S'}R_{S'}a' - WT_1}_2 + 4 \| \mcS WF_{S'}R_{S'}a' - \mcS WT_1  \|_2 \\
		&\leq \norm{WF_{S'}R_{S'}a' - WT_1}_2 + 40 \norm{WF_{S'}R_{S'}a' - WT_1}_2  \\
		& \leq 41 \norm{WF_{S'}R_{S'}a' - WT_1}_2\\
		& = 41 \min_{S \in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{WF_SR_S a - WT_1}_2.
	\end{align*}
	This concludes the proof of the lemma.
\end{proof}

\iffalse % Do not remove - convenient reference to original constant factor proof 
\hltodoil{Old is below}
We can write $\|WFd - WF'd'\|_2$ as $\|W[F,F'][d;-d']\|_2$. Here $[F;F']\in \mathbb{C}^{d\times 2r}$ is also a Fourier matrix. We apply Lemma \ref{lem:subspace} with $\epsilon=9$, $\delta_{1} = 1/(100|N|^{r_1})$, and $\wt{\tau}_j$ values for $d\times 2r$ dimensional weighted Fourier matrices as per Lemma \ref{leveragescorebound} to obtain a sampling matrix $P\in \mathbb{R}^{s\times d}$ that takes $s=O(\log(d|N|^{r_1}) 2r \log (d)\log (r)) = \wt{O}(k^2\log(1/\delta))$ samples. Taking a union bound over all $B\in N^{r_1}$ we get the following which holds with probability at least $1-|N|^{r_1}\delta_1 = 99/100$ over the choice of $P$.
\begin{align*}
	\|PW[F_{S(B)};F']x\|_2 \leq 10 \|W[F_{S(B)};F']x\|_2 \quad \forall B\in N^{r_1}, x\in \mathbb{C}^{2r}
\end{align*}
This in particular implies that  the following holds with probability at least $99/100$.
\begin{align*}
	\|WFd - WF'd'\|_2 &\leq 10 \|PWFd - PWF'd'\|_2\\
	&\leq 10 (\|PWFd - PWT_1\|_2 + \|PWF'd' - PWT_1\|_2)\\
	&\leq 10 (\|PWF'd' - PWT_1\|_2 + \|PWF'd' - PWT_1\|_2)\\
	&= 20\|PWF'd'-PWT_1\|_2
\end{align*}
Where the third inequality follows by observing that $F,d = \underset{B\in N^{r_1},x\in \mathbb{R}^{r}}{\argmin} \|PWF_{S(B)}x-PWT_1\|_2$. Now by the unbiasedness property of the sampling matrix $P$ as per Lemma \ref{leveragescoresampling} we get that $\mathbb{E}[\|PWF'd'-PWT_1\|_2^2] = \|WF'd'-WT_1\|_2^2$. Thus applying Markov's inequality we get that $\|PWF'd'-PWT_1\|_2\leq 10 \|WF'd'-WT_1\|_2$ with probability $99/100$. Thus taking a union bound we get that the following holds with probabililty at least $98/100$ over the choice of $P$.
\begin{align*}
	\|WFd - WT_1\|_2 &\leq \|WF'd'-WT_1\|_2 + \|WFd - WF'd'\|_2	\\		
	&\leq \|WF'd'-WT_1\|_2 +  20\|PWF'd'-PWT_1\|_2\\
	& \leq \|WF'd'-WT_1\|_2 +  200\|WF'd'-WT_1\|_2 \\
	& \leq 201\|WF'd'-WT_1\|_2\\
	& \leq \wt{O}(1)\|T-T_k\|_F + \delta \|T\|_F
\end{align*}
Thus we can finally conclude the following which completes the proof of point 2 of the theorem.
\begin{equation*}
	\|F\diag(d)F^{*}-T\|_F = \|WFd - WT_1\|_2 \leq \wt{O}(1)\|T-T_k\|_F + \delta \|T\|_F
\end{equation*}
Note that while computing $d_{S(B)} = \argmin_{x}\|PWF_{S(B)} - PWT_1\|_2$ for any $B\in N^{r_1}$ we can restrict $x$ to have the same value for any frequency and its negative counterpart. This would ensure that $ F_{S(B)}\diag(d_{S(B)})F_{S(B)}^{*}$ is a real symmetric Toeplitz matrix for any $B\in N^{r_1}$. The proof above goes through even with this modification. Finally, we only need to know $PWT_1$ while executing our algorithm. This requires reading just $s=\wt{O}(k^2\log(1/\delta))$ entries of $T_1$, as specified by the $s\times d$ sampling matrix $P$.
\fi 



\subsection{$(1+\epsilon)$-approximation.}\label{sec:eps}

Theorem \ref{thm:const} combined with Lemma \ref{lem:regressionReduction} yields a $\tilde O \left (\frac{k^2\log(1/\delta)}{\epsilon^2}\right )$ query algorithm for outputting $\tilde T$ with rank $\tilde O(k \log(1/\delta)/\epsilon)$ and $\norm{T-\tilde T}_F = O(1)  \norm{T-T_k}_F + \delta \norm{T}_F$. To prove Theorem \ref{sublinearqueryalgo} we need to improve this constant factor approximation to $(1+\epsilon)$.
We do this using recently developed guarantees for high probability relative error active regression via leverage score sampling \cite{musco2021active}. Importantly, we first compute a constant error solution via Theorem \ref{thm:const}. We then show that we can fit the \emph{residual} of this approximation to high accuracy via leverage score sampling. % \Cam{If I have time I really need to explain these ideas more/where they have been used before, etc.} 
Formally,
\begin{theorem}\label{thm:relative}
	Consider the setting of Lemma \ref{lem:regressionReduction} and let $\tilde S \in \mathcal{N}_{d,r_1,r_2,\gamma}$ and $\tilde a \in \R^{|\tilde S|}$ satisfy the lemma with $\alpha = O(1)$. Let $T_R = T_1 - F_{\tilde S} R_{\tilde S} \tilde a$ be their residual  in fitting the first column of $T$.
	
	Let
	$\mathcal{S} \in \mathbb{R}^{m \times d}$ be a random sampling matrix drawn according to \ref{def:levsampling}, using the distribution $\wt{\tau}_j$ defined in Def. \ref{leveragescorebound} with $m =  \tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{6}} \Big)$. Let
	\begin{align*}
		S', a' = \argmin_{S \in \mathcal{N}_{d,2r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{\mathcal{S}WF_SR_S a - \mathcal{S}WT_R}_2.
	\end{align*}
	Then with probability at least $99/100$, letting $\bar S = \tilde S \cup S'$ and $\bar a = [\tilde a, a']$, we have that $\bar S,\bar a$ satisfy Lemma \ref{lem:regressionReduction} with $\alpha = (1+\epsilon)$. I.e.,
	\begin{align*}
		\norm{WF_{\bar S} R_{\bar S} \bar a - WT_1}_2 \le (1+\epsilon) \cdot \min_{S \in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{WF_SR_S a - WT_1}_2,
	\end{align*}
	and thus, letting $\bar T= F_{\bar S} \diag(\bar a) F_{\bar S}^*$,
	\begin{align*}
		\norm{T-\bar T}_F \le (1+3\epsilon) \norm{T-T_k}_F + 2 \delta \norm{T}_F.
	\end{align*}
\end{theorem}
Note that $\bar  S$ output by Theorem \ref{thm:relative} does not lie in $\mathcal{N}_{d,r_1,r_2,\gamma}$. Since $S' \in \mathcal{N}_{d,2r_1,r_2,\gamma}$ and $\tilde S \in \mathcal{N}_{d,r_1,r_2,\gamma}$, we have $\bar S \in \mathcal{N}_{d,3r_1,r_2,\gamma}$. Lemma \ref{lem:regressionReduction} allows this -- it simply means that the rank of the corresponding Toeplitz matrix $\bar T$ may be three times as large as if $\bar S$ were in $\mathcal{N}_{d,r_1,r_2,\gamma}$.  
\begin{proof}
	Let $OPT = \min_{S \in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{WF_SR_S a - WT_1}_2$. Observe that 
	\begin{align*}
		\norm{WF_{\bar S} R_{\bar S} \bar a - WT_1}_2 = \norm{WF_{S'} R_{S'} a' + WF_{\tilde  S} R_{\tilde S} \tilde  a- WT_1}_2 = \norm{WF_{S'} R_{S'} a' - WT_R}_2.
	\end{align*}
	Thus, to prove the theorem, it suffices to show that
	\begin{align}\label{eq:sufficesBound1}
		\norm{WF_{S'} R_{S'} a' - WT_R}_2 \le (1+\epsilon) \cdot OPT.
	\end{align}
	Further note that by the assumption that $\tilde S,\tilde a$ satisfy Lemma \ref{lem:regressionReduction} with $\alpha = O(1)$ we have:
	\begin{align*}%\label{eq:residualBound}
		\norm{WT_R}_2 \le \alpha \cdot OPT = O(OPT).
	\end{align*}
	By Markov's inequality, since by construction $\E[\norm{\mathcal S WT_R}_2^2] = \norm{W T_R}_2^2$, with probability at least $999/1000$, this also gives that $\norm{\mathcal{S}WT_R}_2 \le \sqrt{1000} \cdot \alpha \cdot OPT =  O(OPT)$. 
	
	For a given $S \in \mathcal{N}_{d,2r_1,r_2,\gamma}$ define:
	\begin{align*}
		&a_S = \argmin_{a \in \R^{|S|}} \norm{W F_S R_S a - W T_R}_2 \\ &\text{ and }\\
		&a'_S = \argmin_{a \in \R^{|S|}} \norm{\mathcal{S} W F_S R_S a - \mathcal{S}W T_R}_2.
	\end{align*}
	Using that $\norm{W T_R}_2 = O(OPT)$ and applying triangle inequality, we have
	\begin{align}\label{eq:solutionNormBound1}
		\norm{WF_SR_Sa_S - WT_R}_2 &\le \norm{WT_R}_2\nonumber\\
		\norm{WF_SR_Sa_S}_2 - \norm{WT_R}_2 &\le \norm{WT_R}_2\nonumber\\
		\norm{WF_SR_Sa_S}_2 &= O(OPT).
	\end{align}
	Similarly, using that $\norm{SWT_R}_2 = O(OPT)$ with good probability, for all $S$ we have $\norm{\mathcal S WF_SR_Sa'_S}_2 = O(OPT)$. Further, as in Theorem \ref{thm:const}, with probability at least $1-|N|^{2r_1}\eta = 99/100$ for $\eta=1/(100|N|^{2r_1})$, the subspace embedding guarantee of Lemma \ref{lem:subspace} holds for all $WF_S R_S$ simultaneously for $\beta = O(1)$, giving  that for all $S \in \mathcal{N}_{d,2r_1,r_2,\gamma}$
	\begin{align}\label{eq:solutionNormBound2}
		\norm{WF_SR_Sa'_S}_2 = O(OPT).
	\end{align}
	
	Given \eqref{eq:solutionNormBound1} and \eqref{eq:solutionNormBound2}, to prove the theorem it suffices to show the following claim:
	\begin{claim}\label{clm:mainClaim}
		With probability at least $99/100$, for any $S \in \mathcal{N}_{d,2r_1,r_2,\gamma}$ and any $a \in \R^{|S|}$ with $\norm{WF_SR_Sa}_2 = O(OPT)$,
		\begin{align*}%\label{eq:mainClaim}
			\left | \norm{WF_SR_Sa - W T_R}_2^2 - \norm{\mathcal S WF_SR_Sa - \mathcal S W T_R}_2^2 - C \right | \le \epsilon \cdot OPT^2,
		\end{align*}
		where $C$ is a fixed constant that may depend on $\mathcal S$ and $WT_R$, but does not depend on $S$ or $a$.
	\end{claim}
	I.e., for any frequency set $S$ and coefficient vector $a \in \R^{|S|}$ where $\norm{WF_SR_Sa}_2 = O(OPT),$ the sampled regression cost, after shifting by a fixed constant, approximates the true regression cost up to additive error $\epsilon \cdot OPT^2$. This ensures that:
	\begin{align*}
		\norm{WF_{S'} R_{S'} a' - WT_R}_2^2 &= \norm{WF_{S'} R_{S'} a'_{S'} - WT_R}_2^2\\
		&\le \norm{\mathcal S WF_{S'}R_{S'}a'_{S'} - \mathcal S W T_R}_2^2 + C + \epsilon \cdot OPT^2\\
		&\le \norm{\mathcal S WF_{S^*}R_{S^*}a^* - \mathcal S W T_R}_2^2 + C + \epsilon \cdot OPT^2,
	\end{align*}
	where $S^*,a^* = \argmin_{S \in \mathcal{N}_{d,2r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{WF_{S}R_{S}a -  W T_R}_2$. The first inequality follows from Claim \ref{clm:mainClaim}, which can be applied since $\norm{WF_{S'}R_{S'}a'_{S'}}_2 = O(OPT)$ by \eqref{eq:solutionNormBound2}. The second inequality follows since $S', a'_{S'} = \argmin_{S \in \mathcal{N}_{d,2r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{\mathcal{S}WF_SR_S a - \mathcal{S}WT_R}_2$. Applying Claim \ref{clm:mainClaim} again to $S^*,a^*$, which is valid by \eqref{eq:solutionNormBound1}, we continue to bound:
	\begin{align}\label{eq:camInter}
		\norm{WF_{S'} R_{S'} a' - WT_R}_2^2 &\le \norm{\mathcal S WF_{S^*}R_{S^*}a^* - \mathcal S W T_R}_2^2 + C + \epsilon \cdot OPT^2\nonumber\\
		&\le \norm{WF_{S^*}R_{S^*}a^* - W T_R}_2^2 + 2 \epsilon \cdot OPT^2.
	\end{align}
	Finally, note that since we allow $S^* \in \mathcal{N}_{d,2r_1,r_2,\gamma},$ we have:
	\begin{align*}
		\norm{WF_{S^*}R_{S^*}a^* - W T_R}_2^2 &\le \min_{S \in  \mathcal{N}_{d,r_1,r_2,\gamma},a \in \R^{|S|}} \norm{WF_SR_S a + WF_{\tilde S} R_{\tilde S} \tilde a- W T_R}_2^2\\
		&= \min_{S \in  \mathcal{N}_{d,r_1,r_2,\gamma},a \in \R^{|S|}} \norm{WF_SR_S a - W T_1}_2^2 = OPT^2.
	\end{align*}
	Combined with \eqref{eq:camInter}, this gives that $\norm{WF_{S'} R_{S'} a' - WT_R}_2^2 \le (1 + 2\epsilon) \cdot OPT^2$, which, after taking a square root and adjusting $\epsilon$ by a constant yields \eqref{eq:sufficesBound1} and in turn the theorem.
	%
	%and $\norm{\mathcal S W T_R}_2 = O(OPT)$, we must have $\norm{W F_S R_S a
		%\begin{align}
		%\left | \norm{\mathcal{S} W F_S R_S a(S) - \mathcal{S}W T_R}_2
		%\end{align}
	\end{proof}
	We finally present the proof of Claim \ref{clm:mainClaim} below.
	\begin{proof}
		Claim \ref{clm:mainClaim} can be proven following the same approach as Theorem 3.4 of \cite{musco2021active}. For simplicity of notation, let $z := WT_R$. We define a set of `bad indices' where the relative size of $z_j$ is significantly larger than the leverage score $\tilde \tau_j$. The regression error on these bad indices will not be well approximated via leverage score sampling. However, this is ok, since no $W F_S R_S a$ can do a good job fitting these indices, given the leverage score bounds on $WF_S R_S$. Formally, let
		\begin{align*}
			\mathcal{B} = \left \{j \in [d] : \frac{z_j^2}{OPT^2} \ge \frac{\tilde \tau_j}{\epsilon^2} \right \}.
		\end{align*}
		Further, we let $\bar z \in \R^d$ be equal to $z$, except with  $\bar z_j = 0$ for all $j \in \mathcal{B}$. Importantly $\mathcal{B}$ and $\bar z$ are defined independently of any specific $S$. For any $S, a \in \R^{|S|}$ with $\norm{WF_SR_Sa}_2 = O(OPT)$ and any $j \in \mathcal{B}$, we have by the definition of the leverage score (Def. \ref{leveragescoresdefn}),
		\begin{align*}
			\left | (WF_SR_S a)_j \right |^2 &\le \norm{WF_SR_SA}_2^2 \cdot {\tilde \tau_j}\\
			&\le O(OPT^2) \cdot \frac{\epsilon^2 \cdot |z_j|^2}{OPT^2}\\
			&= O(\epsilon^2 \cdot |z_j|^2).
		\end{align*}
		This gives that 
		\begin{align*}
			\left | (WF_SR_S a)_j - z_j \right |^2 - \left | (WF_SR_S a)_j - \bar z_j \right |^2 &= \left | (WF_SR_S a)_j - z_j \right |^2 - \left | (WF_SR_S a)_j \right |^2 = (1 \pm O(\epsilon)) \cdot z_j^2.
		\end{align*}
		Thus, for $C_1 = \sum_{j \in \mathcal{B}} |z_j|^2 = \norm{z-\bar z}_2^2$, 
		\begin{align}\label{eq:zBar1Bound}
			\left | \norm{WF_SR_S a - z}_2^2 - \norm{WF_SR_S a - \bar z}_2^2 - C_1 \right | = O(\epsilon) \cdot OPT^2,
		\end{align}
		where we use that $\norm{z}_2^2 = O(OPT^2)$.
		Using the same proof, and the fact that with probability at least $999/1000$ by Markov's inequality, $\norm{\mathcal{S}z}_2^2 = O(OPT^2)$, we have for $C_2 = \norm{\mathcal S (z-\bar z)}_2^2$,
		\begin{align}\label{eq:zBar2Bound}
			\left | \norm{\mathcal S WF_SR_S a - \mathcal S z}_2^2 - \norm{\mathcal S WF_SR_S a - \mathcal S \bar z}_2^2 - C_2 \right | = O(\epsilon) \cdot OPT^2.
		\end{align}
		Observe that $C_1$ and $C_2$ only depend on the sampling matrix $\mathcal{S}$ and truncated vector $\bar z$, whose definition is independent of any specific frequency set $S$ or coefficient vector $a$. Thus, 
		with \eqref{eq:zBar1Bound} and \eqref{eq:zBar2Bound} in place, to prove Claim \ref{clm:mainClaim} it suffices to show that, for all $S \in  \mathcal{N}_{d,r_1,r_2,\gamma}$ and  $a \in \R^{|S|}$ with $\norm{WF_SR_Sa}_2 = O(OPT)$,
		\begin{align}\label{eq:bernsteinError}
			\left | \norm{WF_SR_Sa - \bar z}_2^2 - \norm{\mathcal S WF_SR_Sa - \mathcal S \bar z}_2^2  \right | = O(\epsilon)  \cdot OPT^2.
		\end{align}
		Observe that by definition of $\mathcal{B}$, the entries of $\bar z$ are bounded by $\bar z_j^2 \le OPT^2 \cdot \frac{\tilde \tau_j}{\epsilon^2}$. Similarly, since by assumption $\norm{WF_SR_Sa}_2^2 = O(OPT^2)$ and by the definition  of the leverage scores (Def. \ref{leveragescoresdefn}) $(WF_SR_Sa)_j^2 \le OPT^2 \cdot \tilde \tau_j$. Thus, sampling entries with probabilities proportional to their leverage scores as in Def. \ref{def:levsampling} ensures that for any fixed $S$ and $a \in \R^{|s|}$, by a standard Bernstein bound, \eqref{eq:bernsteinError} holds with high probability. This bound can then be extended to hold to all $S$ and $a$ via an $\epsilon$-net analysis as follows.
		\begin{comment}
		\begin{corollary}[Lemma 3.7 and Lemma 4.2 of \cite{musco2021active}]
			For any fixed $S$, for $m=\wt{O}(r_1r_2 \log(1/\eta)/\epsilon^9)$, equation \eqref{eq:bernsteinError} holds with probability $1-\eta$ for all $a\in \mathbb{R}^{|S|}$ with $\|WF_SR_S a\|_2 = O(OPT)$.
		\end{corollary}
	\end{comment}
	Fix an $S$. For simplicity we assume by scaling that $\|z\|_2=1$ and $OPT =\Theta(1)$. By Claim 3.8 in the version 1 of \cite{musco2021active}, to prove \eqref{eq:bernsteinError} it suffices to show that the following holds with high probability, for all $y\in \mathcal{N}_{\epsilon}$,
	\begin{equation*}
		|\|\mathcal S y - \mathcal S \bar z\|_2^2 - \|y - \bar z\|_2^2 | \leq \epsilon
	\end{equation*}
where $\mathcal{N}_{\epsilon} $ is an $\epsilon$-net of the set $\{WF_SR_S a: \|WF_SR_S a\|_2\leq 1\}$. By a standard volume argument, it is known that one can construct such a net with $\log |\mathcal{N}_{\epsilon}| = \wt{O}(r_1r_2 \log (1/\epsilon))$. We will show equation \eqref{eq:bernsteinError} for a fixed $S$ and all $a\in \mathbb{R}^{|S|}$ using Bernstein's inequality and a union bound. We have that $\mathbb{E}[\|\mathcal S y - \mathcal S \bar z\|_2^2] = \|y-\bar z\|_2^2 = O(1)$. Additionally by definition $|\bar z_i|^2 \leq  \frac{\wt \tau_i}{\epsilon^2}$ for all $i$. Similarly by the definition of leverage scores $|y_i|^2 \leq \wt \tau_j$. This implies the following,
\begin{equation*}
	|y_i-\bar z_i|^2 = O\left(\frac{\wt \tau_i}{\eps^2}\right)
\end{equation*} 
for all $i$.
By the construction of $\mathcal S$, we have the following,
\begin{equation*}
	|[\mathcal Sy - \mathcal S \bar z]_i|^2 \leq \frac{\sum_i \wt \tau_i}{m \wt \tau_i}\cdot \frac{\wt \tau_i}{\epsilon^2} \leq \wt{O} \left(\frac{r_1r_2}{m\epsilon^2}\right)
\end{equation*}
for all $i$. Thus, by applying a Bernstein bound, we get the following,
\begin{align*}
	Pr[|\|\mathcal S y - \mathcal S \bar z\|_2^2 - \|y - \bar z\|_2^2| > \epsilon] &\leq 2 \exp \left( -\wt \Omega\left(\frac{\epsilon^4 m}{r_1r_2}\right)\right)\\
	& \leq \eta/|\mathcal{N}_{\epsilon}|
\end{align*}
for $m = \wt O (r_1r_2 \log (|\mathcal{N}_{\epsilon}|/\eta)/\epsilon^4)$. Taking a union bound over all $y$ and by Claim 3.8 of \cite{musco2021active}, we get that equation \eqref{eq:bernsteinError} holds for a fixed $S$ and all $a\in \mathbb{R}^{|S|}$ with probability at least $1-\eta$.
		%By the analysis of that lemma, for any fixed $S$,  for $m = \tilde O \left (\frac{r_1 r_2 \log(1/\eta)}{\epsilon^9} \right )$, \eqref{eq:bernsteinError} holds with probability $1-\eta$ for all $a \in \R^{|S|}$ with $\norm{WF_SR_Sa}_2 = O(OPT)$. 
Setting $\eta = \frac{1}{100 \cdot |\mathcal{N}_{d,2r_1,r_2,\gamma}|} = \frac{1}{100 \cdot |N|^{2r_1}}$ in the previous corollary, we have that for 
\begin{align*}
	m &= \tilde O \left (\frac{r_1 r_2}{\epsilon^4}\log(|\mathcal{N}_{\epsilon}| \cdot 100|N|^{2r_1})\right )  \\
	& = \tilde O \left (\frac{r_1 r_2}{\epsilon^4}\left (\log(|\mathcal{N}_{\epsilon}|)+ \log( |N|^{2r_1})\right )\right ) \\
	& = \tilde O \left (\frac{r_1 r_2}{\epsilon^4}\left (r_1r_2 + r_1\right )\right )\\
	&= \tilde O \left (\frac{k^2 \log(1/\delta)}{\epsilon^{6}} \right ),
\end{align*}
equation \eqref{eq:bernsteinError} holds for all $S \in \mathcal{N}_{d,2r_1,r_2,\gamma}$ simultaneously with probability at least $99/100$. This completes the proof of the claim.
	\end{proof}
	
	%We will use  \ref{thm:updatedleveragesampling}, which formalizes this.  \ref{thm:updatedleveragesampling} gives worse $\epsilon$ and log dependencies than standard results on approximate regression with leverage score sampling . However, it provides two key guarantees that such theorems do not: 1) it gives a logarithmic dependence on the failure probability, which will be key in our setting, since we need to take a union bound over $N^{r_1}$ regression problems, and 2) it gives an estimate to the error of the approximate regression solution, which will be critical in choosing the set $\wt S$ that gives $\wt T$ best fitting $T$.
	%\iffalse
	%one can obtain spectral approximations to matrices by sampling their rows using probabilities proportional to their leverage scores. The following lemma formalizes this for complex matrices. 
	%\begin{lemma}[Corollary 5.2 in \cite{tropp2012user}]\label{leveragescoresampling}
	%	\hltodo{Do we still need this lemma? Check back}
	%	\mmtodoil{corollary 5.2 is matrix Chernoff, this lemma is considerably different to warrant some explanations how we get it from there.\\
		%	Is the first claim really true? I would personally expect that it holds with high probabilty for each $x$, not for all of them. }
	%	Given a matrix $A\in \mathbb{C}^{d\times r}$ and values $\wt{\tau}_{1},\ldots,\wt{\tau}_{d}\in [0,1]$ that satisfy the following for all $j\in [n]$.
	%	\begin{equation*}
		%		\wt{\tau}_{j}\geq \tau_{j}(A) 
		%	\end{equation*}
	%	Then there are universal constants $c,C$ such that if we perform the following:
	%	\begin{enumerate}
		%		\item Set $p_{j}= \min (1,c\wt{\tau}_{j}\log(r/\delta_{1})/\epsilon^2)$.
		%		\item Create a sampling matrix $P\in \mathbb{C}^{s\times d}$ that takes $s$ samples as follows - Sample each row $a_j$ of $A$ independently with probability $p_j$ and add a row with $1/\sqrt{p_j}$ at the $j^{th}$ entry and $0$ elsewhere to $P$ for each such sampled row $a_j$. 
		%	\end{enumerate}
	%	Then the following holds with probability at least $1-\delta_{1}$:
	%	\begin{enumerate}
		%		\item $(1-\epsilon)\|Ax\|_2^2\leq \|PAx\|_2^2\leq (1+\epsilon)\|Ax\|_2^2$ for all $x\in \mathbb{C}^{d}$.
		%		\item $s\leq \frac{C\log(r/\delta_1)}{\epsilon^2}\sum_{j=1}^{d}\wt{\tau}_{j}$.
		%	\end{enumerate}
	%\end{lemma}
	%\fi
	%
	%Using \ref{def:levsampling}, we are ready to state \ref{thm:updatedleveragesampling}. 
	%\begin{theorem}[High-probability $(1+\epsilon)$-regression using leverage scores]\label{thm:updatedleveragesampling}
	%Suppose we are given $A \in \mathbb{R}^{d \times r}$, query access to $b \in \mathbb{R}^d$, an accuracy parameter $\epsilon>0$, failure probability $\eta>0$, and leverage score upper bounds  $\wt{\tau}_j$ that satisfy $\wt{\tau}_j \ge \tau_j(A)$ for all $j \in [n]$. Suppose further that $\sum_j\wt{\tau}_j = T$. 
	%
	%Let $\mathcal{S} \in \mathbb{R}^{m \times d}$ be a random sampling matrix drawn according to \ref{def:levsampling}, using the distribution $\wt{\tau}_j$ and $m=O\big(\frac{T \log^2(T) \log(1/\eta)}{\epsilon^9}\big)$ samples. Then there is an algorithm \texttt{LevSample}($\mathcal{S}A$, $\mathcal{S}b$, $\epsilon$, $\eta$) outputting with probability $1-\eta$ over the randomness of $S$,
	%\begin{enumerate}
	%\item $\wt{x} \in \R^d$ satisfying $\|A\wt{x}-b\|_2 \leq (1+\epsilon)\min_{x \in \mathbb{R}^r}\|Ax-b\|$.
	%\item An approximate cost $val(\wt x) \in \R$ satisfying $|val(\wt x) - \|A\wt{x}-b\|_2 - C | \le \epsilon \cdot  \|A\wt{x}-b\|_2$ where $C$ is a constant that depends only on the leverage score upper bounds $\{\tilde \tau_j \}_{j \in [n]}$ and $b$.
	%\end{enumerate}
	%\end{theorem}
	%\begin{proof}
	%\Cam{Cameron will do later tonight.}
	%This theorem follows\footnote{Although the original theorem statement from \cite{musco2021active} assumes access to the exact leverage scores, all proofs go through using only leverage score \emph{upper bounds} as well.} by combining Theorem 3.4 and Section 4 of \cite{musco2021active} for the $\ell_2$ norm, i.e. $p=2$.
	%\end{proof}
	
	%\iffalse
	%We will need one more result from \cite{musco2021active} to enable our sublinear sample complexity algorithm. In the notation of \ref{thm:updatedleveragesampling}, after sampling by leverage scores, we also need the sampled error estimate of the computed coefficients $\|\mathcal{S}A\tilde{x}-\mathcal{S}b\|_2$ to capture well the true error $\|A\tilde{x}-b\|_2$. The following theorem shows that this will hold up to a constant offset.
	%
	%\begin{theorem}\label{thm:leverage_score_error}
	%	In the setting of \ref{thm:updatedleveragesampling}, $\tilde{x}$ satisfies the following inequality:
	%	\begin{align*}
		%		\| \|\mathcal{S}A\tilde{x}-\Sb\|_2 - \|A\tilde{x}-b\|_2 \| = 
		%	\end{align*}
	%\end{theorem}
	%
	%This theorem follows from Lemma 3.7 and the proof of Theorem 3.4 in \cite{musco2021active}.
	%\fi 
	
	%Let $F_S \in \mathbb{C}^{d \times r}$ be a symmetric Fourier matrix corresponding to some frequencies $S=\{f_1,\dots,f_{r/2}\} \subset [0,1]$ as in \ref{def:symmetric_fourier_matrix}. In our setting, we will obtain non-trivial leverage score upper bounds on $WF_S$, which are crucially \emph{universal} (in the sense that they are independent of $S$). The importance of having \emph{universal} leverage score bounds is that a single set of samples will work for \emph{all} possible guesses of the true frequencies $\tilde{S}$ in our brute force search. However, note that \ref{thm:updatedleveragesampling} applies only to \emph{real} matrices as stated. In the notation of \ref{thm:updatedleveragesampling}, although we are sampling a real-valued vector $b$ (corresponding to the weighted first column of $T$) and seeking a real-valued vector $x$, the regression matrix itself is complex, $A=WF_S$. This is possible only because we would like to require that $x$ takes equal values at indices corresponding to symmetric frequencies (in the sense of \ref{thm:vandermonde}).
	
	
	\subsection{Full algorithm.}
	
	Equipped with these tools, we now describe the recovery algorithm and its guarantees. %The proofs of the previous lemmas are presented in the next sub-section after the proof of correctness of the algorithm.
	
	\begin{algorithm}[H]
		\caption{\textsc{ToeplitzRecovery}}
		\label{toeplitzrecovery}
		\begin{algorithmic}[1]
			
			\STATE $\textbf{Input:}$ Query access to $T\in \mathbb{R}^{d\times d}$, $k, \epsilon, \delta$.
			\STATE $\textbf{Init:}$ Set $r_1=O(k\log^8d/\eps)$, $r_2 = O(\log d +\log(1/\delta))$, $\eta=\frac{1}{100|N|^{r_1}}$, $\wt{\tau}_j$ as defined in \ref{leveragescorebound}, $\mathcal{N}_{d,r_1,r_2,\gamma}$ and $\mathcal{N}_{d,2r_1,r_2,\gamma}$ as defined in \ref{def:search}, and $\gamma= \delta / (2^{C_2 \log^7(d)})$ as in \ref{frobeniusexistence}.
			\STATE Draw $\mathcal{S}_1$ according to \ref{def:levsampling}, using $\wt{\tau}_j$ with $m=\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^2} \Big)$ samples. 
			\STATE Set $\tilde S, \tilde a = \argmin_{S \in \mathcal{N}_{d,r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{\mathcal{S}_1WF_SR_S a - \mathcal{S}_1WT_1}_2$.
			
			\STATE Set $T_R = T_1 - F_{\tilde{S}}R_{\tilde{S}}\ta$ .
			
			\STATE Draw $\mathcal{S}_2$ according to \ref{def:levsampling}, using $\wt{\tau}_j$ with $m=\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{6}} \Big)$ samples.
			\STATE Set $S', a' = \argmin_{S \in \mathcal{N}_{d,2r_1,r_2,\gamma}, a \in \R^{|S|}} \norm{\mathcal{S}_2WF_SR_S a - \mathcal{S}_2WT_R}_2$.
			
			\STATE Set $\bar{S} := \tilde{S} \cup S'$, $d := \bar{a} = [\tilde{a}; a']$, and $F = F_{\bar{S}}$.
			\STATE $\textbf{Return:}$ $F,d$.
		\end{algorithmic}
	\end{algorithm}
	
	\begin{reptheorem}{sublinearqueryalgo}
		Assume we are given query access to a PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$ and parameters $k,\epsilon, \delta$. Let $r = \wt{O}(\frac{k}{\epsilon}\log(1/\delta))$. Then Algorithm \ref{toeplitzrecovery} returns $F\in \mathbb{C}^{d\times \ell},d\in \mathbb{R}^{\ell}$ such that $F \diag(d)F^{*}$ is a symmetric Toeplitz matrix of rank at most $\ell = O(r)$ and the following holds.
		\begin{enumerate}
			\item Algorithm \ref{toeplitzrecovery} makes $\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{6}} \Big)$ queries to $T$. 
			\item $\|T-F\diag(d)F^{*}\|_F\leq (1+3\epsilon)\|T-T_k\|_F + 2\delta \|T\|_F$ with probability at least $97/100$. 
		\end{enumerate}
	\end{reptheorem}
	\begin{proof}
		By \ref{thm:const}, with probability at least $98/100$, $\tilde{S}$ and $\ta$ satisfy \ref{lem:regressionReduction} with $\alpha=41$. The conditions for \ref{thm:relative} are then satisfied, so with conditional probability at least $99/100$, the Toeplitz matrix $\bar{T} := F\diag(d)F^*$ satisfies 
		$$ \norm{T - \bar{T}}_F \leq (1+3\epsilon) \norm{T-T_k}_F + 2 \delta \norm{T}_F.$$
		By a union bound, the matrix $\bar{T} := F\diag(d)F^*$ based on the output of Algorithm \ref{toeplitzrecovery} then satisfies $\norm{T - \bar{T}}_F \leq (1+3\epsilon) \norm{T-T_k}_F + 2 \delta \norm{T}_F$ with probability at least $97/100$. 
		The overall sample complexity is  $\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{6}} \Big)$, as this is the sample complexity of $\mcS_2$ and dominates that of $\mcS_1$.  
	\end{proof}
	
	% old algo and thm below
	\iffalse
	\begin{algorithm}[H] 
		\SetAlgoLined
		$\textbf{Input:}$ Query access to $T\in \mathbb{R}^{d\times d}$, $k, \epsilon, \delta,\gamma$\; 
		$\textbf{Init:}$ Set $N=\{\frac{1}{2d},\frac{3}{2d},\ldots, 1-\frac{1}{2d}\}$, $r_1=O(k\log^8d/\eps)$, $r_2 = O(\log d +\log(1/\delta))$, $\eta=\frac{1}{100|N|^{r_1}}$ \; %\Cam{Make sure $r_1$ and $r_2$ exactly match valued defined in Thm 4, which I think have changed a little (and which I've suggested more changes to).}
		Set $F = [0]_{d\times r_1r_2}$, $d = [0]_{r_1r_2\times 1}$ and $OPT=0$\;
		%Let $P\in \mathbb{R}^{s\times d}$ be an i.i.d. sampling matrix as per Lemmas \ref{leveragescoresampling} and \ref{leveragescorebound} \;
		Draw $\mathcal{S}$ according to \ref{def:levsampling}, using $\wt{\tau}_j$ (from \ref{leveragescorebound}) with $m=\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{11}} \Big)$ %O\big(\frac{r\log^2(d)\log^3(r)\log(1/\delta)}{\epsilon^9}\big)$ 
		samples \\
		\For{all $B\in N^{r_1}$}{
			For all $f_i\in B$ define $B_i$ as follows:
			\begin{equation*}
				B_i = \underset{1\leq j\leq r_2}{\bigcup}\{f_i+\gamma j,f_i-\gamma j\} %,-(f_i+\gamma j),-(f_i-\gamma j)\}
			\end{equation*}
			Let $F_{S(B)}$ be the symmetric Fourier matrix corresponding to $S(B)=\underset{1\leq i\leq r_1}{\bigcup}B_i$\;
			
			Let $val(d_{S(B)}), \: d_{S(B)} = \texttt{LevSample}(\mathcal{S}WF_{S(B)}R_{S(B)}, \mathcal{S}WT_1, \epsilon, \eta)$ %, and $val(d_{S(B)}) = \|\mathcal{S}WF_{S(B)}R_{S(B)}d_{S(B)}-\mathcal{S}WT_1\|_2$ 
			
			%Let $d_{S(B)} = \argmin_{x}\|PWF_{S(B)}x-PWT_1\|_2 $ and $val(d_{S(B)}) =\min_{x}\|PWF_{S(B)}x-PWT_1\|_2  $\;
			
			\textbf{If} $val(d_{S(B)})\leq OPT$ \textbf{then} $OPT = val(d_{S(B)}),F = F_{S(B)},d = R_{S(B)}d_{S(B)}$\;
		}
		
		$\textbf{Return:}$ $F,d$
		\caption{\textsc{ToeplitzRecovery}}\label{toeplitzrecovery}
	\end{algorithm}
	
	\begin{theorem}\label{sublinearqueryalgo}
		Assume we are given query access to a PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$ and parameters $k,\epsilon, \delta$. \hltodo{How do we set/pick $\gamma$?} Let $r = r_1r_2 = \wt{O}(\frac{k}{\epsilon}\log(1/\delta))$. Then Algorithm \ref{toeplitzrecovery} returns $F\in \mathbb{C}^{d\times r},d\in \mathbb{R}^{r}$ such that $F \diag(d)F^{*}$ is a symmetric Toeplitz matrix of rank $O(r)$\hltodo{I added big O here - it's not exactly r} and the following holds.
		\begin{enumerate}
			\item Algorithm \ref{toeplitzrecovery} makes $\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{11}} \Big)$ %$O\big(\frac{r\log(d)\log^2(r) \log^2(r\log(d)\log(r)) \log(1/\delta)}{\epsilon^9}\big)$ %$\wt{O}(k^2\log(1/\delta))$
			queries to $T$. 
			\item $\|T-F\diag(d)F^{*}\|_F\leq (1+\epsilon)^2\|T-T_k\|_F + \delta(1+\epsilon) \|T\|_F$ with probability at least $99/100$. \hltodo{This guarantee needs to be updated and epsilon/delta modified based on the final guarantee}
		\end{enumerate}
	\end{theorem}
	
	Let $F_{\wt{S}},\wt{D}$ be the Fourier and diagonal matrices guaranteed to exist by Theorem \ref{frobeniusexistence}, and recall that $F$ and $d$ are the Fourier matrix and vector, respectively, returned by Algorithm \ref{toeplitzrecovery}.  Let $B',d' = \underset{B\in N^{r_1},x\in \mathbb{R}^{r}}{\argmin} \|W(F_{S(B)}x-T_1)\|_2$ and $F'=F_{S(B')}$. Since Algorithm \ref{toeplitzrecovery} brute force searches over all possible frequencies having the structure described in part \ref{thm:existence_freq_grid} of Theorem \ref{frobeniusexistence}, and uses the same $\gamma$ as per Theorem \ref{frobeniusexistence}, by Claim \ref{frobtoeuclid} we have the following:
	\begin{align*}
		\|WF'd'-WT_1\|_2&=\underset{B\in N^{r_1},x\in \mathbb{R}^{\frac{r}{2}}}{\min} \|W(F_{S(B)}x-T_1)\|_2 \\&= \underset{B\in N^{r_1},x\in \mathbb{R}^{\frac{r}{2}}}{\min} \|F_{S(B)}\diag(x) F_{S(B)}^{*}-T\|_F\\
		&\leq \|F_{\wt{S}}\wt{D}F_{\wt{S}}-T\|_F\\
		&\leq (1+\epsilon)\|T-T_k\|_F + \delta \|T\|_F.
	\end{align*}
	We then apply \ref{thm:updatedleveragesampling} with $\epsilon=\epsilon$, $\eta = \frac{1}{100|N|^{r_1}}$, and the upper bounds $\wt{\tau}_j$ are as described in \ref{leveragescorebound}, and crucially use the \emph{same} samples every time \texttt{LevSample} is called. Since the probability of failure each time \texttt{LevSample} is called is at most $\eta = \frac{1}{100|N|^{r_1}}$, and \texttt{LevSample} is called $|N|^{r_1}$ times, via a union bound the probability that any one of the calls fails is at most $\frac{1}{100}$. Therefore, with probability at least $\frac{99}{100}$, every call to $\texttt{LevSample}$ returns a $(1+\epsilon)$-approximation and a validation error satisfying (2) of \ref{thm:updatedleveragesampling}. When this occurs, then we can upper bound the error $||F\diag(d)F^*-T||_F = ||WFd - WT_1||_2$ of the returned matrix as follows.
	
	First, by part (2) of \ref{thm:updatedleveragesampling}, observe that $val(d)$ is within $\epsilon\|WFd-WT_1\|_2$ of $\| WFd-WT_1\|_2 + C$, and likewise for $val(d')$:
	\begin{align*}
		|val(d) - (\| WFd-WT_1\|_2 + C)| &\leq \epsilon\|WFd-WT_1\|_2 \\
		|val(d') - (\| WF'd'-WT_1\|_2 + C)| &\leq \epsilon\|WF'd'-WT_1\|_2.
	\end{align*}
	Moreover, by design of Algorithm \ref{algorithm}, $val(d) \leq val(d')$. Therefore, $\|WFd-WT_1\|_2$ and $\|WF'd'-WT_1\|_2$ are within at most $\epsilon(\|WFd-WT_1\|_2 + \|WF'd'-WT_1\|_2)$ of one another, as shown below.
	\begin{align*}
		\|WFd-WT_1\|_2 - \|WF'd'-WT_1\|_2 &= (\|WFd-WT_1\|_2 + C) - (\|WF'd'-WT_1\|_2 + C) \\
		&\leq (val(d) + \epsilon\|WFd-WT_1\|_2) - (val(d') -  \epsilon\|WF'd'-WT_1\|_2) \\
		&= (val(d) - val(d')) + \epsilon(\|WFd-WT_1\|_2 + \|WF'd'-WT_1\|_2) \\
		&\leq \epsilon(\|WFd-WT_1\|_2 + \|WF'd'-WT_1\|_2) 
	\end{align*}
	Rearranging terms and applying the previous bound on $\|WF'd'-WT_1\|_2$ then yields
	\begin{align*}
		\|WFd-WT_1\|_2 \leq \frac{1+\epsilon}{1-\epsilon} \|WF'd'-WT_1\|_2 \\
		\leq \frac{(1+\epsilon)^2}{1-\epsilon}\|T-T_k\|_F + \frac{\delta(1+\epsilon)}{1-\epsilon} \|T\|_F\\
	\end{align*}
	
	\iffalse
	\begin{align*}
		\|WFd - WT_1\|_2 &\leq (1+\epsilon) \min_{B\in N^{r_1}, x \in \mathbb{R}^{\frac{r}{2}}}\|WF_{S(B)}x-WT_1\|_2 \\  
		&\leq (1+\epsilon)^2 ||T-T_k|| + \delta (1+\epsilon)||T||_F
	\end{align*}
	The first inequality above followed by the guarantee of \ref{thm:updatedleveragesampling} combined with the optimality of $F$ and $d$, while the second inequality follows from the earlier bound on $\|WF'd'-WT_1\|_2$. 
	\fi
	
	Substituting $T = O(r\log(d)\log(r))$ into the guarantee of \ref{thm:updatedleveragesampling} yields $m=\tilde{O}\big(\frac{r\log^3(r)\log(1/\eta)}{\epsilon^{9}}\big)$, where $r=\tilde{O}(\frac{k \log(1/\delta)}{\epsilon})$ from \ref{sec:existence_main}, $|N| = O(d)$, $\eta = \frac{1}{100|N|^{r_1}}$, and $\tilde{O}$ notation hides $\log(d)$ factors. Further simplifying this expression completes the proof of the sample complexity of Algorithm \ref{toeplitzrecovery}.\hltodo{Use different $\epsilon$ for lev score and rest of paper so that the final guarantee is cleaner}
	
	\fi 
	
	
	\subsection{Leverage score bounds for weighted Fourier matrices.}\label{subsec:weighted_fourier_lev_bounds}
	In this subsection, we focus on proving the leverage score upper bounds for weighted Fourier matrices of Lemma \ref{leveragescorebound}. Recall the statement of Lemma \ref{leveragescorebound} was as follows.
	\begin{replemma}{leveragescorebound}
		Let $F_S\in \mathbb{C}^{d\times r}$ be any Fourier matrix with symmetric (in the sense of \ref{thm:vandermonde}) frequency set $S\subset [0,1], |S| = r\leq d$,$r\leq d$, and let $W$ be as defined in \ref{weightingdef} and and $M_S$ be any real valued matrix with $r$ rows. Then there exist non-negative numbers $\wt{\tau}_{j}$ for all $j\in [d]$ such that the following hold:
		\begin{enumerate}
			\item $\tau_j(WF_SM_S) \leq \tau_j(WF_S) \leq \wt{\tau}_{j}$ for all $j\in [d]$.
			\item $\sum_{j=1}^{d} \wt{\tau}_{j} \leq O(r\log (d)\log (r))$.
		\end{enumerate}
	\end{replemma}
	
	To prove this lemma, we will use the following three helper lemmas. %Their proofs are deferred to the end of this subsection. \hltodo{Is it really easier to defer these proofs? The proof of lemma 4.4 is already out of order}
	\begin{lemma}\label{levscore_reweight}
		Let $A \in \mathbb{C}^{d \times r}$ be a matrix, and let $D$ be a diagonal matrix with positive entries satisfying %$$\max_{i,j}\frac{D_{jj}}{D_{ii}} \leq C $$
		$$ \alpha \leq D_{ii}^2 \leq \beta .$$
		Then, 
		$$ \tau_i(DA) \leq \frac{\beta}{\alpha}\tau_i(A). $$
	\end{lemma}
	%We now finish this subsection with the proofs of helper Lemmas \ref{levscore_reweight} and \ref{levscore_submatrix}respectively. 
	\begin{proof}
		By the definition of leverage scores, we have the following:
		$$\tau_i(DA) = \max_{y\in \mathbb{C}^{r}} \frac{|DAy|_i^2}{\sum_{j=1}^d |DAy|_j^2}. $$
		For any $y$, the numerator is given by $|DAy|_i^2 = D_{ii}^2|Ay|_i^2$. The denominator satisfies
		$$ \sum_{j=1}^d |DAy|_j^2 \geq \alpha \sum_{j=1}^d |Ay|_j^2.$$
		As a result,
		$$ \max_{y\in \mathbb{C}^{r}} \frac{|DAy|_i^2}{\sum_{j=1}^d |DAy|_j^2} = \max_{y \in \mathbb{C}^{r}} \frac{D_{ii}^2|Ay|_i^2}{\sum_{j=1}^d |DAy|_j^2} \leq \max_{y\in \mathbb{C}^{r}} \frac{\beta|Ay|_i^2}{\alpha\sum_{j=1}^d |Ay|_j^2}.$$
		This proves that $ \tau_i(DA) \leq \frac{\beta}{\alpha}\tau_i(A)$ as desired.
	\end{proof}
	
	\begin{lemma}\label{levscore_submatrix}
		Let $A \in \mathbb{C}^{d \times r}$ be a matrix, and let $B \in \mathbb{C}^{d' \times r}$ be a matrix formed by taking any subset $R \subseteq [1,\dots,d]$ of the rows of $A$. Then the leverage score of any row $b_i$ in $B$ is at least the leverage score of row $b_i$ in $A$.
	\end{lemma}
	
	\begin{proof}
		Let $b_i$ correspond to the $i^{th}$ row of $A$ and the $i'^{th}$ row of $B$. Then by the definition of leverage scores we have the following.
		\begin{align*}
			\tau_i(A) &= \max_{y} \frac{|Ay|_i^2}{\sum_{j=1}^d |Ay|_j^2} \\
			&\leq \max_{y} \frac{|Ay|_i^2}{\sum_{j \in R} |Ay|_j^2} \\
			&= \max_{y} \frac{|By|_{i'}^2}{\sum_{j=1}^{d'} |By|_j^2} \\
			&= \tau_{i'}(B).
		\end{align*}
		This completes the proof of the lemma.
	\end{proof}
	\begin{lemma}\label{lemma:lev_score_col_span}
		Let $A \in \mathbb{C}^{d \times r}$ be a matrix, and let $B \in \mathbb{C}^{d \times r'}$ be a matrix formed by taking $r'$ linear combinations of the columns of $A$ (i.e. there is some matrix $M \in \mathbb{C}^{r \times r'}$ such that $B = AM$). Then the $i^{th}$ leverage score of $B$, $\tau_i(B)$, is at most the $i^{th}$ leverage score of $A$, $\tau_i(A)$. 
	\end{lemma}
	\begin{proof}
		We again rely on the maximization characterization of leverage scores: 
		\begin{align*}
			\tau_i(B) &= \max_{y} \frac{|By|_i^2}{\sum_{j=1}^d |By|_j^2} \\
			&= \max_{y} \frac{|AMy|_i^2}{\sum_{j=1}^d |AMy|_j^2} \\
			&\leq \max_{z} \frac{|Az|_i^2}{\sum_{j=1}^d |Az|_j^2} \\
			&= \tau_i(A).
		\end{align*}
		where the second inequality follows from the fact that $\{ My | y \in \mathbb{C}^{r'} \} \subseteq \{ z | z \in \mathbb{C}^r\}$.
	\end{proof}
	Equipped with these lemmas, the high level strategy for bounding the leverage scores of $WF_SM_S$ is as follows. By \ref{lemma:lev_score_col_span}, it suffices to bound the leverage scores of $WF_S$. To do so, first we will bucket the rows of $WF_S$ into submatrices, such that within each submatrix, the weights vary by at most a constant factor. We will then be able to bound the leverage scores of each submatrix using Lemma \ref{levscore_reweight}, and apply Lemma \ref{levscore_submatrix} to ensure that these upper bounds remain valid upper bounds for the entire matrix $WF_S$.
	
	Formally, begin by dividing $WF_S$ into submatrices as follows.
	\begin{definition}
		For all $i\in [\log d]$, let $W_i$ %\in \mathbb{R}^{(d/2^{i})\times d}$ 
		be the submatrix of $W$ consisting of rows with indices in $[d(1-1/2^{i-1})+1, d(1-1/2^{i})]$. For the edge case $i=(\log d) + 1$, let $W_i$ consist of only the last row of $WF_S$. For convenience, let $\mathcal{R}_i$ denote the index set of rows corresponding to $W_i$, and let $r_i = |\mathcal{R}_i|$ denote the number of rows in $W_i$. Note also that $r_i \leq \frac{d}{2^i}$ for $i \in [\log d]$, and $r_{\log d + 1} = 1$. 
	\end{definition}
	Then we can write $WF_S$ as $WF_S = [(W_1F_S)^{T};\ldots; (W_{\log d +1}F_S)^{T}]^{T}$. Now consider any $i\in [\log d +1]$ and $W_i F_S$. Since $W_i$ is diagonal and $d/2^{i-1}\leq (W_{i})_{j,j}^2 \leq 2d/2^{i-1}$ for all $j\in [r_i]$, applying Lemma \ref{levscore_reweight} with $\beta = 2\alpha = 2d/2^{i}$ we get the following for all $i\in [\log d + 1]$:
	\begin{equation*}
		\tau_{j}(W_i F_S) \leq 2 \tau_{j}(F_{S,i}) \quad \forall j\in [r_i].
	\end{equation*}
	Here, $F_{S,i}\in \mathbb{C}^{r_i\times s}$ is the matrix consisting of all rows of $F_{S}$ in the index set $\mathcal{R}_i$. %$d(1-1/2^{i-1})+1$ to the $d(1-1/2^{i})$ row.
	Note that the column span of $F_{S,i}$ and the first $r_i$ rows of $F_S$ is identical. This is because the $j^{th}$ column of $F_{S,i}$ is %just $e^{2\pi i (d(1-1/2^{i-1})f_j)}$, which is 
	a constant times the $j^{th}$ column of the matrix formed by considering the first $r_i$ rows of $F_S$. Since the first $r_i$ rows of $F_S$ forms a $r_i \times r$ Fourier matrix, their leverage scores are then identical as well. Finally, we appeal to Corollary C.2 of \cite{eldar2020toeplitz}, restated below:
	\begin{corollary}[Corollary C.2 of \cite{eldar2020toeplitz}]\label{corr:C2_eldar}
		For any positive integers $d$ and $s \leq d$, there is an explicit set of values $\wt{\tau}_1^{(s)},\dots,\wt{\tau}_d^{(s)} \in (0,1])$ such that, for any Fourier matrix $F_S \in \mathbb{C}^{d \times s}$ with leverage scores $\tau_1,\dots,\tau_d$,
		\begin{align*}
			&\forall j, \wt{\tau}_j^{(s)} \geq \tau_j .\\
			& \sum_{j=1}^d \wt{\tau}_j^{(s)} = O(s \log s).
		\end{align*}
	\end{corollary}
	
	Thus by Corollary \ref{corr:C2_eldar} (C.2 of \cite{eldar2020toeplitz}), we easily obtain the following claim.
	\begin{claim}\label{levscore_upperbound}
		For any $i\in [\log (d/r)]$ and any $j\in [r_i]$ define $\wt{\tau}_{j,i}$ as follows.
		\begin{equation*}
			\wt{\tau}_{j,i} = \min\left(1,\frac{r}{\min(j,d/2^i+1-j)},\frac{O(r^6\log^3 (r+1))}{(d/2^i)}\right).
		\end{equation*}
		For any $\log(d/r)<i\leq \log(d)$ and $j\in [r_i]$ let $\wt{\tau}_{j,i}=1$. Then we have the following.
		\begin{enumerate}
			\item $\tau_j(W_iF_S) \leq \wt{\tau}_{j,i}$ for all $i\in [\log d]$ and $j\in [r_i]$.
			\item $\sum_{j=1}^{d/2^i} \wt{\tau}_{j} \leq O(r\log r)$ for all $i\in [\log d]$.
		\end{enumerate}
	\end{claim}
	Equipped with these tools, we can now easily finish the proof of Lemma \ref{leveragescorebound}.
	\begin{proof}
		Define $\wt{\tau}_j$ values for $j\in [d]$ as follows.
		
		\begin{equation}
			\wt{\tau}_{j} = \wt{\tau}_{i,j'}.
		\end{equation}
		where $i,j'$ are chosen such that $d(1-1/2^{i-1})+1 \leq j\leq d(1-1/2^{i})$ and $j = d(1-1/2^{i-1})+1 + j'$, and $\wt{\tau}_{i,j}$ are obtained from Claim \ref{levscore_upperbound}. Finally, using Lemma \ref{levscore_submatrix} we can easily conclude that these upper bounds also serve as upper bounds on the leverage scores of $WF_S$, and by \ref{lemma:lev_score_col_span}, upper bounds on the leverage scores of $WF_SM_S$ as well. This completes the proof of Lemma \ref{leveragescorebound}.
	\end{proof}
	


==> approx_algorithm_old.tex <==
% !TEX root = ./main.tex

\section{Low-Rank Approximation with Sublinear Query Complexity}\label{algorithm}
%Now that we have established the existence of a good low rank approximation $\wt{T}$ which itself is Toeplitz, we present an alg orithm that constructs such a low rank approximation by only reading $poly(k)<<d$ entries of $T$. Note that we can trivially recover $T$ exactly by reading all the entries of the first column, that is the trivial sample complexity for this problem is $d$ samples. \\
In this section, we present our main algorithm, Algorithm \ref{sublinearqueryalgo} and prove the corresponding Theorem \ref{sublinearqueryalgo}, which shows that the algorithm outputs a near optimal low-rank approximation to $T$, while reading only sublinearly many entries. 
We treat $\wt{T}$, the low-rank Toeplitz approximation to $T$ (guaranteed to exist from Theorem \ref{frobeniusexistence}), as the true matrix, which we noisily access by reading entries of $T$.

\subsection{Main algorithm}

%\hltodo{Need to double check the sparsity is updated throughout this section for the $1+\epsilon$ approximation: $\wt{O}(\frac{k}{\epsilon}\log(\frac{1}{\delta}))$} 
The near optimal Toeplitz low-rank approximation $\wt T \in \R^{d \times d}$ guaranteed to exist by Theorem \ref{frobeniusexistence} is of the form $\wt T =F_{\wt{S}}\wt{D}F_{\wt{S}}^{*}$, where $ F_{\wt{S}}\in \mathbb{C}^{d\times r}$ and $\wt{D}\in \mathbb{R}^{\wt{O}(r\times r}$ are Fourier and diagonal matrices, respectively, and $r=\wt{O}(\frac{k}{\epsilon}\log(1/\delta))$. At a high level, Algorithm \ref{sublinearqueryalgo} uses brute force search to find the frequencies in $\wt{S}$. In particular, it uses an approximate regression oracle to test the quality of any guess for the frequencies in $\wt{S}$, without reading many entries of $T$.  

\hltodo{Need to double check the sparsity is updated throughout this section for the $1+\epsilon$ approximation: $\wt{O}(\frac{k}{\epsilon}\log(\frac{1}{\delta}))$} 
The near optimal Toeplitz low-rank approximation $\wt T \in \R^{d \times d}$ guaranteed to exist by Theorem \ref{frobeniusexistence} is of the form $\wt T =F_{\wt{S}}\wt{D}F_{\wt{S}}^{*}$, where $ F_{\wt{S}}\in \mathbb{C}^{d\times \wt{O}(\frac{k}{\epsilon}\log(1/\delta))}$ and $\wt{D}\in \mathbb{R}^{\wt{O}(\frac{k}{\epsilon}\log(1/\delta))\times \wt{O}(\frac{k}{\epsilon}\log(1/\delta))}$ are Fourier and diagonal weight matrices, respectively. At a high level, Algorithm \ref{sublinearqueryalgo} uses brute force search to find the frequencies in $\wt{S}$. In particular, it uses an approximate regression oracle to test the quality of any guess for the frequencies in $\wt{S}$, without reading many entries of $T$.  

Recall from Theorem \ref{frobeniusexistence} that these frequencies lie in $r_1 = \tilde O(k/\epsilon)$  clusters of equispaced frequencies centered around points in $N =\{1/2d,3/2d,\ldots, 1-1/2d\}$. Thus, our search space will be all subsets of $r_1$ elements of $N$, of which there at at most $N^{r_1}$. Since the first column of $\wt{T}$ defines $\wt{T}$, the approximate regression oracle will simply attempt to fit the first column of $\wt{T}$. However, since different entries in the first column of $\wt{T}$ appear with different frequencies in $\wt{T}$, we require the following weighting function to translate error bounds in the first column into error bounds for approximating the entire matrix $\wt{T}$ in the Frobenius norm. 
\begin{definition}\label{weightingdef}
	Let $w\in \mathbb{R}^{d}$ be defined as follows:
	\begin{equation*}
		w_{i} =  \begin{cases} 
			\sqrt{d} & i = 1 \\
			\sqrt{2(d-i+1)} & i > 1 
		\end{cases}
	\end{equation*}
	Let $W = \diag(w)\in \mathbb{R}^{d\times d}$.
\end{definition}
We have the following immediate claim, which expresses the Frobenius norm of a symmetric Toeplitz matrix as the weighted $\ell_2$ norm of its first column. 
\begin{claim}\label{frobtoeuclid}
	Let $T\in \mathbb{R}^{d\times d}$ be a symmetric Toeplitz matrix and let $T_{1}\in \mathbb{R}^{d}$ be its first column. Then $\|T\|_F = \|WT_1\|_2$, where $W$ is as in Definition \ref{weightingdef}.
\end{claim}
%While performing the brute force search over all possible frequencies, we need an approximate regression oracle which accesses only a few rows of the coefficient matrix ($F_S$) and entries of the label vector ($T_1$), and evaluates how well those frequencies fit the samples of $T$. We can achieve this using leverage score sampling, which requires bounding the sum of leverage scores of our coefficent matrix (a weighted Fourier matrix). We recall the definition of leverage scores (\ref{leveragescoresdefn}) as introduced in \cref{sec:preliminaries}.

\medskip

\noindent\textbf{Leverage Score Sampling.} 
To perform the brute force search over all possible frequency sets $\tilde S$, we need an approximate regression oracle, which accesses only a few entries of $T_1$. We will construct such an oracle using leverage score sampling. The \emph{leverage scores} \cite{spielman2011graph,drineas2006sampling} of a matrix are formally defined in \cref{leveragescoresdefn} below.
\begin{definition}\label{leveragescoresdefn}
	For any $A\in \mathbb{C}^{d\times r}$ and $j\in [d]$ let $\tau_j(A)$ denote the leverage score of the $j^{th}$ row of $A$:
	\begin{equation}
		\tau_j(A) = \max_{y\in \mathbb{C}^{s}} \frac{|(Ay)_i|^2}{\sum_{j=1}^d |(Ay)_j|^2}.
	\end{equation}
\end{definition}
It is known that leverage score sampling can be used to approximately solve linear regression problems in a sample-efficient manner. We will use  \cref{thm:updatedleveragesampling}, which formalizes this.  \cref{thm:updatedleveragesampling} gives worse $\epsilon$ and log dependencies than standard results on approximate regression with leverage score sampling \cite{Sarlos:2006vn,Woodruff:2014tg}. However, it provides two key guarantees that such theorems do not: 1) it gives a logarithmic dependence on the failure probability, which will be key in our setting, since we need to take a union bound over $N^{r_1}$ regression problems, and 2) it gives an estimate to the error of the approximate regression solution, which will be critical in choosing the set $\wt S$ that gives $\wt T$ best fitting $T$.
\iffalse
one can obtain spectral approximations to matrices by sampling their rows using probabilities proportional to their leverage scores. The following lemma formalizes this for complex matrices. 
\begin{lemma}[Corollary 5.2 in \cite{tropp2012user}]\label{leveragescoresampling}
	\hltodo{Do we still need this lemma? Check back}
	\mmtodoil{corollary 5.2 is matrix Chernoff, this lemma is considerably different to warrant some explanations how we get it from there.\\
	Is the first claim really true? I would personally expect that it holds with high probabilty for each $x$, not for all of them. }
	Given a matrix $A\in \mathbb{C}^{d\times r}$ and values $\wt{\tau}_{1},\ldots,\wt{\tau}_{d}\in [0,1]$ that satisfy the following for all $j\in [n]$.
	\begin{equation*}
		\wt{\tau}_{j}\geq \tau_{j}(A) 
	\end{equation*}
	Then there are universal constants $c,C$ such that if we perform the following:
	\begin{enumerate}
		\item Set $p_{j}= \min (1,c\wt{\tau}_{j}\log(r/\delta_{1})/\epsilon^2)$.
		\item Create a sampling matrix $P\in \mathbb{C}^{s\times d}$ that takes $s$ samples as follows - Sample each row $a_j$ of $A$ independently with probability $p_j$ and add a row with $1/\sqrt{p_j}$ at the $j^{th}$ entry and $0$ elsewhere to $P$ for each such sampled row $a_j$. 
	\end{enumerate}
	Then the following holds with probability at least $1-\delta_{1}$:
	\begin{enumerate}
		\item $(1-\epsilon)\|Ax\|_2^2\leq \|PAx\|_2^2\leq (1+\epsilon)\|Ax\|_2^2$ for all $x\in \mathbb{C}^{d}$.
		\item $s\leq \frac{C\log(r/\delta_1)}{\epsilon^2}\sum_{j=1}^{d}\wt{\tau}_{j}$.
	\end{enumerate}
\end{lemma}
\fi
First, we need to formally define leverage score \emph{sampling} below.
\begin{definition}[Leverage score sampling; Def. 2.7 of \cite{musco2021active}]\label{def:levsampling}
	For any number of samples $m$ and a set of leverage score bounds $\{\tilde \tau_j \}_{j \in [n]}$ (which upper bound the true leverage scores $\tau_j$ of some matrix with $d > m$ rows) with $T = \sum_{j=1}^d \wt{\tau}_j$, let $\mathcal{S} \in \mathbb{R}^{m \times d}$ be a sampling matrix with each row set independently to the $i^{th}$ standard basis vector multiplied by $(m \cdot p_i)^{-1/2}$, with probability 
	\begin{align*}
		p_i &= \frac{1}{2} \Bigg( \frac{\wt{\tau}_i}{T} + \frac{1}{d} \Bigg).
	\end{align*}
\end{definition}

Using \cref{def:levsampling}, we are ready to state \cref{thm:updatedleveragesampling}. 
\begin{theorem}[High-probability $(1+\epsilon)$-regression using leverage scores]\label{thm:updatedleveragesampling}
Suppose we are given $A \in \mathbb{R}^{d \times r}$, query access to $b \in \mathbb{R}^d$, an accuracy parameter $\epsilon>0$, failure probability $\eta>0$, and leverage score upper bounds  $\wt{\tau}_j$ that satisfy $\wt{\tau}_j \ge \tau_j(A)$ for all $j \in [n]$. Suppose further that $\sum_j\wt{\tau}_j = T$. 

Let $\mathcal{S} \in \mathbb{R}^{m \times d}$ be a random sampling matrix drawn according to \cref{def:levsampling}, using the distribution $\wt{\tau}_j$ and $m=O\big(\frac{T \log^2(T) \log(1/\eta)}{\epsilon^9}\big)$ samples. Then there is an algorithm \texttt{LevSample}($\mathcal{S}A$, $\mathcal{S}b$, $\epsilon$, $\eta$) outputting with probability $1-\eta$ over the randomness of $S$,
\begin{enumerate}
\item $\wt{x} \in \R^d$ satisfying $\|A\wt{x}-b\|_2 \leq (1+\epsilon)\min_{x \in \mathbb{R}^r}\|Ax-b\|$.
\item An approximate cost $val(\wt x) \in \R$ satisfying $|val(\wt x) - \|A\wt{x}-b\|_2 - C | \le \epsilon \cdot  \|A\wt{x}-b\|_2$ where $C$ is a constant that depends only on the leverage score upper bounds $\{\tilde \tau_j \}_{j \in [n]}$ and $b$.
\end{enumerate}
\end{theorem}
\begin{proof}
\Cam{Cameron will do later tonight.}
This theorem follows\footnote{Although the original theorem statement from \cite{musco2021active} assumes access to the exact leverage scores, all proofs go through using only leverage score \emph{upper bounds} as well.} by combining Theorem 3.4 and Section 4 of \cite{musco2021active} for the $\ell_2$ norm, i.e. $p=2$.
\end{proof}

\iffalse
We will need one more result from \cite{musco2021active} to enable our sublinear sample complexity algorithm. In the notation of \cref{thm:updatedleveragesampling}, after sampling by leverage scores, we also need the sampled error estimate of the computed coefficients $\|\mathcal{S}A\tilde{x}-\mathcal{S}b\|_2$ to capture well the true error $\|A\tilde{x}-b\|_2$. The following theorem shows that this will hold up to a constant offset.

\begin{theorem}\label{thm:leverage_score_error}
	In the setting of \cref{thm:updatedleveragesampling}, $\tilde{x}$ satisfies the following inequality:
	\begin{align*}
		\| \|\mathcal{S}A\tilde{x}-\Sb\|_2 - \|A\tilde{x}-b\|_2 \| = 
	\end{align*}
\end{theorem}

This theorem follows from Lemma 3.7 and the proof of Theorem 3.4 in \cite{musco2021active}.
\fi 

Let $F_S \in \mathbb{C}^{d \times r}$ be a symmetric Fourier matrix corresponding to some frequencies $S=\{f_1,\dots,f_{r/2}\} \subset [0,1]$ as in \cref{def:symmetric_fourier_matrix}. In our setting, we will obtain non-trivial leverage score upper bounds on $WF_S$, which are crucially \emph{universal} (in the sense that they are independent of $S$). The importance of having \emph{universal} leverage score bounds is that a single set of samples will work for \emph{all} possible guesses of the true frequencies $\tilde{S}$ in our brute force search. However, note that \cref{thm:updatedleveragesampling} applies only to \emph{real} matrices as stated. In the notation of \cref{thm:updatedleveragesampling}, although we are sampling a real-valued vector $b$ (corresponding to the weighted first column of $T$) and seeking a real-valued vector $x$, the regression matrix itself is complex, $A=WF_S$. This is possible only because we would like to require that $x$ takes equal values at indices corresponding to symmetric frequencies (in the sense of \cref{thm:vandermonde}). To incorporate both this restriction on $x$ and the real-valued requirement of \cref{thm:updatedleveragesampling}, we introduce a new frequency-dependent matrix, $R_S$, which collapses the $2|S|=r$ conjugate pair columns of $WF_S$ into $|S|=\frac{r}{2}$ real-valued columns, each corresponding to a degree of freedom of $x$. %\Cam{Like in Def 1.2 we need to result the issues of odd $r$ here.}

\begin{definition}\label{def:RS} 
Let $S \subset [0,\frac{1}{2})$ with $|S|=\frac{r}{2}$. % with $|S| = \frac{r}{2}$. 
Then, define the matrix $R_S \in \mathbb{R}^{2|S| \times |S|}$ (or equivalently $R_S \in \mathbb{R}^{r \times \frac{r}{2}}$) by setting the $j^{th}$ column $(R_S)_{:,j}$ equal to $0$ everywhere except at $j$ and $|S|+j$, corresponding to the $j^{th}$ \emph{pair} of conjugate frequencies, where it is equal to $1$. %(Here, we assume that both $S$ and the frequency pairs are ordered according to some arbitrary ordering.)  
%\Cam{Fix to match new notation later.}\hltodo{Checking back, it seems like $r$ is indeed used as the rank and $F_S$, $F_{-S}$ are ordered correspondingly? What exactly needs to be changed (or what earlier sec. has the inconsistency)?}
\end{definition}
%Note in the above definition that if $r$, the rank of a Toeplitz matrix, is odd, then there exists some frequency in its Vandermonde decomposition which is its own conjugate. According to the convention of \cref{def:symmetric_fourier_matrix}, the frequency set $S$ is then of size $\frac{r}{2} \rceil$, where the column vector of $F_S$ corresponding to the self-conjugate frequency is repeated. This motivates the dimensionality of $R_S$ in the case when $r$ is odd. 

It is trivial to check from this definition that $F_SR_S$ is always real-valued, so we can equivalently interpret $F_S$ applied to any $r$-length symmetric vector $x$ (which takes equal values on conjugate frequencies, ie. $x_j=x_{\frac{r}{2}+j}$ for $j\in[\frac{r}{2}]$) as $F_SR_S$ applied to the $\frac{r}{2}$-length scaled subset of $x$, $\frac{1}{2}R_S^Tx$. Therefore, we will apply leverage score sampling to the real-valued matrix $F_SR_S$, and optimize only over the desired $\frac{r}{2}$ degrees of freedom.

To apply \cref{thm:updatedleveragesampling} in the proof of our approximate regression oracle, we therefore need good upper bounds on the leverage scores of $WF_SR_S$. We obtain such bounds in this section, which are in fact independent of the frequencies $S$. This is formalized in the following lemma.
\begin{lemma}\label{leveragescorebound}
	Let $W$ be the weight matrix defined in \cref{weightingdef}. Then there exist non-negative numbers $\{\wt{\tau}_{j}\}_{j=1}^d$ such that the following hold for all frequency sets $S\subset [0,\frac{1}{2}), |S| = \frac{r}{2}\leq d$: 
	\begin{enumerate}
		\item $\tau_j(WF_SR_S) \leq \tau_j(WF_S) \leq \wt{\tau}_{j}$ for all $j\in [d]$.
		\item $\sum_{j=1}^{d} \wt{\tau}_{j} \leq O(r\log (d)\log (r))$.
	\end{enumerate}
	Here, $F_S\in \mathbb{C}^{d\times r}$ is the symmetric Fourier matrix with frequency set $S$ as defined in \cref{def:symmetric_fourier_matrix}, and $R_S$ is as defined in \cref{def:RS}. 

\end{lemma}
\cref{leveragescorebound} is similar to Corollary C.2 of \cite{eldar2020toeplitz}, but applies to \emph{weighted} Fourier matrices. (Corollary C.2 of \cite{eldar2020toeplitz} holds only for $W=I$, and does not have the $\log(d)$ dependence in the upper bound on $\sum_{j=1}^{d} \wt{\tau}_{j} $.) We will later restate Corollary C.2 of \cite{eldar2020toeplitz} as \cref{corr:C2_eldar}, and use it in the proof of \cref{leveragescorebound}, which we defer to \cref{subsec:weighted_fourier_lev_bounds}.

Equipped with these tools, we now describe the recovery algorithm and its guarantees. %The proofs of the previous lemmas are presented in the next sub-section after the proof of correctness of the algorithm.

\begin{algorithm}[H] 
	\SetAlgoLined
	$\textbf{Input:}$ Query access to $T\in \mathbb{R}^{d\times d}$, $k, \epsilon, \delta,\gamma$\; 
	$\textbf{Init:}$ Set $N=\{\frac{1}{2d},\frac{3}{2d},\ldots, 1-\frac{1}{2d}\}$, $r_1=O(k\log^8d/\eps)$, $r_2 = O(\log d +\log(1/\delta))$, $\eta=\frac{1}{100|N|^{r_1}}$ \; %\Cam{Make sure $r_1$ and $r_2$ exactly match valued defined in Thm 4, which I think have changed a little (and which I've suggested more changes to).}
	Set $F = [0]_{d\times r_1r_2}$, $d = [0]_{r_1r_2\times 1}$ and $OPT=0$\;
	%Let $P\in \mathbb{R}^{s\times d}$ be an i.i.d. sampling matrix as per Lemmas \ref{leveragescoresampling} and \ref{leveragescorebound} \;
	Draw $\mathcal{S}$ according to \cref{def:levsampling}, using $\wt{\tau}_j$ (from \cref{leveragescorebound}) with $m=\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{11}} \Big)$ %O\big(\frac{r\log^2(d)\log^3(r)\log(1/\delta)}{\epsilon^9}\big)$ 
	samples \\
	\For{all $B\in N^{r_1}$}{
		For all $f_i\in B$ define $B_i$ as follows:
		\begin{equation*}
			B_i = \underset{1\leq j\leq r_2}{\bigcup}\{f_i+\gamma j,f_i-\gamma j\} %,-(f_i+\gamma j),-(f_i-\gamma j)\}
		\end{equation*}
		Let $F_{S(B)}$ be the symmetric Fourier matrix corresponding to $S(B)=\underset{1\leq i\leq r_1}{\bigcup}B_i$\;
		
		Let $val(d_{S(B)}), \: d_{S(B)} = \texttt{LevSample}(\mathcal{S}WF_{S(B)}R_{S(B)}, \mathcal{S}WT_1, \epsilon, \eta)$ %, and $val(d_{S(B)}) = \|\mathcal{S}WF_{S(B)}R_{S(B)}d_{S(B)}-\mathcal{S}WT_1\|_2$ 

		%Let $d_{S(B)} = \argmin_{x}\|PWF_{S(B)}x-PWT_1\|_2 $ and $val(d_{S(B)}) =\min_{x}\|PWF_{S(B)}x-PWT_1\|_2  $\;

		\textbf{If} $val(d_{S(B)})\leq OPT$ \textbf{then} $OPT = val(d_{S(B)}),F = F_{S(B)},d = R_{S(B)}d_{S(B)}$\;
	}
	
	$\textbf{Return:}$ $F,d$
	\caption{\textsc{ToeplitzRecovery}}\label{toeplitzrecovery}
\end{algorithm}
\begin{theorem}\label{sublinearqueryalgo}
	Assume we are given query access to a PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$ and parameters $k,\delta$. Let  $r = r_1r_2 = \wt{O}(\frac{k}{\epsilon}\log(1/\delta))$. Then Algorithm \ref{toeplitzrecovery} returns $F\in \mathbb{C}^{d\times r},d\in \mathbb{R}^{r}$ such that $F \diag(d)F^{*}$ is a symmetric Toeplitz matrix of rank $O(r)$\hltodo{I added big O here - it's not exactly r} and the following holds.
	\begin{enumerate}
		\item Algorithm \ref{toeplitzrecovery} makes $\tilde{O}\Big( \frac{k^2\log(\frac{1}{\delta})}{\epsilon^{11}} \Big)$ %$O\big(\frac{r\log(d)\log^2(r) \log^2(r\log(d)\log(r)) \log(1/\delta)}{\epsilon^9}\big)$ %$\wt{O}(k^2\log(1/\delta))$
		 queries to $T$. 
		\item $\|T-F\diag(d)F^{*}\|_F\leq (1+\epsilon)^2\|T-T_k\|_F + \delta(1+\epsilon) \|T\|_F$ with probability at least $99/100$. \hltodo{This guarantee needs to be updated and epsilon/delta modified based on the final guarantee}
	\end{enumerate}
\end{theorem}
\begin{proof}
	
	Let $F_{\wt{S}},\wt{D}$ be the Fourier and diagonal matrices guaranteed to exist by Theorem \ref{frobeniusexistence}, and recall that $F$ and $d$ are the Fourier matrix and vector, respectively, returned by Algorithm \ref{toeplitzrecovery}.  Let $B',d' = \underset{B\in N^{r_1},x\in \mathbb{R}^{r}}{\argmin} \|W(F_{S(B)}x-T_1)\|_2$ and $F'=F_{S(B')}$. Since Algorithm \ref{toeplitzrecovery} brute force searches over all possible frequencies having the structure described in part \ref{thm:existence_freq_grid} of Theorem \ref{frobeniusexistence}, and uses the same $\gamma$ as per Theorem \ref{frobeniusexistence}, by Claim \ref{frobtoeuclid} we have the following:
	\begin{align*}
		\|WF'd'-WT_1\|_2&=\underset{B\in N^{r_1},x\in \mathbb{R}^{\frac{r}{2}}}{\min} \|W(F_{S(B)}x-T_1)\|_2 \\&= \underset{B\in N^{r_1},x\in \mathbb{R}^{\frac{r}{2}}}{\min} \|F_{S(B)}\diag(x) F_{S(B)}^{*}-T\|_F\\
		&\leq \|F_{\wt{S}}\wt{D}F_{\wt{S}}-T\|_F\\
		&\leq (1+\epsilon)\|T-T_k\|_F + \delta \|T\|_F.
	\end{align*}
	We then apply \cref{thm:updatedleveragesampling} with $\epsilon=\epsilon$, $\eta = \frac{1}{100|N|^{r_1}}$, and the upper bounds $\wt{\tau}_j$ are as described in \cref{leveragescorebound}, and crucially use the \emph{same} samples every time \texttt{LevSample} is called. Since the probability of failure each time \texttt{LevSample} is called is at most $\eta = \frac{1}{100|N|^{r_1}}$, and \texttt{LevSample} is called $|N|^{r_1}$ times, via a union bound the probability that any one of the calls fails is at most $\frac{1}{100}$. Therefore, with probability at least $\frac{99}{100}$, every call to $\texttt{LevSample}$ returns a $(1+\epsilon)$-approximation and a validation error satisfying (2) of \cref{thm:updatedleveragesampling}. When this occurs, then we can upper bound the error $||F\diag(d)F^*-T||_F = ||WFd - WT_1||_2$ of the returned matrix as follows.

	First, by part (2) of \cref{thm:updatedleveragesampling}, observe that $val(d)$ is within $\epsilon\|WFd-WT_1\|_2$ of $\| WFd-WT_1\|_2 + C$, and likewise for $val(d')$:
	\begin{align*}
		|val(d) - (\| WFd-WT_1\|_2 + C)| &\leq \epsilon\|WFd-WT_1\|_2 \\
		|val(d') - (\| WF'd'-WT_1\|_2 + C)| &\leq \epsilon\|WF'd'-WT_1\|_2.
	\end{align*}
	Moreover, by design of Algorithm \ref{algorithm}, $val(d) \leq val(d')$. Therefore, $\|WFd-WT_1\|_2$ and $\|WF'd'-WT_1\|_2$ are within at most $\epsilon(\|WFd-WT_1\|_2 + \|WF'd'-WT_1\|_2)$ of one another, as shown below.
	\begin{align*}
		\|WFd-WT_1\|_2 - \|WF'd'-WT_1\|_2 &= (\|WFd-WT_1\|_2 + C) - (\|WF'd'-WT_1\|_2 + C) \\
		&\leq (val(d) + \epsilon\|WFd-WT_1\|_2) - (val(d') -  \epsilon\|WF'd'-WT_1\|_2) \\
		&= (val(d) - val(d')) + \epsilon(\|WFd-WT_1\|_2 + \|WF'd'-WT_1\|_2) \\
		&\leq \epsilon(\|WFd-WT_1\|_2 + \|WF'd'-WT_1\|_2) 
	\end{align*}
	Rearranging terms and applying the previous bound on $\|WF'd'-WT_1\|_2$ then yields
	\begin{align*}
		\|WFd-WT_1\|_2 \leq \frac{1+\epsilon}{1-\epsilon} \|WF'd'-WT_1\|_2 \\
		\leq \frac{(1+\epsilon)^2}{1-\epsilon}\|T-T_k\|_F + \frac{\delta(1+\epsilon)}{1-\epsilon} \|T\|_F\\
	\end{align*}
 
	\iffalse
	\begin{align*}
		\|WFd - WT_1\|_2 &\leq (1+\epsilon) \min_{B\in N^{r_1}, x \in \mathbb{R}^{\frac{r}{2}}}\|WF_{S(B)}x-WT_1\|_2 \\  
		&\leq (1+\epsilon)^2 ||T-T_k|| + \delta (1+\epsilon)||T||_F
	\end{align*}
	The first inequality above followed by the guarantee of \cref{thm:updatedleveragesampling} combined with the optimality of $F$ and $d$, while the second inequality follows from the earlier bound on $\|WF'd'-WT_1\|_2$. 
	\fi

	Substituting $T = O(r\log(d)\log(r))$ into the guarantee of \cref{thm:updatedleveragesampling} yields $m=\tilde{O}\big(\frac{r\log^3(r)\log(1/\eta)}{\epsilon^{9}}\big)$, where $r=\tilde{O}(\frac{k \log(1/\delta)}{\epsilon})$ from \cref{sec:existence_main}, $|N| = O(d)$, $\eta = \frac{1}{100|N|^{r_1}}$, and $\tilde{O}$ notation hides $\log(d)$ factors. Further simplifying this expression completes the proof of the sample complexity of Algorithm \ref{toeplitzrecovery}.\hltodo{Use different $\epsilon$ for lev score and rest of paper so that the final guarantee is cleaner}

	% below: the old proof (constant factor approx)

	\hltodoil{Old proof below, uncommenting}

	We can write $\|WFd - WF'd'\|_2$ as $\|W[F;F']([d^{T};{d'}^{T}])^{T}\|_2$. Here $[F;F']\in \mathbb{C}^{d\times 2r}$ is also a Fourier matrix. We apply Lemma \ref{leveragescoresampling} with $\epsilon=9$, $\delta_{1} = 1/(100|N|^{r_1})$, and $\wt{\tau}_j$ values for $d\times 2r$ dimensional weighted Fourier matrices as per Lemma \ref{leveragescorebound} to obtain a sampling matrix $P\in \mathbb{R}^{s\times d}$ that takes $s=O(\log(d|N|^{r_1}) 2r \log (d)\log (r)) = \wt{O}(k^2\log(1/\delta))$ samples. Taking a union bound over all $B\in N^{r_1}$ we get the following which holds with probability at least $1-|N|^{r_1}\delta_1 = 99/100$ over the choice of $P$.
	\begin{align*}
		\|PW[F_{S(B)};F']x\|_2 \leq 10 \|W[F_{S(B)};F']x\|_2 \quad \forall B\in N^{r_1}, x\in \mathbb{C}^{2r}
	\end{align*}
	This in particular implies that  the following holds with probability at least $99/100$.
	\begin{align*}
		\|WFd - WF'd'\|_2 &\leq 10 \|PWFd - PWF'd'\|_2\\
		&\leq 10 (\|PWFd - PWT_1\|_2 + \|PWF'd' - PWT_1\|_2)\\
		&\leq 10 (\|PWF'd' - PWT_1\|_2 + \|PWF'd' - PWT_1\|_2)\\
		&= 20\|PWF'd'-PWT_1\|_2
	\end{align*}
	Where the third inequality follows by observing that $F,d = \underset{B\in N^{r_1},x\in \mathbb{R}^{r}}{\argmin} \|PWF_{S(B)}x-PWT_1\|_2$. Now by the unbiasedness property of the sampling matrix $P$ as per Lemma \ref{leveragescoresampling} we get that $\mathbb{E}[\|PWF'd'-PWT_1\|_2^2] = \|WF'd'-WT_1\|_2^2$. Thus applying Markov's inequality we get that $\|PWF'd'-PWT_1\|_2\leq 10 \|WF'd'-WT_1\|_2$ with probability $99/100$. Thus taking a union bound we get that the following holds with probabililty at least $98/100$ over the choice of $P$.
	\begin{align*}
		\|WFd - WT_1\|_2 &\leq \|WF'd'-WT_1\|_2 + \|WFd - WF'd'\|_2	\\		
		&\leq \|WF'd'-WT_1\|_2 +  20\|PWF'd'-PWT_1\|_2\\
		& \leq \|WF'd'-WT_1\|_2 +  200\|WF'd'-WT_1\|_2 \\
		& \leq 201\|WF'd'-WT_1\|_2\\
		& \leq \wt{O}(1)\|T-T_k\|_F + \delta \|T\|_F
	\end{align*}
	Thus we can finally conclude the following which completes the proof of point 2 of the theorem.
	\begin{equation*}
		\|F\diag(d)F^{*}-T\|_F = \|WFd - WT_1\|_2 \leq \wt{O}(1)\|T-T_k\|_F + \delta \|T\|_F
	\end{equation*}
	Note that while computing $d_{S(B)} = \argmin_{x}\|PWF_{S(B)} - PWT_1\|_2$ for any $B\in N^{r_1}$ we can restrict $x$ to have the same value for any frequency and its negative counterpart. This would ensure that $ F_{S(B)}\diag(d_{S(B)})F_{S(B)}^{*}$ is a real symmetric Toeplitz matrix for any $B\in N^{r_1}$. The proof above goes through even with this modification. Finally, we only need to know $PWT_1$ while executing our algorithm. This requires reading just $s=\wt{O}(k^2\log(1/\delta))$ entries of $T_1$, as specified by the $s\times d$ sampling matrix $P$.

\end{proof}

\subsection{Leverage score bounds for weighted Fourier matrices}\label{subsec:weighted_fourier_lev_bounds}
In this subsection, we focus on proving the leverage score upper bounds for weighted Fourier matrices of Lemma \ref{leveragescorebound}. Recall the statement of Lemma \ref{leveragescorebound} was as follows.
\begin{replemma}{leveragescorebound}
	Let $F_S\in \mathbb{C}^{d\times r}$ be any Fourier matrix with symmetric (in the sense of \cref{thm:vandermonde}) frequency set $S\subset [0,1], |S| = r\leq d$,$r\leq d$, and let $W$ and $R_S$ be as defined in \cref{weightingdef} and \cref{def:RS}. Then there exist non-negative numbers $\wt{\tau}_{j}$ for all $j\in [d]$ such that the following hold:
	\begin{enumerate}
		\item $\tau_j(WF_SR_S) \leq \tau_j(WF_S) \leq \wt{\tau}_{j}$ for all $j\in [d]$.
		\item $\sum_{j=1}^{d} \wt{\tau}_{j} \leq O(r\log (d)\log (r))$.
	\end{enumerate}
\end{replemma}

To prove this lemma, we will use the following three helper lemmas. %Their proofs are deferred to the end of this subsection. \hltodo{Is it really easier to defer these proofs? The proof of lemma 4.4 is already out of order}
\begin{lemma}\label{levscore_reweight}
Let $A \in \mathbb{C}^{d \times r}$ be a matrix, and let $D$ be a diagonal matrix with positive entries satisfying %$$\max_{i,j}\frac{D_{jj}}{D_{ii}} \leq C $$
$$ \alpha \leq D_{ii}^2 \leq \beta $$
Then, 
$$ \tau_i(DA) \leq \frac{\beta}{\alpha}\tau_i(A) $$
\end{lemma}
%We now finish this subsection with the proofs of helper Lemmas \ref{levscore_reweight} and \ref{levscore_submatrix}respectively. 
\begin{proof}[Proof of Lemma \ref{levscore_reweight}]
	By the definition of leverage scores, we have the following:
	$$\tau_i(DA) = \max_{y\in \mathbb{C}^{r}} \frac{|DAy|_i^2}{\sum_{j=1}^d |DAy|_j^2} $$
	For any $y$, the numerator is given by $|DAy|_i^2 = D_{ii}^2|Ay|_i^2$. The denominator satisfies
	$$ \sum_{j=1}^d |DAy|_j^2 \geq \alpha \sum_{j=1}^d |Ay|_j^2$$
	As a result,
	$$ \max_{y\in \mathbb{C}^{r}} \frac{|DAy|_i^2}{\sum_{j=1}^d |DAy|_j^2} = \max_{y \in \mathbb{C}^{r}} \frac{D_{ii}^2|Ay|_i^2}{\sum_{j=1}^d |DAy|_j^2} \leq \max_{y\in \mathbb{C}^{r}} \frac{\beta|Ay|_i^2}{\alpha\sum_{j=1}^d |Ay|_j^2}$$
	This proves that $ \tau_i(DA) \leq \frac{\beta}{\alpha}\tau_i(A)$ as desired.
\end{proof}

\begin{lemma}\label{levscore_submatrix}
Let $A \in \mathbb{C}^{d \times r}$ be a matrix, and let $B \in \mathbb{C}^{d' \times r}$ be a matrix formed by taking any subset $R \subseteq [1,\dots,d]$ of the rows of $A$. Then the leverage score of any row $b_i$ in $B$ is at least the leverage score of row $b_i$ in $A$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{levscore_submatrix}]
	Let $b_i$ correspond to the $i^{th}$ row of $A$ and the $i'^{th}$ row of $B$. Then by the definition of leverage scores we have the following.
	\begin{align*}
		\tau_i(A) &= \max_{y} \frac{|Ay|_i^2}{\sum_{j=1}^d |Ay|_j^2} \\
		&\leq \max_{y} \frac{|Ay|_i^2}{\sum_{j \in R} |Ay|_j^2} \\
		&= \max_{y} \frac{|By|_{i'}^2}{\sum_{j=1}^{d'} |By|_j^2} \\
		&= \tau_{i'}(B)
	\end{align*}
	
\end{proof}
\begin{lemma}\label{lemma:lev_score_col_span}
	Let $A \in \mathbb{C}^{d \times r}$ be a matrix, and let $B \in \mathbb{C}^{d \times r'}$ be a matrix formed by taking $r'<r$ linear combinations of the columns of $A$ (i.e. there is some matrix $M \in \mathbb{C}^{r \times r'}$ such that $B = AM$). Then the $i^{th}$ leverage score of $B$, $\tau_i(B)$, is at most the $i^{th}$ leverage score of $A$, $\tau_i(A)$. 
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:lev_score_col_span}]
	We again rely on the maximization characterization of leverage scores: 
	\begin{align*}
		\tau_i(B) &= \max_{y} \frac{|By|_i^2}{\sum_{j=1}^d |By|_j^2} \\
		&= \max_{y} \frac{|AMy|_i^2}{\sum_{j=1}^d |AMy|_j^2} \\
		&\leq \max_{z} \frac{|Az|_i^2}{\sum_{j=1}^d |Az|_j^2} \\
		&= \tau_i(A)
	\end{align*}
	where the second inequality follows from the fact that $\{ My | y \in \mathbb{C}^{r'} \} \subseteq \{ z | z \in \mathbb{C}^r\}$.
\end{proof}
Equipped with these lemmas, the high level strategy for bounding the leverage scores of $WF_SR_S$ is as follows. By \cref{lemma:lev_score_col_span}, it suffices to bound the leverage scores of $WF_S$. To do so, first we will bucket the rows of $WF_S$ into submatrices, such that within each submatrix, the weights vary by at most a constant factor. We will then be able to bound the leverage scores of each submatrix using Lemma \ref{levscore_reweight}, and apply Lemma \ref{levscore_submatrix} to ensure that these upper bounds remain valid upper bounds for the entire matrix $WF_S$.

Formally, begin by dividing $WF_S$ into submatrices as follows.
\begin{definition}
For all $i\in [\log d]$, let $W_i$ %\in \mathbb{R}^{(d/2^{i})\times d}$ 
be the submatrix of $W$ consisting of rows with indices in $[d(1-1/2^{i-1})+1, d(1-1/2^{i})]$. For the edge case $i=(\log d) + 1$, let $W_i$ consist of only the last row of $WF_S$. For convenience, let $\mathcal{R}_i$ denote the index set of rows corresponding to $W_i$, and let $r_i = |\mathcal{R}_i|$ denote the number of rows in $W_i$. Note also that $r_i \leq \frac{d}{2^i}$ for $i \in [\log d]$, and $r_{\log d + 1} = 1$. 
\end{definition}
Then we can write $WF_S$ as $WF_S = [(W_1F_S)^{T};\ldots; (W_{\log d +1}F_S)^{T}]^{T}$. Now consider any $i\in [\log d +1]$ and $W_i F_S$. Since $W_i$ is diagonal and $d/2^{i-1}\leq (W_{i})_{j,j}^2 \leq 2d/2^{i-1}$ for all $j\in [r_i]$, applying Lemma \ref{levscore_reweight} with $\beta = 2\alpha = 2d/2^{i}$ we get the following for all $i\in [\log d + 1]$:
\begin{equation*}
	\tau_{j}(W_i F_S) \leq 2 \tau_{j}(F_{S,i}) \quad \forall j\in [r_i]
\end{equation*}
Here, $F_{S,i}\in \mathbb{C}^{r_i\times s}$ is the matrix consisting of all rows of $F_{S}$ in the index set $\mathcal{R}_i$. %$d(1-1/2^{i-1})+1$ to the $d(1-1/2^{i})$ row.
 Note that the column span of $F_{S,i}$ and the first $r_i$ rows of $F_S$ is identical. This is because the $j^{th}$ column of $F_{S,i}$ is %just $e^{2\pi i (d(1-1/2^{i-1})f_j)}$, which is 
 a constant times the $j^{th}$ column of the matrix formed by considering the first $r_i$ rows of $F_S$. Since the first $r_i$ rows of $F_S$ forms a $r_i \times r$ Fourier matrix, their leverage scores are then identical as well. Finally, we appeal to Corollary C.2 of \cite{eldar2020toeplitz}, restated below:
\begin{corollary}[Corollary C.2 of \cite{eldar2020toeplitz}]\label{corr:C2_eldar}
	For any positive integers $d$ and $s \leq d$, there is an explicit set of values $\wt{\tau}_1^{(s)},\dots,\wt{\tau}_d^{(s)} \in (0,1])$ such that, for any Fourier matrix $F_S \in \mathbb{C}^{d \times s}$ with leverage scores $\tau_1,\dots,\tau_d$,
	\begin{align*}
		&\forall j, \wt{\tau}_j^{(s)} \geq \tau_j \\
		& \sum_{j=1}^d \wt{\tau}_j^{(s)} = O(s \log s)
	\end{align*}
\end{corollary}

Thus by Corollary \ref{corr:C2_eldar} (C.2 of \cite{eldar2020toeplitz}), we easily obtain the following claim.
\begin{claim}\label{levscore_upperbound}
For any $i\in [\log (d/r)]$ and any $j\in [r_i]$ define $\wt{\tau}_{j,i}$ as follows.
\begin{equation*}
\wt{\tau}_{j,i} = \min\left(1,\frac{r}{\min(j,d/2^i+1-j)},\frac{O(r^6\log^3 (r+1))}{(d/2^i)}\right)
\end{equation*}
For any $\log(d/r)<i\leq \log(d)$ and $j\in [r_i]$ let $\wt{\tau}_{j,i}=1$. Then we have the following.
\begin{enumerate}
	\item $\tau_j(W_iF_S) \leq \wt{\tau}_{j,i}$ for all $i\in [\log d]$ and $j\in [r_i]$.
	\item $\sum_{j=1}^{d/2^i} \wt{\tau}_{j} \leq O(r\log r)$ for all $i\in [\log d]$.
\end{enumerate}
\end{claim}
Now we can easily finish the proof of Lemma \ref{leveragescorebound}.
\begin{proof}[Proof of Lemma \ref{leveragescorebound}]
Define $\wt{\tau}_j$ values for $j\in [d]$ as follows.

\begin{equation}
	\wt{\tau}_{j} = \wt{\tau}_{i,j'}
\end{equation}
where $i,j'$ are chosen such that $d(1-1/2^{i-1})+1 \leq j\leq d(1-1/2^{i})$ and $j = d(1-1/2^{i-1})+1 + j'$, and $\wt{\tau}_{i,j}$ are obtained from Claim \ref{levscore_upperbound}. Finally, using Lemma \ref{levscore_submatrix} we can easily conclude that these upper bounds also serve as upper bounds on the leverage scores of $WF_S$, and by \cref{lemma:lev_score_col_span}, upper bounds on the leverage scores of $WF_SR_S$ as well. This completes the proof of Lemma \ref{leveragescorebound}.
\end{proof}



==> existence.tex <==
\section{Existence of a near optimal low-rank approximation which itself is Toeplitz.}
\label{sec:existence_main}

The goal of this section is to prove Theorems \ref{spectralexistence} and \ref{frobeniusexistence}. 
\begin{comment}
	content...

%\hltodo{Update hyperlinks to informal versions at start of paper.}
Recall that we are given PSD Toeplitz matrix $T$ and $T=F_SDF_S^{*}$, where $F_S$ is a symmetric Fourier matrix (recall Definition \ref{def:symmetric_fourier_matrix}), with frequencies $S\subset [0,1/2]$ and  $D= diag(\{a_f\}_{f\in S})$ in its Vandermonde decomposition. We briefly discuss how this section is organized. In subsection \ref{case1}, we consider the case when all the frequencies in $S$ are very close to each other; this is the \emph{clustered} case.
Then in subsection \ref{case2}, we tackle the general case when the frequencies in $S$ are not necessarily clustered. We partition the frequency domain into buckets, where the weight of each bucket is the sum of the weights of all frequencies in $S$ landing in that bucket. The formal definition of buckets is as follows.
\begin{definition}\label{bucketing} %\Cam{$S$ and $a_f$  in this definition have no context. So you need to say that like... Given a toeplitz matrix with vandermonde decomposition $F_S D F_S^*$ as in...}
	For any PSD Toeplitz matrix $T=F_SDF_S^{*}$, where $F_S$ is a Fourier matrix with frequencies $S\subset [0,1/2]$,  $D= diag(\{a_f\}_{f\in S})$, and $j$ is a positive integer, we define the $j$-th bucket $B_j$ by 
	$$
	B_j := \left[\frac{j-1}{d},\frac{j}{d}\right)\cap S,
	$$
	and let
	$$
	w(B_j)=\sum_{f\in B_j} a_f,
	$$
	denote the weight of the $j$-th bucket.
\end{definition}
The main claim in this subsection is to show that having heavy buckets implies that $T$ has many large eigenvalues. This claim is shown in two steps. First, we show the claim for Toeplitz matrices that have a well-separated spectrum as defined formally below.
\begin{definition}[$(\lambda,w)$-well separated]\label{wellseparatedcase}
	A PSD Toeplitz matrix $T=F_SDF_S^{*}$ is said to be $(\lambda,w)$-well separated if all non-empty buckets of $T$ have weight exactly $\lambda$, and for any two non-empty buckets, the minimum wrap-around distance between any two frequencies in these two buckets is at least $w$.
\end{definition}
Second, we show how to reduce from proving the claim for general Toeplitz matrices, to proving it for well separated Toeplitz matrices.
In subsection \ref{case3}, we use the same tools to complete the characterization relating buckets and eigenvalues. In particular, we show that if all buckets have weight smaller than $\lambda$, then all eigenvalues of $T$ are smaller than $O(d\lambda\log d)$. 
Finally, in subsection \ref{finalproof}, we show how to use the structural statements proven in subsections \ref{case2} and \ref{case3} to prove Theorems \ref{frobeniusexistence} and \ref{spectralexistence}.
\subsection{Case of clustered frequencies.}\label{case1}
We begin with the case when all the frequencies in $S$ are clustered, as formalized by Definition \ref{clustered_case-mod}. We first state some preliminaries. Define the $t^{th}$ entry of the $k^{th}$ column denoted by $T_k(t)$ for $t\in [0,d-1]$ as follows %\Cam{Should say in words what it is. I.e., that its }
\begin{equation*}
	T_{k}(t) = \sum_{f\in S} a_fe^{2\pi i (f^*+r_f) (t-(k-1))} + \sum_{f\in S} a_fe^{-2\pi i (f^*+r_f) (t-(k-1))} \quad \forall k\in [d].
\end{equation*}
Then the following lemma, which follows trivially from expanding $T$'s Vandermonde decomposition $F_SDF_S^{*}$, says that the $k^{\text{th}}$ column of $T$ is the evaluation of $T_{k}(t)$ at $t=0,\ldots,d-1$.
\begin{lemma}
	For all $(m,k) \in [d]\times [d]$, $T_{m,k} = T_{k}(m-1)$. 
\end{lemma}
\begin{proof}
	Denote by $F_{S, i}$ the $i$-th row of $F_S$. Then
	\begin{multline*}
		T_{m, k} = (F_S D F_S^*)_{m, k} = F_{S, m} D F_{S, k}^* =\\
		\sum_{f\in S} a_f e^{2\pi i (f^*+r_f) m} e^{-2\pi i (f^*+r_f) k} + \sum_{f\in S} a_f e^{-2\pi i (f^*+r_f) m} e^{2\pi i (f^*+r_f) k} = \\
		\sum_{f\in S} a_f e^{2\pi i (f^*+r_f) (m - k)} + 			\sum_{f\in S} a_f e^{-2\pi i (f^*+r_f) (m - k)} = T_k(m - 1).
	\end{multline*}
	This concludes the proof of the lemma.
\end{proof}


Our main result in this section is stated in the following lemma.
\begin{replemma}{lem:clusteredcase}
	There exists a universal constant $C_1>0$ such that, given any symmetric PSD Toeplitz  $T$ that is $(f^*,\Delta)$-clustered for some $f^*\in [0,1/2]$ and $\Delta \leq 1/d$, and  for $0<\varepsilon,\delta,\gamma<1$ satisfying $\gamma\leq \varepsilon/(\tr(T)2^{C_1\log^7 d})$, the following conditions hold.  There exists a symmetric Toeplitz matrix $\wt{T}=F_{\wt{S}}\wt{D}F_{\wt{S}}^{*}$ of rank at most $O(\ell)$ for $\ell=O(\log d + \log(1/\delta))$ such that
	\begin{enumerate}
		\item $\wt{S}=\{f^*+j\gamma\}_{j=1}^{\ell+1}\cup \{f^*-j\gamma\}_{j=1}^{\ell+1}$, and $\wt{D}$ is a diagonal matrix such that for any $f\in \wt{S}$, the weights corresponding to $f$ and $-f$ are identical. 
		\item $\|T-\wt{T}\|_{F} \leq \delta (\sum_{f\in S}a_{f}) +\varepsilon d$.
	\end{enumerate} 
\end{replemma}
\begin{remark}
	The value of the diagonal elements in $\widetilde{D}$ depends on $\varepsilon$, and in particular the value of the diagonal elements would go to infinity as $\varepsilon$ goes to zero. However, we do not state this tradeoff explicitly in the lemma, since we use this lemma later in Section 4 to obtain leverage score upper bounds on Fourier sparse functions (based on the work of \cite{chen2016fourier}). These bounds do not depend on the magnitude of the coefficients in the function; instead, they depend only on its sparsity, as long as the coefficients are finite. Thus $\varepsilon$ can be set to any strictly positive number of one's choice.
\end{remark}

\begin{proof}
	\begin{comment}
		Define
		\begin{equation}\label{eq:t-def}
			T(t) = \sum_{f\in S} a_fe^{2\pi i (f^*+r_f)t } + \sum_{f\in S} a_fe^{-2\pi i (f^*+r_f)t}
		\end{equation} 
		for $t\in [-d,d]$. 
	
	
	%Let $S$ be $(f_*, \Delta)$.
	Define for all $t\in [-d,d]$
	\begin{equation}\label{eq:t-def}
		\begin{split}
			T(t) &= \sum_{f\in S} a_ f e^{2\pi i (f^*+r_f) t} + \sum_{f\in S} a_fe^{-2\pi i (f^*+r_f) t}.
			%&= \sum_{f\in S} a_ f \left(e^{2\pi i (f_*+r_f) t} + e^{-2\pi i (f_*+r_f) t}\right)\\
			%&= \sum_{f\in S} a_ f \cos\left(2\pi  (f_*+r_f) t\right)\\
		\end{split}.
	\end{equation} 
	
	
	Note that $T_{k}(t)$ is just the restriction of $T(t)$ to $t\in [-(k-1),d-k]$ for all $k\in [d]$. Thus we focus on uniformly approximating $T(t)$ over $t\in [-d,d]$, as this will yield uniform approximations for each $T_k(t)$ simultaneously. 
	
	
	The next Lemma shows how to approximate $T(t)$ with a modulated low degree polynomial. The proof of this Lemma is deferred to the end of this subsection.
	\begin{lemma}\label{lowdeg_taylorapprox}
		For polynomials $p_1,p_2$ of degree $\ell=O(\log d +\log(1/\delta))$ defined as \\$p_{1}(t) = \sum_{m=0}^{\ell} \left[\sum_{f\in S} a_f\frac{(2\pi ir_f)^m}{m!}\right]t^m$ and $p_{2}(t) = \sum_{m=0}^{\ell}$ $ \left[\sum_{f\in S} a_f\frac{(-2\pi ir_f)^m}{m!}\right]t^m$, the following equality holds:
		\begin{equation*}
			|T(t) - e^{2\pi i f^* t}p_{1}(t) - e^{-2\pi i f^* t}p_{2}(t) |\leq \delta(\sum_{f\in S} a_f)  \quad \forall t\in [-d,d].
		\end{equation*}
	\end{lemma} 
	
	Observe that we can write the $p_{1}(t)$ and $p_{2}(t)$ obtained from Lemma~\ref{lowdeg_taylorapprox} as $p_1(t) = p_{even}(t)+ ip_{odd}(t)$ and $p_2(t) = p_{even}(t) - ip_{odd}(t)$, where $p_{even}$ and $p_{odd}$ contain the even and odd powered terms in $\sum_{m=0}^{\ell} \left[\sum_{f\in S} a_f\frac{(2\pi ir_f)^m}{m!}\right]t^m$ respectively. Now we can use the following lemma, which is a minor variation of Lemma 8.8 in \cite{chen2016fourier}, to express $p_{even}(t)$ and $p_{odd}(t)$ as $O(\log d+\log(1/\delta))$-Fourier sparse functions. For completeness, we present its proof at the end of this section.
	\begin{lemma}[Lemma 8.8 in \cite{chen2016fourier}]\label{polytofourier}
		Let $p(t)$ be a degree $\ell$ polynomial with coefficients $c_1,\ldots,c_{\ell}$, defined over $t\in [-d,d]$ and containing only even powers of $t$. For every  $\varepsilon\in (0, 1)$ and $\gamma \in (0, 1)$ satisfying
		\begin{equation*}
			\gamma \leq \varepsilon/(d2^{\Theta({\ell}^3\log (\ell))}\underset{1\leq i \leq p}{\max}|c_i|),
		\end{equation*}
		there exists $\wt{p}(t) = \sum_{j=1}^{\ell+1} \alpha_j(e^{2\pi i (j\gamma)t }+e^{-2\pi i (j\gamma)t })$ such that 
		\begin{equation*}
			|p(t) - \wt{p}(t)| \leq \varepsilon \quad \forall t\in [-d,d].
		\end{equation*}
		If $p(t)$ has only odd powers of $t$, then there exists $\wt{p}(t) = -i \sum_{j=1}^{\ell+1} \beta_j(e^{2\pi i (j\gamma)t }-e^{-2\pi i (j\gamma)t })$ that satisfies the above guarantee.
	\end{lemma}
	
	%Let $\epsilon = \delta \sum_{j=1}^d a_j$.
	We apply Lemma~\ref{polytofourier} to approximate $p_{even}(t)$ by $\wt{p}_{even}(t)=\sum_{j=1}^{\ell+1}\alpha_j(e^{2\pi i (j\gamma)t}+e^{-2\pi i (j\gamma)t})$ and $p_{odd}(t)$ by $\wt{p}_{odd}(t)=-i\sum_{j=1}^{\ell+1}\beta_j(e^{2\pi i (j\gamma)t}-e^{-2\pi i (j\gamma)t})$. Note that since $r_f\in [0,1]$ for all $f\in S$, we can trivially upper bound the absolute value of the $j^{th}$ coefficient of $p_{even}$ and $p_{odd}$ by $d\sum_{f\in S}a_f$. Thus we can choose any $\gamma \leq \varepsilon/(d(\sum_{f\in S} a_f)2^{C_1\log^7 d})$ while applying Lemma~\ref{polytofourier}, since $\ell^3 \log (\ell)\leq O(\log^7 d)$. Now define $\wt{T}(t)$ as follows:
	\begin{align*}
		\wt{T}(t) &= e^{2\pi i f^*t}(\wt{p}_{even}(t)+i\wt{p}_{odd}(t)) +  e^{-2\pi i f^*t}(\wt{p}_{even}(t)-i\wt{p}_{odd}(t))\\
		&=\sum_{j=1}^{\ell+1}\alpha_j\left[(e^{2\pi i (f^*+j\gamma)t}+e^{-2\pi i (f^*+j\gamma)t})+(e^{2\pi i (f^*-j\gamma)t}+e^{-2\pi i (f^*-j\gamma)t})\right]\\
		&+\sum_{j=1}^{\ell+1}\beta_j\left[(e^{2\pi i (f^*+j\gamma)t}+e^{-2\pi i (f^*+j\gamma)t})-(e^{2\pi i (f^*-j\gamma)t}+e^{-2\pi i (f^*-j\gamma)t})\right]\\
		&=\sum_{j=1}^{\ell+1}(\alpha_j+\beta_j)\left[(e^{2\pi i (f^*+j\gamma)t}+e^{-2\pi i (f^*+j\gamma)t})\right]+(\alpha_j-\beta_j)\left[(e^{2\pi i (f^*-j\gamma)t}+e^{-2\pi i (f^*-j\gamma)t})\right].
	\end{align*}
	%Thus letting $\wt{p}_k(t)=\sum_{j=1}^{O(\log^2 d)} \alpha_j(e^{2\pi i (j\gamma)(t-(k-1)) }+e^{2\pi i (-j\gamma)(t-(k-1)) })$, that is the restriction of $\wt{p}(t)$ to $t\in [-(k-1),d-k]$, 
	Let $\wt{T}_{k}(t)$ be the restriction of $\wt{T}(t)$ to $t\in [-(k-1),d-k]$. Thus applying the error guarantees of Lemma~\ref{lowdeg_taylorapprox} and \ref{polytofourier} and applying triangle inequality, we get that for all $k\in [d]$
	\begin{equation*}
		|T_k(t) - \wt{T}_k(t)| \leq \delta (\sum_{f\in S} a_f) + \varepsilon \quad \forall t \in [-(k-1),d-k].
	\end{equation*}
	
	Now $\wt{T}_k(t)$ for $k\in\{1,\ldots,d\}$ naturally defines the rank $4(\ell+1)$ symmetric Toeplitz matrix $\wt{T}=F_{\wt{S}}\wt{D}F_{\wt{S}}^{*}$, where $\wt{S}=\{f^*+j\gamma\}_{j=1}^{\ell+1}\cup \{f^*-j\gamma\}_{j=1}^{\ell+1}$ and $\wt{D}=diag(\{\alpha_j+\beta_j\}_{j=1}^{\ell+1}\cup\{\alpha_j-\beta_j\}_{j=1}^{\ell+1})$. The previous equation and this observation immediately that for $\wt{T}$,
	\begin{equation*}
		\|T-\wt{T}\|_F \leq \sqrt{\sum_{(i,j)\in [d]\times [d]} ( \delta (\sum_{f\in S} a_f) + \varepsilon)^2} = \delta d(\sum_{f\in S} a_f) + \varepsilon d.
	\end{equation*}
	We redefine $\delta$ as $\delta/d$. This concludes the proof of statement 2 in Lemma~\ref{lem:clusteredcase}.
	Lemma~\ref{tracetrick} implies that choosing $\gamma \leq \varepsilon/(d(\sum_{f\in S} a_f)2^{C_1\log^7 d}) = \varepsilon/(\tr(T)2^{C_1\log^7 d}) $ suffices for the first claim of the lemma to hold. 
\end{proof}
We now state the proof of Lemma~\ref{lowdeg_taylorapprox}.
\begin{proof}
	First, using a Taylor expansion we can write $T(t)$ as follows
	\begin{align*}
		T(t) &= \sum_{f\in S} a_fe^{2\pi i (f^*+r_f) t} + \sum_{f\in S} a_fe^{-2\pi i (f^*+r_f)t}\\
		& = e^{2\pi i f^* t}\left(\sum_{f\in S} a_f(\sum_{m=0}^{\infty} \frac{(2\pi i r_f t)^m}{m!})\right)+e^{-2\pi i f^* t}\left(\sum_{f\in S} a_f(\sum_{m=0}^{\infty} \frac{(-2\pi i r_f t)^m}{m!})\right)\\
		& = e^{2\pi i f^* t}\sum_{m=0}^{\ell} \left[\sum_{f\in S} a_f\frac{(2\pi ir_f)^m}{m!}\right]t^m+e^{-2\pi i f^* t}\sum_{m=0}^{\ell} \left[\sum_{f\in S} a_f\frac{(-2\pi ir_f)^m}{m!}\right]t^m\\
		&+ e^{2\pi i f^* t}\left(\sum_{f\in S} a_f(\sum_{m=\ell}^{\infty} \frac{(2\pi i r_f t)^m}{m!})\right)+ e^{-2\pi i f^* t}\left(\sum_{f\in S} a_f(\sum_{m=\ell}^{\infty} \frac{(-2\pi i r_f t)^m}{m!} )\right).
	\end{align*}
	Using the fact that $|r_f|\leq \Delta$ and $t\in [-d,d]$, we have that $|2\pi i r_f|< 10 \Delta d$ for all $f\in S$. Also note that for any $m>1, m!\geq (m/2)^{m/2}$. This implies that the following holds for all $r_f$ and $t\in[-d,d]$
	\begin{align*}
		\left|\sum_{m=\ell}^{\infty} \frac{(2\pi i r_f t)^m}{m!}\right|&\leq \sum_{m=\ell}^{\infty} \left|\frac{(2\pi i r_f t)^m}{m!}\right|  \leq \sum_{m=\ell}^{\infty} (10\Delta d)^m/(m/2)^{m/2} \\
		&\leq \sum_{m=\ell}^{\infty} (10\Delta d/\sqrt{m/2})^m \leq \sum_{m=\ell}^{\infty} (10/100 \sqrt{\log d})^{m}\\
		&= \sum_{m=\ell}^{\infty} (0.1)^m \leq (0.1)^{O(\log(1/\delta))}/0.9 \leq \delta/2.
	\end{align*}
	Thus letting $p_{1}(t) = \sum_{m=0}^{\ell} \left[\sum_{f\in S} a_f\frac{(2\pi ir_f)^m}{m!}\right]t^m$ and $p_{2}(t) = \sum_{m=0}^{\ell}$ $ \left[\sum_{f\in S} a_j\frac{(-2\pi ir_f)^m}{m!}\right]t^m$,  we get that
	\begin{align*}
		|T(t) - e^{2\pi i f^*t}p_{1}(t) - e^{-2\pi i f^*t}p_{2}(t)| &\leq \sum_{f\in S} a_{j}\left(\left|\sum_{m=\ell}^{\infty} \frac{(2\pi i r_f t)^m}{m!} \right|+ \left|\sum_{m=\ell}^{\infty} \frac{(-2\pi i r_f t)^m}{m!} \right|\right)\\&\leq \delta(\sum_{f\in S} a_j),
	\end{align*}
	where in the second inequality we used that all the $a_j$'s are non-negative.
\end{proof}
We finish this subsection with the proof of Lemma~\ref{polytofourier}.\begin{proof}
	The proof of this is almost identical to the proof of Lemma 8.8 in \cite{chen2016fourier}. We first consider the case when the degree $\ell$ polynomial $p(t)$ has only even powers of $t$. Let $p(t) = \sum_{j=0}^{\ell/2} c_{2j}t^{2j}$. First, note we can write $\wt{p}(t)$ as 
	\begin{align*}
		\wt{p}(t) &= \sum_{j=1}^{\ell+1} \alpha_{j}( e^{2\pi i (\gamma j)t}+e^{-2\pi i (\gamma j)t})\\
		&= \sum_{j=1}^{\ell+1} 2\alpha_{j} (\sum_{k=0:k \text{ even}}^{\infty} \frac{(2\pi i \gamma j t)^k}{k!})\\
		&= \sum_{k=0:k\text{ even}}^{\infty} 2\frac{(2\pi i \gamma  t)^k}{j!}\sum_{j=1}^{\ell+1} \alpha_j j^k\\
		&= \sum_{k=0:k\text{ even}}^{\ell} 2\frac{(2\pi i \gamma  t)^k}{j!}\sum_{j=1}^{\ell+1} \alpha_j j^k+\sum_{k=\ell+1:k\text{ even}}^{\infty} 2\frac{(2\pi i \gamma  t)^k}{j!}\sum_{j=1}^{\ell+1} \alpha_j j^k\\
		& = p(t)+ (\sum_{k=0:k\text{ even}}^{\ell} 2\frac{(2\pi i \gamma  t)^k}{j!}\sum_{j=1}^{\ell+1} \alpha_j j^k-p(t))+\sum_{k=\ell+1:k\text{ even}}^{\infty} 2\frac{(2\pi i \gamma  t)^k}{j!}\sum_{j=1}^{\ell+1} \alpha_j j^k.
	\end{align*}
	We will show that there exists some $\gamma$ and $\alpha_1,\ldots,\alpha_{\ell+1}$ such that $\sum_{k=0:k\text{ even}}^{\ell} 2\frac{(2\pi i \gamma  t)^k}{j!}\sum_{j=1}^{\ell+1} \alpha_j j^k-p(t)$ is identically zero. The $\ell+1 \times \ell+1$ Vandermonde matrix $A'$ is the same as in the proof of Lemma 8.8 in \cite{chen2016fourier}; however, the $\ell+1$ dimensional vector $c'$ is slightly different: $c'_{j} =  c_j j!/(2\pi i \gamma)^j$ for $j$ even and $c'_j=0$ for $j$ odd. The rest of the argument is identical to the proof of Lemma 8.8 in \cite{chen2016fourier}.
	Now, the argument to show that the absolute value of $C_2 = \sum_{k=\ell+1:k\text{ even}}^{\infty} 2\frac{(2\pi i \gamma  t)^k}{j!}\sum_{j=1}^{\ell+1} \alpha_j j^k$ is less than $\epsilon$ for all $|t|\leq d$ (for the choice of $\gamma$ and $\alpha_1,\ldots,\alpha_{\ell+1}$ shown to exist previously) is also nearly identical to the proof of Lemma 8.8 in \cite{chen2016fourier}. The only difference is that, while upper bounding the value of $|C_2|$, we replace $t^j$ with $|t|^j$ for all $j\in [\ell+1,\infty]$.
	
	The proof for the case when $p(t)$ has only odd powered terms is identical to the proof discussed above, with the exception that the goal is to show the existence of  $\wt{p}(t) = -i\sum_{j=1}^{\ell+1} \beta_j(e^{2\pi i(\gamma j)t}-e^{-2\pi i(\gamma j)t})$ satisfying the claim of the theorem. 
\end{proof}

\subsection{Many heavy buckets implies many large eigenvalues.}\label{case2}


In this subsection, we present our first structural result relating the Vandermonde decomposition $T = F_S D F_{S}^{*}$ to the eigenvalue decomposition of $T=U\Sigma U^{T}$. We first bucket the frequencies in the Vandermonde decomposition, as described in Definition \ref{bucketing}. 
\begin{comment}
	\begin{Definition}\label{bucketing}
		Define the $j^{th}$ bucket of $T$ as $B(j) = \{f \in S | f \in [(j-1)/d,j/d]\}$ for all $j\in \mathbb{N}$. Also, let $w(B(j))=\underset{f\in B(j)}{\sum}a_f$ be the weight of the $j^{th}$ bucket. 
	\end{Definition}



Equipped with this definition, we now state the main result of this section.
\begin{replemma}{heavybucketlemma}
	For every $\lambda,k>0$, if $T$ has at least $k$ buckets with weight at least $\lambda$, then $T$ has at least $k/\log^3 d$ eigenvalues that have value $\Omega(d\lambda/\log d)$. 
\end{replemma}
Before we prove Lemma~\ref{heavybucketlemma}, we state the following helper lemmas. We will then present the proof of Lemma~\ref{heavybucketlemma} using these helper lemmas, and finally end this subsection with their proofs. % of these helper lemmas.
\begin{lemma}\label{innerproduct}
	For any two frequencies $f,g\in [-1/2,1/2]$, 
	\begin{align*}
		|v(f)^{*}v(g)|\leq O(1/|f-g|_{\circ}),
	\end{align*}
	where $v(f),v(g)$ are the corresponding frequency vectors (recall Definition \ref{freqvector} of frequency vectors) and $|f-g|_{\circ}$ is the wrap-around distance between $f$ and $g$.  
\end{lemma}

The next lemma essentially is a strengthening of Gershgorin's circle theorem for block matrices. 
\begin{lemma}[Section 1.13 in \cite{tretter2008spectral}, or Corollary 3.2 in \cite{echeverria2018block}]
	\label{blockgershgorin}
	Let $A = (A_{ij})\in \mathbb{C}^{dn\times dn}$ be a Hermitian matrix composed of blocks $A_{ij}\in \mathbb{C}^{d\times d}$. Then each $A_{ii}$ is Hermitian, and the following is true:
	\begin{equation*}
		\|A\|_2\leq \max_{i\in [n]}(\|A_{ii}\|_2+\sum_{\substack{j\in [n]\\ j\neq i}}\|A_{ij}\|_2).
	\end{equation*}
\end{lemma}
The final helper lemma will help us upper bound the norms of the off-diagonal blocks when applying Lemma~\ref{blockgershgorin}. 
\begin{lemma}\label{frobnormupperbound}
	For any $\lambda\geq 0$, $\sigma_1,\sigma_2\in \{+,-\}$, sets of frequencies $S_1,S_2\subseteq [0,1/2]$ and corresponding diagonal weight matrices $D_1,D_2$ both of whose traces are at most $\lambda$, $A = D_1^{1/2}F_{\sigma_1S_1}^{*}F_{\sigma_2S_2}D_{2}^{1/2}$ satisfies $\|A\|_F \leq O(\lambda/d(\sigma_1S_1,\sigma_2S_2))$. Here recall that for any set of frequencies $S\subset [0,1/2]$, $+S$ and $-S$ contain the frequencies in $S$ and their negations, respectively, and $d(A,B)$ for any sets $A,B\subseteq[-1/2,1/2]$ is the minimum wraparound distance between any two frequencies in $A,B$.
\end{lemma}
\begin{comment}
	\begin{lemma}\label{frobnormupperbound}
		For $m\neq n$ let $A_{m,n} = D_{m}^{1/2}F_{B_m}^{*}F_{B_n}D_{n}^{1/2}$ where $F_{B_m},D_m$ are the Fourier and diagonal weight matrices corresponding the frequencies in the $m^{th}$ bucket respectively. Let $\lambda\geq 0$ be such that $w(B_m)$ and $w(B_n)$ are at most $\lambda$ and let $d_{m,n}$ be the minimum wrap around distance between any frequency in the $m^{th}$ and $n^{th}$ bucket. Then $\|A_{m,n}\|_F \leq O(\lambda/d_{m,n})$. 
	\end{lemma}


We first consider a Toeplitz matrix with a well separated spectrum (as per Definition \ref{wellseparatedcase}) and prove Lemma~\ref{heavybucketlemma} for this case. Then, we reduce the general case to the well separated case, which proves Lemma~\ref{heavybucketlemma} in full generality. 

It can be seen from the following lemma that, essentially, we can reduce from a general Toeplitz matrix to the well-separated case.
\begin{lemma}\label{wellseparatedreduction}
	For any $w,\lambda,k>0$ and a PSD Toeplitz matrix $T$ having at least $k$ buckets with weight at least $\lambda$, there exists a $(\lambda,w)$-well separated PSD Toeplitz matrix $T_{separated}$ having at least $k/dw$ non-empty buckets satisfying $T_{separated}\preceq T$.
\end{lemma}

The following lemma essentially proves Lemma~\ref{heavybucketlemma} for the special case of well-separated matrices. 
\begin{lemma}\label{heavybucketspecialcase}
	For every $\lambda,w,k>0$ and a $(\lambda,w)$-well separated $T$ having at least $k$ non-empty buckets, $T$ has at least $k$ eigenvalues that have value at least $\Omega(\lambda(d/\log d - \log d/w))$.
\end{lemma}

Equipped with these helper lemmas, we are ready to present the proof of Lemma~\ref{heavybucketlemma}.
\begin{proof}
	Refer to the $k$ buckets with weight at least $\lambda$ as \emph{heavy buckets}. Without loss of generality, we can assume that each bucket has weight exactly $\lambda$. This can be seen by the following argument. We reduce the weight of each heavy bucket if needed to ensure that each heavy bucket has weight exactly $\lambda$. This change will only make $T$ PSD smaller, and thus it suffices to lower bound eigenvalues of $T$ after this operation. We can easily obtain a $(\lambda,w)$-well separated Toeplitz matrix from $T$ as per Claim \ref{wellseparatedreduction}.
	
	Consider the matrix $T_{separated}$ guaranteed to exist by Lemma \ref{wellseparatedreduction}. Thus, invoking Lemma~\ref{heavybucketspecialcase} for $T_{separated}$ with parameters $\lambda,k/dw,w$ for $w=\log^3d/d$, we get that $T_{separated}$ has at least $k/\log^3d$ eigenvalues of value $\Omega(d\lambda (1/\log d - 1/\log^2d)) = \Omega(d\lambda/\log d)$. Since $T_{separated} \preceq T$, $T$ also has at least $k/\log^3d$ eigenvalues of value $\Omega(d\lambda (1/\log d - 1/\log^2d)) = \Omega(d\lambda/\log d)$. This finishes the proof of Lemma~\ref{heavybucketlemma}.
\end{proof}
Now we present the proof of the well separated case (Lemma~\ref{heavybucketspecialcase}).
\begin{proof}
	\begin{comment}
		To show how the second property can be achieved, we need to define a \emph{splitting} operation, which essentially replaces a frequency in any bucket with $t$ copies and its weight equally distributed among its copies for any desired $t$. More formally, for any frequency $f_i$ and its corresponding weight $a_i$ in some bucket $B_j$ and any integer $t>0$ we define splitting $f_i$ $t$ times as updating $B_j$ as $B_j = (B_j\setminus\{f_i\})\cup\{f_{i_1},f_{i_2},\ldots,f_{i_t}\}$ where each $f_{i_{k}}=f_i$ and $a_{i_k}=a_{i}/t$. Note that splitting any frequency $t$ times does not change the Toeplitz matrix $T$ for any $t$. We can now ensure that each bucket of $T$ has the same number of frequencies by splitting frequencies in each bucket enough number of times, without changing $T$. \kstodo{Cam and Michael - do you think this is formal enough ?} \xxx[MK]{not really. I would separate this out into another lemma. Also weird that the splitting operation introduces multisets, need to make this explicit} 
		
		
		
		Denote the $k$ heavy buckets by $B(j_1),B(j_2)\ldots,B(j_k)$. Recall that this notation implies any such heavy bucket $B(j_m)$ contains all frequencies of $S$ in the interval $[(j_{m}-1)\log d/d,j_{m}\log d/d]$. Note that there could be two heavy buckets adjacent to each other, that is the minimum wrap around distance between any frequency in the first and any frequency in the second bucket could be arbitrarily small. To ensure a certain minimum distance between any two buckets, which we would need in our analysis, we only retain one out of every $\log^3 d^{th}$ heavy bucket. More formally consider the $k/\log^3 d$ heavy buckets $B(j_1),B(j_{\log^3 d}),B(j_{2\log^3 d})\ldots,B(j_k)$, and refer to them as \textit{remaining} heavy buckets.\xxx[MK]{ambiguous}
		% Thus the following claim easily follows
		%\begin{claim}\label{bucketseparation}
		%	For any two heavy buckets $B_{j_{m}}$ and $B_{j_{n}}, d_{m,n} = \Omega (\min \{|m-n|\log^4 d/d,|1-(m+n)\log^4 d/d|\})$
		%\end{claim}
		
		For every remaining heavy bucket $B(j_m)$ let $F_{B(j_m)}\in \mathbb{C}^{d\times 2|B(j_m)|}$ denote the Fourier matrix corresponding to frequencies in $B(j_m)$ and let $D_m\in \mathbb{R}^{2|B(j_m)|\times 2|B(j_m)|}$ denote the diagonal weight matrix corresponding to weights of frequencies in $B(j_m)$. Let $\wt{F} =[F_{B(j_1)};F_{B(j_{\log^3 d})};\ldots;F_{B(j_{k})}]$ and $D$ be the diagonal matrix of the corresponding weights of all the remaining heavy buckets. Since $\wt{F}D\wt{F}^{*}\preceq T$, it suffices to show that $\wt{F}D\wt{F}^{*}$ has $k/\log^3 d$ eigenvalues that have value $\Omega(d\lambda/\log^2 d)$. 

	Let $T=F_S D F_S^{*}$ denote the Vandermonde decomposition of $T$.
	%and
	%denote the $k$ non-zero buckets of $T$ by $B(j_1),B(j_2)\ldots,B(j_k)$ with corresponding diagonal weight matrices $D_1,\ldots D_k$.
	Observe that $F_S D F_S^{*}$ has the same eigenvalues as $D^{1/2}F_S^{*}F_SD^{1/2}$. This is because, for any matrix $A$, $A^* A$ and $AA^{*}$ have the same eigenvalues; apply this fact to $A=F_SD^{1/2}$. It can be easily seen that $D^{1/2}F_S^{*}F_SD^{1/2}$ is a block matrix, where each of its blocks is of the form $D_{m}^{1/2}F_{B_m}^{*}F_{B_n}D_{n}^{1/2}$ for some $m,n$, and $D_m$ is the diagonal matrix containing weights of the frequencies in bucket $B_m$ for every $m$. We can pad each block with enough zero rows and columns to ensure that the dimensions of each block are the same, without affecting its spectral norm. Thus we can express $D^{1/2}F_S^{*}F_SD^{1/2} = A+E$, where $A$ contains the diagonal blocks with zero matrices on the off diagonal blocks, and $E$ contains the off-diagonal blocks with zero matrices on the diagonal blocks. Our high level strategy is to prove the theorem statement for $A$ by using the fact that it is block diagonal. Then, we show that $E$ has small spectral norm, so the eigenvalues of $A+E$ are close to the eigenvalues of $A$.\\
	\\
	\textbf{Lower bounding largest eigenvalue of diagonal blocks.} $A$ is block diagonal with at least $k$ blocks. Consider any of its blocks $D_{m}^{1/2}F_{B_m}^{*}F_{B_m}D_{m}^{1/2}$ for some $m$. We know that $F_{B_m}D_{m}F_{B_m}^{*}$ is $((m-1/2)/d,1/d)$-clustered. Thus by Lemma~\ref{lem:clusteredcase} with $\delta=1/2d^{11}$ and $\varepsilon = \lambda/2d^{12}$,$F_{B_m}D_{m}F_{B_m}^{*}$ is  $\delta(\sum_{f\in B_m}a_{f}) + \varepsilon d = \lambda/d^{11}$ close to a symmetric Toeplitz matrix $\wt{T}$ with rank at most $C\log d$ in the Frobenius norm for some universal constant $C>0$. Thus by Weyl's inequality (Theorem \ref{weylineq}), we get the following for any $k>C\log d$
	
	\begin{align*}
		\lambda_{k}(F_{B_m}D_{m}F_{B_m}^{*})&\leq \lambda_{k}(\wt{T})+\|F_{B_m}D_{m}F_{B_m}^{*}-\wt{T}\|_{2}\\
		&\leq 0+ \|F_{B_m}D_{m}F_{B_m}^{*}-\wt{T}\|_{F}\\
		&\leq \lambda/d^{11}.
	\end{align*}
	Thus we get the following bound on the trace of $F_{B_m}D_{m}F_{B_m}^{*}$
	\begin{equation*}
		\tr(F_{B_m}D_{m}F_{B_m}^{*}) \leq C\log d\lambda_{1}(F_{B_m}D_{m}F_{B_m}^{*})+\lambda/d^{10}.    
	\end{equation*}
	This implies that
	\begin{align*}
		\lambda_{max}(D_{m}^{1/2}F_{B_m}^{*}F_{B_m}D_{m}^{1/2})&=\lambda_{1}(F_{B_m}D_{m}F_{B_m}^{*})\\
		&\geq \tr(F_{B_m}D_{m}F_{B_m}^{*})/(C\log d) - \lambda/(Cd^{10}\log d)\\
		&=d\lambda/(C\log d) - \lambda/(Cd^{10}\log d) = \Omega(d\lambda/\log d).
	\end{align*}
	Since $A$ is a block diagonal matrix with at least $k$ blocks, and each block has largest eigenvalue $\Omega(d\lambda/\log d)$, we get that $A$ has at least $k$ eigenvalues which are at least $\Omega(d\lambda/\log d)$ in value.\\
	\\
	\textbf{Upper bounding the contribution of off-diagonal blocks.} In the rest of the proof, we bound the spectral norm of $E$. We do this by applying Lemma~\ref{blockgershgorin} to $E$ where its diagonal blocks are $0$ and any off diagonal block is of the form $D_{m}^{1/2}F_{B_m}^{*}F_{B_n}D_{n}^{1/2}$ for some buckets $B_m,B_n$ satisfying $m\neq n$. 
	Consider an arbitrary but fixed bucket index $m$. In order to apply Lemma~\ref{blockgershgorin}, we need to upper bound $\sum_{n:n\neq m} \|D_{m}^{1/2}F_{B_m}^{*}F_{B_n}D_{n}^{1/2}\|_2\leq \sum_{n:n\neq m} \|D_{m}^{1/2}F_{B_m}^{*}F_{B_n}D_{n}^{1/2}\|_F$. We recall that for any $n$, $F_{B_n}= [F_{+B_n};F_{-B_n}]$ as per the notation in Definition \ref{def:symmetric_fourier_matrix}. We apply Lemma~\ref{frobnormupperbound} to bound $\|D_{m}^{1/2}F_{B_m}^{*}F_{B_n}D_{n}^{1/2}\|_F$ as follows
	\begin{align*}
		\|D_{m}^{1/2}F_{B_m}^{*}F_{B_n}D_{n}^{1/2}\|_F &\leq \|D_{m}^{1/2}F_{+B_m}^{*}F_{+B_n}D_{n}^{1/2}\|_F+\|D_{m}^{1/2}F_{+B_m}^{*}F_{-B_n}D_{n}^{1/2}\|_F\\&+\|D_{m}^{1/2}F_{-B_m}^{*}F_{+B_n}D_{n}^{1/2}\|_F+\|D_{m}^{1/2}F_{-B_m}^{*}F_{-B_n}D_{n}^{1/2}\|_F\\
		&\leq O(\lambda(1/d(+B_m,+B_n)+1/d(+B_m,-B_n)+\\
		&1/d(-B_m,+B_n)+1/d(-B_m,-B_n))).
	\end{align*}
	Thus, we need to upper bound the following
	\begin{align*}
		\sum_{n:n\neq m}O(\lambda(1/d(+B_m,+B_n)+1/d(+B_m,-B_n)+
		1/d(-B_m,+B_n)+1/d(-B_m,-B_n))).
	\end{align*}
	It is easy to see that the maximum value the above expression can take will correspond to the case when, informally, there are as many buckets as possible in $S$,  while still ensuring that any two buckets have separation at least $w$. More formally, this corresponds to the case when for every $n\in [m-d/(2w),m+d/(2w)]$, there is a bucket at distance $d_{m,n} = \Theta(|m-n|w)$ from $B_m$. Thus, the above expression is bounded by
	\begin{align*}
		\sum_{n=m+1}^{m+d/(2w)}O(\lambda/((n-m)w))  &+\sum_{n=m-d/(2w)}^{m-1}O(\lambda/((m-n)w)) \\
		& \leq 2\sum_{l=1}^d O(\lambda/(lw))\\&= O(\lambda/w)\sum_{l=1}^{d}1/l\\
		&= O(\lambda \log d/w).
	\end{align*}
	Since any diagonal block has spectral norm $0$ and the previous bound holds for all $m$, Lemma~\ref{blockgershgorin} applied to $E$ implies that $\|E\|_2\leq O(\lambda \log d/w)$.
	Now, applying Weyl's inequality for all $i$ such that $\lambda_i(A)=\Omega( d\lambda/\log d)$, we have
	\begin{equation*}
		\lambda_i(A+E)\geq\lambda_{i}(A) - \|E\|_2 = \Omega(d\lambda/\log d) - \|E\|_2\geq \Omega(\lambda(d/\log d-\log d/w)).    
	\end{equation*}
	Since there are at least $k$ such indices $i$, this completes the proof of the Lemma.
\end{proof}
We now present the proof of Lemma~\ref{innerproduct}.
\begin{proof}
	Denote by $\delta = |f - g|_{\circ}$ the wrap around distance between $f$ and $g$. 
	Since $|v_{f}^{*}v_{g}| = |v_{f}^{*}v_{g}|$, we have the following. %maybe add more explanation here ?
	
	\[
	|v(g)^{*}v(f)| = \left|\sum_{l = 0}^{d - 1} \exp(2 \pi i \delta l)\right| = \left|\frac{\exp(2 \pi i \delta d) - 1}{\exp(2 \pi i \delta) - 1}\right| = \left|\frac{\exp(\pi i \delta d)}{\exp(\pi i \delta)} \cdot \frac{\sin(\pi \delta d)}{\sin(\pi \delta)}\right|.
	\]
	Therefore, it holds that
	\begin{equation*}
		|v(g)^{*}v(f)| = \left| \frac{\sin(\pi \delta d)}{\sin(\pi \delta )} \right| \leq \frac{1}{|\sin(\pi \delta)|} \leq  O\left(\frac{1}{\delta}\right).
	\end{equation*}
	Here, the last inequality follows by the fact that $\sin(\pi x)\geq 2x$ for $x\in [0,1/2]$, and the wrap around distance between any two frequencies lies between $0$ and $1/2$.
\end{proof}
Now, we present the proof of Lemma~\ref{frobnormupperbound}.

\begin{proof}
	We have the following for all $i,j$:
	\begin{equation*}
		|(A)_{i,j}| = \sqrt{(D_1)_i(D_2)_j}|v(f_i)^{*}v(f_j)|\leq O(\sqrt{(D_1)_i(D_2)_j}/|f_i-f_j|)\leq O(\sqrt{(D_1)_i(D_2)_j}/d(\sigma_1S_1,\sigma_2S_2)),
	\end{equation*}
	where $(D_1)_i,(D_2)_j$ and $f_{i},f_{j}$ are the weights and frequencies of the $i^{th}$ frequency in the $\sigma_1S_1$ and $j^{th}$ frequency in the $\sigma_2S_2$ respectively. Also, note that the second to last inequality follows from Lemma~\ref{innerproduct}.
	%Thus $|f_{i,m}-f_{j,m}|=\Theta(d_{i,j})$ as each bucket has width $\log d/d$ and the buckets are at least $\log^4 d/d$ apart.
	This implies
	\begin{align*}
		\|A\|_{F}^2 &\leq O( \sum_{i,j}(D_1)_i(D_2)_j/d(\sigma_1S_1,\sigma_2S_2)^2) \\
		&=O((\sum_{i}(D_1)_i)(\sum_{j}(D_2)_j)/d(\sigma_1S_1,\sigma_2S_2)^2)\\
		&\leq O(\lambda^2/d(\sigma_1S_1,\sigma_2S_2)^2).
	\end{align*}
	Thus $\|A\|_F \leq O( \lambda/d(\sigma_1S_1,\sigma_2S_2))$.  
\end{proof}
We finally end this sub-section with the proof of Claim \ref{wellseparatedreduction}.
\begin{proof}
	Sort the $k$ heavy buckets of $T$ according to their central frequency, and index them by $[k]$. Now consider the Toeplitz matrix $T_{separated}$, obtained by taking the buckets indexed by the residue class $1 \mod dw$ out of the $k$ heavy buckets of $T$. There are at least $k/dw$ such buckets, and the pairwise separation between any two such buckets is at least $w$. This implies $T_{separated}$ is $(\lambda,w)$-well separated and has $k/dw$ non-empty buckets. Moreover, since $T_{separated}$ is obtained by taking a subset of the non-empty buckets of $T$, this implies that $T_{separated}\preceq T$.
\end{proof}
\subsection{All buckets being light implies all eigenvalues are small.}\label{case3}
In this subsection, we show that if all buckets of $T$ have small weight, then all eigenvalues of $T$ are small. This result, combined with the previous section, will suffice to prove Theorems \ref{spectralexistence} and \ref{frobeniusexistence}. This is formalized in the lemma below.

%\Cam{Flagging number here.}
\begin{replemma}{lightbucketlemma}
	For every $\lambda\geq 0$, if all buckets of $T$ have weight at most $\lambda$, then $\|T\|_2\leq O(d\lambda\log d)$.
\end{replemma}
\begin{proof}
	We need to upper bound $\|F_SDF_S^{*}\|_2=\|D^{1/2}F_S^{*}F_SD^{1/2}\|_2$. Again, $A:=D^{1/2}F_S^{*}F_SD^{1/2}$ is a block matrix, where its blocks are of the form $A_{m,n}:=D_{m}^{1/2}F_{B_m}^{*}F_{B_n}D_{n}^{1/2}$ for some buckets $B_m,B_n$. Here $F_{B_m}$ and $D_{m}$ are the Fourier and diagonal weight matrices, respectively, of the $m^{th}$ bucket. To prove the Lemma, we will apply Lemma~\ref{blockgershgorin} on $A$. To do so, we need to upper bound $\|A_{m,m}\|_2+\sum_{n:n\neq m}\|A_{m,n}\|_2\leq \|A_{m,m}\|_2+\sum_{n:n\neq m}\|A_{m,n}\|_F$ for all $m$. Since $A_{m,m}$ is PSD, we upper bound $\|A_{m,m}\|_2$ as follows
	\begin{equation*}
		\|A_{m,m}\|_2\leq \tr(A_{m,m}) = d\sum_{i} (D_m)_i =dw(B_m)\leq d\lambda.
	\end{equation*}
	We can trivially upper bound $\|A_{m,m+1}\|_F$ by first applying Cauchy-Schwarz to each entry $(A_{m,m+1})_{i,j}$:
	\begin{align*}
		|(A_{m,m+1})_{i,j}| = \sqrt{(D_{m})_i(D_{(m+1)})_j}|v(f_{i})^{*}v(f_{j})|\leq & \sqrt{(D_{m})_i(D_{(m+1)})_j}\|v(f_{i})\|_2\|v(f_{j})\|_2\\ &= \sqrt{(D_{m})_i(D_{(m+1)})_j}d,
	\end{align*}
	where $f_{i},(D_m)_i$ are the $i^{th}$ frequency and its corresponding weight in the $m^{th}$ bucket respectively.
	Then we use the previous bound to get that the following holds for any $m$:
	\begin{equation*}
		\|A_{m,m+1}\|_F \leq \sqrt{(\sum_{i}(D_{m})_i)(\sum_{j}(D_{m})_j)d^2}=d\lambda.
	\end{equation*}
	The same bound holds for $\|A_{m,m-1}\|_F$. Thus we obtain the bound
	\begin{equation*}
		\|A_{m,m}\|_2+\sum_{n:n\neq m}\|A_{m,n}\|_F \leq 3d\lambda + \sum_{n:n\notin \{m-1,m,m+1\}} \|A_{m,n}\|_F.
	\end{equation*}
	Since $d(+B_m,+B_{m+1})$ and $d(+B_m,+B_{m-1})$ could be arbitrarily close to $0$ (adjacent buckets could have frequencies very close to each other), the bound $\|A_{m,m+1}\|_F\leq d\lambda$ is tight. For the remaining $n\notin \{m,m-1,m+1\}$, we use Lemma~\ref{frobnormupperbound} to bound $\|A_{m,n}\|_F$ as follows:
	\begin{align*}
		\|A_{m,n}\|_F&\leq O(\lambda(1/d(+B_m,+B_n)+1/d(+B_m,-B_n)+\\
		&1/d(-B_m,+B_n)+1/d(-B_m,-B_n))).
	\end{align*}
	Similar to the proof in the previous subsection, it is easy to see that the maximum value \\$\sum_{n:n\notin \{m-1,m,m+1\}} \|A_{m,n}\|_F$ can take will correspond to the case when all buckets in $[0,1/2]$ are non-empty. More formally, for every $n\in [m-d/2,m+d/2]\setminus \{m-1,m,m+1\}$, there is a bucket at distance $ \Theta(|m-n|/d)$ from bucket $B_m$. Thus we get that the above is bounded by
	\begin{align*}
		\sum_{n=m+2}^{m+d/2}O(\lambda/((n-m)/d))  +&\sum_{n=m-d/2}^{m-2}O(\lambda/((m-n)/d)) \\
		& \leq 2\sum_{l=1}^d O(\lambda/(l/d))\\&= O(d\lambda)\sum_{l=1}^{d}1/l\\
		&= O(d\lambda\log d).
	\end{align*}
	Thus applying Lemma~\ref{blockgershgorin} to $A$, we get that $\|T\|_2 = \|A\|_2 \leq 3d\lambda+ O(d \lambda\log d) = O(d\lambda\log d)$. This completes the proof of Lemma~\ref{lightbucketlemma}.
\end{proof}
\end{comment}
\subsection{Existence of Toeplitz low-rank approximation in the spectral and Frobenius norm.}\label{finalproof}
In this section, we state the main result of \cite{kapralov2022toeplitz} that shows the existence of a near optimal low-rank approximation in the both the spectral and Frobenius norm, which itself is Toeplitz. The first claim is formalized in the following theorem.
\begin{theorem}\label{spectralexistence}
	For any PSD Toeplitz $T\in \mathbb{R}^{d\times d}$,  $0<\delta<1$ and any integer $k\leq d$,  there exists a symmetric Toeplitz matrix $\wt{T}$ of rank $\wt{O}(k\log(1/\delta))$ such that the following holds
	\begin{equation*}
		\|T-\wt{T}\|_2 \leq \wt{O}(1) \|T-T_k\|_2 + \delta\|T\|_F.
	\end{equation*}
	where $T_k=\underset{B:rank(B)\leq k}{\|T-B\|_2}$ is the best rank-$k$ approximation to $T$ in the spectral norm.
\end{theorem}

Next, we state the our main result on the existence of a near optimal Toeplitz low-rank approximation in the Frobenius norm.
\begin{theorem}\label{frobeniusexistence}
	Given any PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$, $0<\eps,\delta<1$ and an integer $k\leq d$, let $r_1=O(k\log^8d/\eps)$ and $r_2 = O(\log d +\log(1/\delta))$. Then there exists a symmetric Toeplitz matrix $\wt{T} = F_{\wt{S}}\wt{D}F_{\wt{S}}^{*}$ of rank $r=2r_1r_2=\wt{O}((k/\eps)\log(1/\delta))$ such that,
	\begin{enumerate}
		\item $\|T-\wt{T}\|_F \leq (1+\eps)\|T-T_k\|_F + \delta\|T\|_F$, where $T_k = \underset{B:rank(B)\leq k}{\|T-B\|_F}$ is the best rank-$k$ approximation to $T$ in the Frobenius norm. Also, $ \wt T\succeq (-\delta \|T\|_F) I_{d} $.
		\item \label{thm:existence_freq_grid}$F_{\wt{S}},\wt{D}$ are Fourier and diagonal matrices respectively. The set of frequencies $\wt{S}$ can be partitioned into $r_1$ sets $\wt{S}_{1},\ldots, \wt{S}_{r_1}$ where each $\wt{S}_i$ is as follows:
		\begin{equation*}
			\wt{S}_i = \underset{1\leq j\leq r_2}{\bigcup}\{f_i+\gamma j,f_i-\gamma j\}.
		\end{equation*}
		\item  $f_i\in N$  for all $i\in [r_1]$, where $N:=\{1/2d,3/2d,\ldots, 1-1/2d\}$. Furthermore, $\gamma = \delta /(2^{C_2 \log^7d})$, where $C_2>0$ is a fixed constant.
	\end{enumerate}
	%\Cam{Its weird in the theorem to define $r_1$ with big-Oh notation,m but state $r_2$ with a fixed constant $C$. Make consistent.}
\end{theorem}
\begin{comment}
\begin{proof}
	Let $T=F_S D F_S$ be $T$'s Vandermonde decomposition and let $\lambda = \lambda_{Ck\log^5 d/\epsilon}(T)\log d/c'd$, where $c'$ is the same constant as in Lemma~\ref{heavybucketlemma} and $C$ is some large constant. Bucket the frequencies in $S$ as per Definition \ref{bucketing}. Let $T_{heavy}$ be the matrix obtained by considering all buckets of $T$ with weight strictly more than $\lambda$. Then $T-T_{heavy}$ is also a Toeplitz matrix defined by the remaining buckets, all of which have weight at most $\lambda$. Thus by Lemma~\ref{lightbucketlemma}, we have the following
	\begin{equation*}
		\|T-T_{heavy}\|_2\leq  O(\lambda d\log d) = O(\log^2d)\lambda_{Ck\log^5 d/\epsilon}(T).
	\end{equation*}
	Since $T-T_{heavy}$ just corresponds to retaining a subset of the frequencies in $S$ and their corresponding weights, it is a PSD change. More formally, $0\preceq T-T_{heavy}\preceq T$. Thus by Weyl's inequality, this implies that $\lambda_i(T-T_{heavy})\leq \lambda_{i}(T)$ for all $i\in [d]$. Thus we have that
	\begin{align*}
		\|T-T_{heavy}\|_F^2 &= \sum_{i=1}^{d} \lambda_{i}^2(T-T_{heavy}) = \sum_{i=1}^{k+1} \lambda_{i}^2(T-T_{heavy}) + \sum_{i=k+2}^{d} \lambda_{i}^2(T-T_{heavy})\\
		&\leq (k+1)\lambda_{1}^2(T-T_{heavy})+ \sum_{i=k+2}^{d} \lambda_{i}^2(T-T_{heavy})\\
		&\leq (k+1)\lambda_{1}^2(T-T_{heavy})+ \sum_{i=k+2}^{d} \lambda_{i}^2(T)    .
		%&\leq \wt{O}(1)(k\lambda_{k+1}^2(T)) + \sum_{i=k+2}^{d} \lambda_{i}^2(T)
	\end{align*}
	Here, we used the fact that $\lambda_i(T-T_{heavy})\leq \lambda_1(T-T_{heavy})$ for all $1\leq i\leq k+1$ and $\lambda_i(T-T_{heavy})\leq \lambda_{i}(T)$ for $i> k+1$. %\hltodo{This isn't clean: define it the right way from the start.} 
	Now, using that $\lambda_1(T-T_{heavy})\leq O(\log^2 d)\lambda_{Ck\log^5 d/\epsilon}(T)$, we get the following:
	\begin{align*}
		\|T-T_{heavy}\|_F^2 &\leq (k+1)\lambda_{1}^2(T-T_{heavy})+ \sum_{i=k+2}^{d} \lambda_{i}^2(T)\\
		&\leq O(k\log^4d)\lambda_{Ck\log^5d/\eps}^2(T) + \sum_{i=k+2}^{d} \lambda_{i}^2(T)\\
		&= \eps O(k\log^4d/\eps)\lambda_{Ck\log^5d/\eps}^2(T) + \sum_{i=k+2}^{d} \lambda_{i}^2(T)\\
		&\leq \eps\sum_{i=k+1}^{O(k\log^4d/\eps)}\lambda_{i}^2(T) + \sum_{i=k+2}^{d} \lambda_{i}^2(T)\\
		&\leq \eps\sum_{i=k+1}^{d}\lambda_{i}^2(T) + \sum_{i=k+1}^{d} \lambda_{i}^2(T)\\
		&= (1+\eps)\|T-T_{k}\|_F^2.
	\end{align*}
	Therefore, we have that $\|T-T_{heavy}\|_F\leq (1+\eps)\|T-T_{k}\|_F$, where $T_{heavy}$ contains all buckets with weight more than $\lambda_{Ck\log^5 d/\eps}\log d/c'd$. There are at most $r_1=O(k\log^8 d/\eps)$ such buckets by Lemma~\ref{heavybucketlemma}.
	Let $F_{S_1},\ldots, F_{S_{r_1}}$ and $D_1,D_2,\ldots, D_{r_1}$ to be the Fourier and diagonal weight matrices corresponding to these $r_1$ heavy buckets defining $T_{heavy}$. We can then write $T_{heavy}$ as follows
	\begin{equation*}
		T_{heavy} = \sum_{m=1}^{r_1} F_{S_m}D_{m}F_{S_m}^{*}.
	\end{equation*}
	
	Since each $ F_{S_m}D_{m}F_{S_m}^{*}$ is $(f,1/d)$-clustered for some $f\in N$, we use Theorem \ref{lem:clusteredcase} to approximate each $ F_{S_m}D_{m}F_{S_m}^{*}$ with a rank $O(\log d+\log(1/\delta))$ symmetric Toeplitz matrix $ F_{\wt{S}_m}\wt{D}_{m}F_{\wt{S}_m}^{*}$ that satisfies 
	\begin{equation*}
		\left\|F_{S_m}D_{m}F_{S_m}^{*} - F_{\wt{S}_m}\wt{D}_{m}F_{\wt{S}_m}^{*}\right\|_{F}\leq \delta(\sum_{i} (D_m)_{i}) + \varepsilon d.
	\end{equation*}
	This implies that
	\begin{align*}
		\left\|T-\sum_{m=1}^{r_1} F_{\wt{S}_m}\wt{D}_{m}F_{\wt{S}_m}^{*}\right\|_F &\leq \left\|T-\sum_{m=1}^{r_1} F_{S_m}D_{m}F_{S_m}^{*}\right\|_F + \left\|\sum_{m=1}^{r_1} (F_{S_m}D_{m}F_{S_m}^{*} - F_{\wt{S}_m}\wt{D}_{m}F_{\wt{S}_m}^{*}) \right\|_F\\
		& = \|T-T_{heavy}\|_F + \left\|\sum_{m=1}^{r_1} (F_{S_m}D_{m}F_{S_m}^{*} - F_{\wt{S}_m}\wt{D}_{m}F_{\wt{S}_m}^{*} )\right\|_F\\
		&\leq \|T-T_{heavy}\|_F + \sum_{m=1}^{r_1} \|F_{S_m}D_{m}F_{S_m}^{*} - F_{\wt{S}_m}\wt{D}_{m}F_{\wt{S}_m}^{*}\|_F\\
		& \leq (1+\epsilon) \|T-T_k\|_F + \delta(\sum_{m,i}(D_m)_{i}) +\varepsilon r d \\
		&\leq  (1+\epsilon) \|T-T_k\|_F + \delta(\sum_{i}(D)_{i}) + \varepsilon r d.
	\end{align*}
	Now using Lemma~\ref{tracetrick}, we get the following:
	\begin{equation*}
		\sum_{i}(D)_{i} = \sum_{i=1}^{d}\lambda_i(T)  /d \leq \left(\sqrt{d \sum_{i=1}^d \lambda_{i}(T)^2}\right)/d = \|T\|_F/\sqrt{d}.
	\end{equation*}
	Setting $\varepsilon = \delta\|T\|_F/rd$, we finally have
	\begin{equation*}
		\left\|T-\sum_{m=1}^{r_1} F_{\wt{S}_m}\wt{D}_{m}F_{\wt{S}_m}^{*}\right\|_F 
		\leq (1+\epsilon) \left\|T-T_k\|_2 + \delta \|T\right\|_{F} .
	\end{equation*}
	Defining $\wt{T}$ as $\wt{T} = \sum_{m=1}^{r_1} F_{\wt{S}_m}\wt{D}_{m}F_{\wt{S}_m}^{*}$, which has rank at most $r_1(C(\log d+\log(1/\delta))=\wt{O}((k/\epsilon)\log(1/\delta))$, we get that $\wt{T}$ satisfies the claim and point 1 of Theorem \ref{frobeniusexistence}. Observe that the Toeplitz matrix corresponding to any bucket $F_{S_m}D_mF_{S_m}^{*}$ is $(f,1/d)$-clustered for some $f\in N$. Thus, it follows by guarantee 1 of Lemma~\ref{lem:clusteredcase} that each $\wt{S}_m$ is of the form described in point 2 of Theorem \ref{frobeniusexistence}. Since $T_{1,1}\leq \|T\|_F$, with this value of $\varepsilon$ we can choose any $\gamma\leq \delta T_{1,1}/(\tr(T)rd^2 2^{C_1 \log^7 d})=\delta/(2^{C_2 \log^7 d})$ for a large enough constant $C_2$. (Here, we used the fact that $\tr(T)=dT_{1,1}$.) This completes the proof of Theorem \ref{frobeniusexistence}.
\end{proof}
\end{comment}

==> introOldTechOverview.tex <==
% !TEX root = ./main.tex

%\Cam{Captialization of section titles should be made consistent. One some of them we use caps for all words, on some for just the first word.}

\section{Introduction}

%\Cam{We need more citation in this first paragraph. They can be drawn from prior work}
A Toeplitz matrix $T\in \mathbb{R}^{d\times d}$ is constant along each of its diagonals. I.e., $T_{i,j}=T_{k,l}$ for all $i,j,k,l$ with $i-j=k-l$. These highly structured  matrices arise in many fields, including signal processing, scientific computing, control theory, approximation theory, and machine learning -- see \cite{Bunch:1985ti} for a survey. In particular, Toeplitz matrices often arise as the covariance matrices of stationary signals, when the covariance structure is shift invariant. I.e., when the covariance between measurements only depends on their distance in space or time \cite{Gray:2006ta}. A row-reversed Toeplitz matrix is known as a Hankel matrix. Such matrices also find broad applications \cite{Fazel:2013vw,Munkhammar:2017ud,Ghadiri:2023tv}. %Toeplitz matrices also arise in control theory, approximation theory, the study of orthogonal polynomials and partial differential equations \cite{Bunch:1985ti}.

Given their importance, significant work has studied fast algorithms for basic linear algebraic tasks on Toeplitz matrices. A $d \times d$ Toeplitz matrix can be multiplied by a vector in just  $O(d\log d)$ time using the fast Fourier transform. Toeplitz linear systems can be solved in $O(d^2)$ time exactly using Levinson recursion \cite{Golub:2013wp}, and to high-precision in $O(d\cdot \polylog d)$ time using randomization  \cite{XiXiaCauley:2014,XiaXiGu:2012}. A full eigendecomposition can be computed in $O(d^2\cdot \polylog d)$ time \cite{pan1999complexity}. 

\subsection{Sublinear query algorithms for Toeplitz matrices} 

Recent work has focused on algorithms for Toeplitz matrices with complexity scaling \emph{sublinearly} in the dimension $d$ \cite{Abramovich:1999vs,Chen:2015wz,Qiao:2017tp,Wu:2017ub,Lawrence:2020ut,eldar2020toeplitz,kapralov2022toeplitz}. Kapralov et al. \cite{kapralov2022toeplitz} study low-rank approximation of positive semidefinite (PSD) Toeplitz matrices. They show that by accessing just $\poly(k,\log(d/\delta),1/\epsilon)$ entries of a PSD Toeplitz matrix $T \in \R^{d \times d}$, one can compute a symmetric Toeplitz matrix $\wt T$ with rank $\tilde O(k \log(1/\delta)/\epsilon)$ such that:\footnote{Throughout we use $\tilde O(\cdot)$ to hide polylogarithmic factors in the dimension $d$ and in the argument.}  
\begin{align}\label{eq:nearRelative}
\|T-\wt{T}\|_F \leq (1+\eps)\|T-T_k\|_F + \delta\|T\|_F,
\end{align}
where $\norm{M}_F = \sqrt{\sum_{i=1}^d \sum_{j=1}^d M_{ij}^2}$ is the Frobenius norm and $T_k = \underset{B:\rank(B)\leq k}{\argmin}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm, given by projecting $T_k$ onto its top $k$ eigenvectors. %$\wt T$ gives a near-optimal \emph{structure preserving} low-rank approximation of $T$. %Observe that since the dependence on $\delta$ is logarithmic, the optimality guarantee is near relative error.

%First we start with the work of \cite{kapralov2022toeplitz}. They showed that a near-optimal low rank approximation to $T$ can be computed by only reading $o(d)$ entries of it, formalized below.
%\begin{theorem}[Theorem 1 of \cite{kapralov2022toeplitz}]\label{thm:sublinear_lra_soda2023}
%There is an algorithm such that given any PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$, $0<\eps,\delta<1$ and an integer rank $k\leq d$, it reads $\wt O(k^2\log(1/\delta)\poly(1/\epsilon))$ entries of $T$ and returns a symmetric Toeplitz matrix $\wt{T}$ of rank $\wt O((k/\epsilon)\log(1/\delta))$,
%		$$\|T-\wt{T}\|_F \leq (1+\eps)\|T-T_k\|_F + \delta\|T\|_F,$$ where $T_k = \underset{B:rank(B)\leq k}{\argmin}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm.    
%\end{theorem}

Observe that $T_k$ may not itself be Toeplitz and it is not a priori clear that Toeplitz $\wt T$ satisfying \eqref{eq:nearRelative} even exists. The key technical contribution of \cite{kapralov2022toeplitz} is to prove that it does, and further that $\wt T$ can be recovered using sample efficient off-grid sparse Fourier transform techniques. Unfortunately, despite its sample efficiency, the algorithm of \cite{kapralov2022toeplitz} is computationally inefficient, with runtime that is  exponential in $\tilde O(k \polylog(d)/\epsilon)$  --  i.e., at least $d^{\tilde O(k/\epsilon)}$. The main open question left by their work is if this runtime can be improved, giving a sublinear time, not just a sublinear query, algorithm. %Roughly, the columns of $\wt T$ are spanned by $\tilde O(k/\epsilon)$ off grid frequencies, and the algorithm must perform a brute-force-search to identify these frequencies.

Eldar et al. \cite{eldar2020toeplitz} study the related problem of recovering an (approximately) low-rank Toeplitz covariance matrix $T \in \R^{d \times d}$ given independent samples from the $d$-dimensional Gaussian $\mathcal{N}(0,T)$. Low-rank Toeplitz covariance estimation is widely applied in signal processing, including in  direction of arrival (DOA) estimation  \cite{krim1996two}, spectrum sensing for cognitive radio \cite{ma2009signal,cohen2018analog}, and medical and radar image processing \cite{snyder1989use,ruf1988interferometric,fuhrmann1991application,brookes2008optimising,asl2012low,cohen2018sparse}. 
%
%We now turn to the work of \cite{eldar2020toeplitz} who also developed sublinear query algorithms in the context of Toeplitz matrices. The work of \cite{eldar2020toeplitz} is concerned with the following problem - given $s$ i.i.d. samples $x^1,x^2,\ldots, x^s$ from a $d$ dimensional Gaussian $\mathcal{N}(0,T)$ with covariance $T$ that is Toeplitz, estimate $T$ upto some error threshold. This problem statement is not only more realistic since the algorithm only has \emph{noisy} implicit access to $T$ via the i.i.d. samples as opposed to the setup of Theorem \ref{thm:sublinear_lra_soda2023}, but also it is directly relevant to practical applications. Toeplitz covariance structure emerges for example when the random measurement vector corresponds to measurements on a spatial or temporal grid, and the covariance between two coordinates just depends on the difference between them. Fast algorithms for this problem of estimating Toeplitz covariance matrices have many applications ranging from Direction of Arrival (DOA) estimation for signals received from antenna arrays \cite{krim1996two}, spectrum sensing for cognitive radio \cite{ma2009signal,cohen2018analog}, medical and radar image processing \cite{snyder1989use,ruf1988interferometric,fuhrmann1991application,brookes2008optimising,asl2012low,cohen2018sparse}. 
Motivated by these applications, \cite{eldar2020toeplitz} consider two relevant sample complexity measures: the vector sample complexity (VSC), which is the number of samples (each a vector in $\R^d$) taken from the distribution $\mathcal{N}(0,T)$, and the entry sample complexity (ESC), which is the number of entries read from each vector sample. % and runtime. We encapsulate the definitions of these complexity measures in the following definition, which we will refer to recurringly in the paper. 
%\begin{definition}\label{def:vsc_and_esc}
%Given $s$ i.i.d. samples $s$ of the form $x^1,x^2,\ldots,x^s \sim \mathcal{N}(0,T)$ consider any algorithm which estimates $T$ upto some specified error tolerance using these samples. The Vector sample complexity (VSC) is the number of i.i.d. samples $s$ of the form $x^1,x^2,\ldots,x^s \sim \mathcal{N}(0,T)$ an algorithm uses and the Entry sample complexity (ESC) is the number of entries the algorithm reads from each sample $x^i$ for $i\in [s]$.  
%\end{definition}
\cite{eldar2020toeplitz} show that with $\poly(k,\log d,1/\epsilon)$ VSC and ESC, it is possible to return $\wt T$ satisfying with high probability:\footnote{Throughout, we let $f(\cdot) \lsim g(\cdot)$ denote that $f(\cdot) \le c \cdot g(\cdot)$ for some fixed constant $c$.}
%The main result of \cite{eldar2020toeplitz} is to achieve a sublinear, i.e. $o(d)$, VSC and ESC, this is formalized below.
%\begin{theorem}[Theorem 2.10 in \cite{eldar2020toeplitz}]\label{thm:elmm_soda20}
%There is an algorithm such given i.i.d samples $x^1,x^2,\ldots, x^s\sim \mathcal{N}(0,T)$ for PSD Toeplitz $T\in \mathbb{R}^{d\times d}$ and parameters $k,\epsilon>0$, it has VSC $s=\wt O(k+1/\epsilon^2)$, ESC $\wt O(k^2\log(1/\epsilon))$ and returns a Toeplitz $\wt T$ satisfying the following with probability $0.9$,
\begin{equation}\label{eq:sampleBound}
    \|T-\wt T\|_2 \lsim \sqrt{\|T-T_k\|_2 \cdot  \tr(T)+ \frac{\|T-T_k\|_F \tr(T)}{k}} + \epsilon \|T\|_2,
\end{equation}
where $\tr(T)$ is the trace and $\norm{T}_2$ is the spectral norm.
%\end{theorem}
While the above error bound may seem somewhat non-standard,  \cite{eldar2020toeplitz} show that it implies fairly strong bounds when $T$ has low stable-rank. Observe that when $T$ is exactly rank-$k$, the error bound becomes $\epsilon \norm{T}_2$. As in \cite{kapralov2022toeplitz}, a key drawback is that algorithm of \cite{eldar2020toeplitz} has runtime scaling exponentially in  $\tilde O(k \polylog d)$. Further,   the output matrix $\wt T$ is not itself guaranteed to be low-rank.

%The main drawbacks of this result are that the runtime of the algorithm is $\exp(k)$ and the output Toeplitz $\wt T$ as per the Theorem then is not guaranteed to be low-rank. The error bound may seem non-standard as well, however \cite{eldar2020toeplitz} show that it implies fairly strong bounds when $T$ has low stable-rank.

\subsection{Our contributions}

In this work, we give a \emph{sublinear time} algorithm for computing a near-optimal low-rank approximation of a PSD Toeplitz matrix given noisy access to its entries. Our robust low-rank approximation primitive can be applied in the settings of both \cite{kapralov2022toeplitz} and \cite{eldar2020toeplitz}, yielding the first sublinear time algorithms for both standard PSD Toeplitz low-rank approximation and low-rank Toeplitz covariance estimation. Our main result is as follows:
\begin{theorem}[Robust Sublinear Time Toeplitz Low-Rank Approximation]\label{thm:sublinear_time_recovery}
	Let $T\in \mathbb{R}^{d\times d}$ be a PSD Toeplitz matrix, $E\in \mathbb{R}^{d\times d}$ be an arbitrary noise matrix, $\delta>0$ be an error parameter, and $k$ be an integer rank parameter. There exists an algorithm that, given query access to the entries of $T+E$, runs in $\poly(k,\log(d/\delta))$ time and outputs a representation of symmetric Toeplitz matrix $\wt T$ with rank $\poly(k,\log(d/\delta))$ that satisfies, with probability at least $0.9$,
	\begin{equation*}
		\|T- \wt T\|_F \lsim \max\{\|E\|_F,\|T-T_k\|_F\} + \delta \|T\|_F,
	\end{equation*}
	where $T_k = \argmin_{B: \rank(B)\leq k}\|T-B\|_F$ is the best rank-$k$ approximation to $T$.
\end{theorem}
Observe that given our runtime, which depends just poly-logarithmically on the input dimension $d$, it is not possible to output $\wt T \in \R^{d \times d}$ explicitly. Thus, our algorithm outputs a compressed representation of $\wt T$. To do so, we use the well known Vandermonde decomposition theorem, which states that any Toeplitz matrix can be diagonalized by a Fourier matrix \cite{cybenko1982moment}. We can show that $\wt T$ in particular, which has rank $r = \poly(k,\log(d/\delta))$, can be written as  $FDF^*$ where $F \in \mathbb{C}^{d\times r}$ is a Fourier matrix, with $j^{th}$ column given by $[1, e^{2\pi i \cdot f_j}, e^{2\pi i \cdot 2f_j},\ldots, e^{2\pi i  \cdot (d-1) f_j}]$ for some frequency $f_j$, and $D \in \R^{r \times r}$ is diagonal. Our algorithm outputs the frequencies $f_1,\ldots,f_r$ and diagonal entries $D_{1,1},\ldots,D_{r,r}$, which fully determine $\wt T$.

As an immediate consequence of Theorem \ref{thm:sublinear_time_recovery} applied with $E=0$, we obtain the following sublinear time constant factor low-rank approximation algorithm for PSD Toeplitz matrices, which resolves the main open problem of \cite{kapralov2022toeplitz} for the case of constant factor approximation.
\begin{theorem}[Sublinear Time Toeplitz Low-Rank Approximation]\label{thm:sublinear_time_lowrankapprox}
Let $T\in \mathbb{R}^{d\times d}$ be a PSD Toeplitz matrix, $k$ be an integer rank parameter, and $\delta>0$ be an error parameter. There exists an algorithm that, given query access to entries of $T$, runs in  $\poly(k,\log(d/\delta))$ time and outputs a representation of symmetric Toeplitz matrix $\wt T$ with rank $\poly(k,\log(d/\delta))$ that satisfies with probability at least 0.9,
	\begin{equation*}
		\|T- \wt T\|_F \lsim \|T-T_k\|_F + \delta \|T\|_F.
	\end{equation*}
	%where $T_k = \argmin_{B: \rank(B)\leq k}\|T-B\|_F$ is the best rank-$k$ approximation to $T$.
\end{theorem}
We can further apply Theorem \ref{thm:sublinear_time_recovery} to the Toeplitz covariance estimation setting of \cite{eldar2020toeplitz}. Here, we set $E=\frac{1}{s} \cdot XX^T -T$ where $X \in \R^{d \times s}$ has $s$ columns sampled i.i.d. from the multivariate Gaussian distribution $\mathcal{N}(0,T)$. That is, $E$ is the error between the true covariance matrix $T$ and a sample covariance  matrix $\frac{1}{s} XX^T$ that our algorithm can access. Using similar ideas to \cite{eldar2020toeplitz}, we show that for $s = \tilde O(k^4/\epsilon^2)$, $\norm{E}_F \lsim \sqrt{\|T-T_k\|_2 \tr(T)+ \frac{\|T-T_k\|_F \tr(T)}{k}} + \epsilon \|T\|_2$. Combined with Theorem \ref{thm:sublinear_time_recovery} applied with $\delta = \epsilon/\sqrt{d}$ so that $\delta \norm{T}_F \le \epsilon \norm{T}_2$, this gives:
\begin{theorem}[Sublinear Time Toeplitz Covariance Matrix Estimation]\label{thm:sublinear_time_covariance_estimation}
	Let $T\in \mathbb{R}^{d\times d}$ be a PSD Toeplitz matrix, $k$ be an integer rank parameter, and $\epsilon > 0$ be an error parameter. There is an algorithm that given i.i.d. samples $x^1,\ldots, x^s \sim \mathcal{N}(0,T)$ for $s=\tilde O(k^4/\epsilon^2)$, runs in $\poly(k,\log (d/\epsilon))$ time and outputs a representation of symmetric Toeplitz $\wt T$with rank $\poly(k,\log(d/\epsilon))$ satisfying, with probability at least 0.9,
	\begin{equation*}
		\|T- \wt T\|_F \lsim \sqrt{\|T-T_k\|_2 \tr(T)+ \frac{\|T-T_k\|_F \tr(T)}{k}} + \epsilon \|T\|_2.
	\end{equation*}
	Further, the algorithm has entry sample complexity (ESC) $\poly(k,\log (d/\epsilon))$ --  it reads just  $\poly(k,\log (d/\epsilon))$ entries of each vector sample $x^i$.
\end{theorem}
Observe that the error guarantee of
Theorem \ref{thm:sublinear_time_covariance_estimation} is at least as strong, and can potentially be much stronger, than that of \eqref{eq:sampleBound}, since the bound is on $\norm{T-\wt T}_F$ rather than $\norm{T - \wt T}_2$. At the same time, our algorithms achieves the same vector and entry sample complexities as \cite{eldar2020toeplitz} up to $\poly(k,\log (d/\epsilon))$ factors, while running in sublinear time. Moreover, our output $\wt T$ is guaranteed to be low-rank, while the output of \cite{eldar2020toeplitz} is not.



%At its heart, our algorithm solves the following problem.  Consider a function $x(t)$ where $x:\mathbb{Z}\to \mathbb{C}$, and $x$ is $k$-sparse in Fourier domain. Then, assuming noisy sample access to the function at any $t\in [d]=\{0,1,\ldots,d\}$, recover the $k$ potentially ``off-grid'' frequencies in the support of $\wh x(f) $ approximately in $\poly(k)$ time. The continuous time version of this problem, that is the $k$-Fourier sparse function $x(t)$ is from $x:\mathbb{R}\to \mathbb{C}$ and one has noisy sample access to it for any $t\in [0,d]$, was studied and solved in \cite{chen2016fourier}. The discrete time version we consider poses additional challenges when compared to \cite{chen2016fourier} due to the constraint that we can only access the function at integer points in $[0,d]$. The formal statement of this result is presented in section 4 as Lemma \ref{lem:heavy_freq_recovery}.

\subsection{Our approach}\label{sec:approach}
In this section, we sketch the ideas behind the proof of our main result: the sublinear time robust Toeplitz low-rank approximation algorithm of Theorem \ref{thm:sublinear_time_recovery}. Our starting point is the main result of \cite{kapralov2022toeplitz}, which shows that any PSD Toeplitz matrix has a near optimal low-rank approximation $\wt T$ which is itself Toeplitz. Armed with this existence result,  the key idea behind the algorithm of \cite{kapralov2022toeplitz} is to leverage the well-known sparse Fourier structure of low-rank Toeplitz matrices \cite{cybenko1982moment} to recover $\wt T$ using a sample efficient (but computationally inefficient) algorithm. %In particular, they leverage the well-known Vandermonde decomposition theorem, which shows that any Toeplitz matrix can be diagonalized by an {off-grid} Fourier matrix. Formally,
The  idea behind \cite{eldar2020toeplitz} is similar, except that they rely on a weaker existence statement, where the low-rank approximation $\wt T$ is guaranteed to have sparse Fourier structure, but not necessarily be Toeplitz.
Formally, after defining the notion of a Fourier matrix, we state the main result of \cite{kapralov2022toeplitz}.
\begin{definition}[Fourier matrix]\label{def:symmetric_fourier_matrix}
	For any set of frequencies $S=\{f_1,f_2,\ldots, f_s\}\subset [0,1]$, let the Fourier matrix $F_S\in \mathbb{C}^{d\times s}$ have $j^{th}$ column equal to $v(f_j) \eqdef [1, e^{2\pi i f}, e^{2\pi i (2f)}\ldots, e^{2\pi i  (d-1) f}]$.
	%For every $j\in \{1, 2,\ldots, s\}$ the $j$-th column of $F_{S}$ is the frequency vector $v(f_{j})$. 
\end{definition}


\begin{theorem}[Theorem 2 of \cite{kapralov2022toeplitz}]\label{frobeniusexistence}
        For any PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$, $0<\eps,\delta<1$, and $k\leq d$, there exists symmetric Toeplitz $\wt{T}$ with rank $r = \tilde {O}(k \log(1/\delta)/\eps))$ such that
		$$\|T-\wt{T}\|_F \leq (1+\eps)\|T-T_k\|_F + \delta\|T\|_F.$$ %where $T_k = \underset{B:rank(B)\leq k}{\argmin}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm.
		
		Further, $\wt T$ can be written as $\wt T = F_S D F_S^*$ where $F_S \in \mathbb{C}^{d \times r}$ is a Fourier matrix (Def. \ref{def:symmetric_fourier_matrix}) and $D \in \R^{r \times r}$ is diagonal.
\end{theorem}



%
%\begin{theorem}[Vandermonde Decomposition \cite{cybenko1982moment}]\label{thm:vandermonde}
%	Any PSD Toeplitz matrix $T \in \R^{d\times d}$ of rank $r$ can be written as $T = F_SDF_S^{*}$ where $F_S \in \mathbb{C}^{d\times r}$ is a Fourier matrix with frequencies $S=\{f_1,\ldots,f_r\}\subset [0,1]$ and $D\in \mathbb{R}^{r\times r}$ is a diagonal matrix with $r$ positive entries. Moreover for every $j\in [r]$ there is a $j'\in [r]$ such that $e^{2\pi if_j}=e^{-2\pi i f_{j'}}$ and $D_{jj}=D_{j'j'}$.
%\end{theorem}

%that $\tilde T$ guaranteed to exist by Theorem \ref{frobeniusexistence} admits a BLAH. The work of \cite{eldar2020toeplitz} follows a similar approach, except only is able to show that BLAH.


%\Cam{This can be either removed or moved to the prelims if needed.}
%\begin{definition}[Frequency vector]\label{freqvector}
%	For any frequency $f \in [0,1]$, we define the {\em frequency vector} $v(f) \in \mathbb{C}^d$ as the column vector $[1, e^{2\pi i f}, e^{2\pi i (2f)}\ldots, e^{2\pi i  (d-1) f}]^T$.
%\end{definition}

%Equipped with these basic concepts,
%the main result of \cite{kapralov2022toeplitz} is stated below as promised.
%\begin{theorem}[Informal version of Theorem 2 of \cite{kapralov2022toeplitz}]\label{frobeniusexistence}
%        Given any PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$, $0<\eps,\delta<1$ and an integer $k\leq d$, there exists a symmetric Toeplitz matrix $\wt{T}=F_{\wt S}\wt D F_{\wt S}^*$ where $\wt S\subset [0,1]$ of size $|\wt S|=\wt{O}((k/\eps)\log(1/\delta))$, $F_{\wt S}$ as per Definition \ref{def:symmetric_fourier_matrix}, and $\wt D\in \mathbb{R}^{|\wt S| \times |\wt S|}$ is a diagonal matrix such that,
%		$$\|T-\wt{T}\|_F \leq (1+\eps)\|T-T_k\|_F + \delta\|T\|_F,$$ where $T_k = \underset{B:rank(B)\leq k}{\argmin}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm.
%\end{theorem}

To prove Theorem \ref{thm:sublinear_time_recovery}, we apply Theorem \ref{frobeniusexistence} to the input PSD Toeplitz matrix $T$ with $\epsilon = \Theta(1)$. Our algorithm is given access to the entries of the noisy matrix $T+E$, which we will write as $\wt T + \wt E$ for $\wt E = E + T-\wt T$. Observe that by triangle inequality, since $\norm{T-\tilde T}_F \lsim \norm{T-T_k}_F + \delta \norm{T}_F$,
$$\norm{\wt E}_F \lsim \norm{E}_F + \norm{T-T_k}_F + \delta \norm{T}_F \lsim \max\{  \norm{E}_F, \norm{T-T_k}_F\} + \delta \norm{T}_F.$$

Thus, to prove Theorem \ref{thm:sublinear_time_recovery} it suffices to show that we can recover $\wt T$ to within a constant factor of the noise level $\norm{\wt E}_F$. Our key contribution is to improve the runtime of this step from being exponential in the rank $r = \tilde O(k \log(1/\delta))$ to being polynomial, and hence sublinear in $d$ (recall that throughout $\tilde O(\cdot)$ hides poly logarithmic factors in $d$ and the argument).

To approximately recover $\wt T$, as in \cite{kapralov2022toeplitz} and \cite{eldar2020toeplitz}, we will leverage its Fourier structure. In particular, 
Theorem \ref{frobeniusexistence} guarantees that $\wt T$ can be written as $\wt T = F_S D F_S^*$, where $F_{S} \in \mathbb{C}^{d \times r}$ is a Fourier matrix (Def. \ref{def:symmetric_fourier_matrix}) and $D \in \R^{r \times r}$ is diagonal. To find $\wt T$, the algorithm of \cite{kapralov2022toeplitz} brute force searches for a good set of frequencies $S$ and corresponding diagonal matrix $D$. In particular, they consider a large pool of candidate frequency sets drawn from an $\epsilon$-net over $[0,1]^r$. For each set $S$, they solve a regression problem to find a diagonal matrix $D$ that (approximately) minimizes $\norm{T-F_S D F_S^*}_F$. These regression problems can be solved using a sublinear number of queries to $T$ using leverage score based random sampling. One can then return the best approximation given by any of the candidate frequency sets as the final output. 

Unfortunately, the above approach incurs exponential runtime, as the number of frequency sets that must be considered grows exponentially in the rank $r = \tilde O(k \log(1/\delta))$. A similar issue plagues the algorithm of \cite{eldar2020toeplitz}, which also performs a brute force search over frequency sets, but with a different regression step, where $D$ is relaxed to be any $r \times r$ matrix.

\medskip 

\noindent{\textbf{Contribution 1: From Column Recovery to Matrix Recovery.}
To avoid this exponential runtime, we will apply tools from the extensive literature on efficient recovery of Fourier-sparse functions \cite{hassanieh2012nearly,indyk2014sample,indyk2014nearly,Boufounos:2015vj,kapralov2016sparse,chen2016fourier,Jin:2023uc}. Observe that if we expand out the decomposition $\wt T = F_S D F_S^*$,  each column of $\wt T$ is an $r$-Fourier sparse function from $[d] \rightarrow \R$. In particular, letting $\wt T_j$ denote the $j^{th}$ column, for any $t \in [d]$, letting $\{a_f\}_f \in S$ be the diagonal entries of $D$,
$$\wt T_j(t) = \sum_{f\in S}a_f e^{2\pi i f(t-j)}.$$ 

Our algorithm will recover a Fourier-sparse approximation to a single column of $\wt T$ using samples of $T + E = \wt T + \wt E$ in just $\poly(r,\log d)$ time using a sparse Fourier transform algorithm. This Fourier-sparse approximation will give us approximations to the frequencies in $F_S$ and the diagonal entries of $D$, which in turn can be used to form an approximation to $\wt T$.

This approach presents several challenges. First, we must ensure that the column that we apply sparse Fourier transform to does not have too much noise on it, compared to its norm. To do so, we sample a random column, which by Markov's inequality, is corrupted with noise whose $\ell_2$ norm is bounded by $\lsim \norm{\wt E}_F/\sqrt{d}$ with good probability. Further, using the fact that $\wt T$ is close to $T$ and hence nearly PSD, we can apply a norm compression inequality of Audenaert \cite{audenaert2006norm} to show that each column of $\wt T$ must have $\ell_2$ norm $\gsim \norm{\wt T}_F/\sqrt{d}$. In combination, these facts ensure that a random column has a similar signal-to-noise ratio as the full matrix $\wt T$ with good probability. Thus, we can expect to recover a good approximation to $\wt T$ from just this column.

Of course, given the noise $\wt E$, we cannot expect to recover approximations to all frequencies in $S$ given sample access to $\wt T + \wt E$. For example, if a frequency $f$ corresponds to a very small entry $a_f$ in $D$, we may not recover it. We must argue that omitting such  frequencies from our approximation of $\wt T$ does not introduce significant error. Again, to do so we will leverage the fact that $\wt T$ is close to PSD and apply a novel `heavy-light' frequency decomposition for PSD Toeplitz matrices.

We detail our approaches to the above challenges further in Section \ref{sec:sublinear_toeplitz_recovery}.

\medskip

\noindent\textbf{Contribution 2: Sublinear Time Discrete-Time Off-Grid Sparse Fourier Transform.}
After showing that applying a sparse Fourier transform to a random column of $\wt T$ suffices to recover a good approximation to the full matrix, it remains to show that we can implement such a sparse Fourier transform efficiently.

%We can thus hope to recover the first column $\wt T_1$, and in turn $\wt T$ using noise-robust sparse Fourier recovery techniques. % on $\wt T_1(t)$, and then fit $\wt D$ using fast regression primitives. This approach was adopted by \cite{kapralov2022toeplitz} however their sparse Fourier recovery algorithm recovered the frequencies using a brute force search running in $\exp(k)$ time, which resulted in an inefficient running time overall.

If the frequencies in $S$ were integer multiples of $1/d$, i.e., they were ``on-grid'', %then the function $\wt T_j(t)$ would be a periodic function with period $d$, and thus completely determined by its values at the integer points $t\in [d]$. 
then we could apply a discrete sparse Fourier transform algorithm to  recover a Fourier-sparse approximation to a random column $\wt T_j$ of $\wt T$ given samples from the column $[T+E]_j = [\wt T + \wt E]_j$. Such algorithms  have been studied extensively in recent years \cite{hassanieh2012nearly,Hassanieh:2012tq,Gilbert:2014tp}. However, the main difficulty in our case is that the frequencies in $S$ may be ``off-grid'', i.e., arbitrary real numbers in $[0,1]$. % in general and thus $\wt T_1(t)$ may have a period $>>d$ making the problem hard. 
Recent work of \cite{chen2016fourier} solves the off-grid sparse Fourier transform problem given sample access to the function $[\wt T +\wt E]_j$ on the \emph{continuous range $[0,d]$}. However, in our setting, we can only access $[\wt T + \wt E]_j$ at the integer points $\{0,1,\ldots,d-1\}$ -- i.e., at the entries in the $j^{th}$ column of our matrix. We must substantially modify the approach of  \cite{chen2016fourier} to show that, nevertheless, we can well approximate $\wt T_j$ from samples  at these points. In doing so, we give to the best of our knowledge, the first efficient \emph{discrete time off-grid} sparse Fourier transform algorithm, which may be applicable in other settings that involve off-grid frequencies but on grid time samples.

We detail our discrete time off-grid sparse Fourier transform algorithm in Section \ref{section:dtft_recovery_techintro}.

%$Since the frequencies in $S$ lie in $[0,1]$, by the Shannon-Nyquist theorem, the function $T_j$ is completely determined by its values at the integers. 

%The work of \cite{chen2016fourier} solved this problem in more generality when $\wt S \subseteq [-F,F]$ for any bandlimit $F$, given access to the input at all $t\in [0,d]$. This won't work in our setting as is, since we only have access to the input at \emph{integer} $t\in [d]=[0,d]\cap \mathbb{Z}$. It is important to note that since all frequencies in $\wt S$ are in $[0,1]$, by the Shannon-Nyquist theorem $\wt T_1(t)$ is completely determined by its values at all $t\in \mathbb{Z}$. Moreover if one settles for recovering frequencies in $\wt S$ \emph{approximately},  then we can hope to use tools from \cite{chen2016fourier} to deal with the fact that we can only access the input on a bounded interval $[0,d]\cap \mathbb{Z}$ and not the entire $\mathbb{Z}$. It is not trivial how to make the framework of \cite{chen2016fourier} work in this case, and that is our first contribution discussed below.


\section{Technical Overview}\label{sec:overview}

We next describe our main contributions in more detail. We first detail our efficient discrete time off-grid sparse Fourier transform in Section \ref{section:dtft_recovery_techintro}. In Section Section \ref{sec:sublinear_toeplitz_recovery} we use this primitive to prove Theorem \ref{thm:sublinear_time_recovery}, by showing how to recover a low-rank Toeplitz approximation $\wt T$ to out input matrix $T$ by applying our sparse Fourier transform to a random  column of the input matrix.

%\Cam{UP TO HERE.}

%\Cam{This was out of place. Move elsewhere. For any function $f:\mathbb{Z}\rightarrow \mathbb{C}$, let $\|f\|_d^2 := \sum_{t\in [d]}|f(t)|^2$. }

\subsection{Discrete Time Off-Grid Sparse Fourier Recovery}\label{section:dtft_recovery_techintro}
A discussed, a key primitive used in our robust Toeplitz low-rank approximation algorithm is an efficient  discrete time off-grid sparse Fourier transform. Informally,  such an algorithm must solve the following sparse Fourier recovery problem:

\Cam{Is the indexing off here? Should $t$ range from $0$ to $d-1$?}
\begin{problem}\label{def:problem_definition}(Off-Grid Sparse DTFT -- Informal)
Let $x^*(t) = \sum_{j=1}^k a_j e^{2\pi i f_j t}$ for $t\in [d]$ and $f_1,\ldots,f_k \in [0,1]$. Let $x(t) = x^*(t)+g(t)$, where $g$ is arbitrary noise. Given sample access to $x(t)$ for any $t\in [d]$, approximately recover all $f_j$ that contribute significantly to $x$. % in $\poly(k, \log d)$ time. %Remark: Note that since we only have time domain access at points $t\in [d]$, this is a harder problem than the one studied in \cite{chen2016fourier}\kstodo{add footnote formalizing the connection}.
\end{problem}
The work of \cite{chen2016fourier} solves the above problem in the more general case when $f_1,\ldots,f_k \in [-F,F]$ for some bandlimit $F$. However, their algorithm critically requires sample access to $x(t)$ for any $t\in [0,d]$. Prony's method \cite{Prony:1795wv} can exactly recover all frequencies $f_j$ and coefficients $a_j$ using just $2k$ samples -- but only in the noiseless setting when $g(t) = 0$.
Observe that in the presence of noise it generally will not be possible to identify all frequencies $f_j$ given sample access to $x(t)$ only on $[d]$. For example, if two frequencies $f_j$ and $f_{j'}$ are extremely close to each other, their contributions to the function $x$ could nearly cancel out, making it impossible to identify them in the presence of noise. 

\Cam{But *why* do we even need to filter the time domain to $[d]$?}
Furthermore we cannot simply truncate the signal to $[d]$, say by multiplying it with the indicator function of the interval $[d]$, as this hard thresholding operation will spread out the frequencies of $x^*$ a lot. To mitigate this \cite{chen2016fourier} design a function $H:\mathbb{Z}\rightarrow
\mathbb{R}$ that satisfies the following for any $k$-sparse $x^*(t):\mathbb{Z}\rightarrow \mathbb{C}$ and $\delta>0$, \Cam{How could it possibly satisfy this for any $\delta$?}
\begin{align}\label{eqn:H_properties_summary}
		 \sum_{t \in \mathbb{Z}\setminus [d]} |x^*(t) \cdot H(t) |^2 &\leq \delta \|x^*\|_d^2\\
		 0.99\|x^*\|_d^2\leq \sum_{t \in [d]} |x^*(t) \cdot H(t) |^2 &\leq \|x^*\|_d^2,
\end{align}
where for any function $f:\mathbb{Z}\rightarrow \mathbb{C}$, we define $\|f\|_d^2 \eqdef \sum_{t\in [d]}|f(t)|^2$.
\Cam{Its more like they design a function satisfying a continuous variant of this and we show that it also satisfies the discrete variant right?}

Furthermore, $supp(\wh{H})$ lives in an interval of size $\poly(k,\log(d/\delta)/d$. Intuitively, the $H$ function approximates the indicator function of the interval $[d]$ by almost killing off the energy of $x^*(t)$ outside $[d]$ and preserving the energy inside $[d]$; and at the same time it is compact in Fourier domain, that is the support of $\wh{H}(f)$ lives in an interval of size at most roughly $\poly(k)/d$. The formal definition and properties of $H$ are in Lemma \ref{lem:H_discrete_properties} imported from \cite{chen2016fourier}. Thus for approximate frequency recovery, we can work with $x\cdot H$ instead of $x$.

The Fourier transform of $x^*\cdot H$ will be $\wh{x^*\cdot H}=\widehat{x^*}\ast \widehat{H}$ ($\ast$ is the convolution operator). Since $|supp(\wh{H})|\leq \poly(k,\log(d/\delta))/d$,  all of the mass of $\widehat{x^*}\ast \widehat{H}$ is within $\poly(k,\log(d/\delta))/d$ of all the frequencies in $supp(\widehat{x^*})$. Thus, for every frequency of $supp(\widehat{x^*})$ which is not corrupted by noise, one can aim for locating it approximately with an additive error of roughly $\poly(k,\log(d/\delta))/d$. Moreover we can aim for recovering a list of frequencies such that for every frequency of $\wh{x^*}$ not corrupted by noise, this list will contain at least one frequency within distance $\poly(k,\log(d/\delta))/d$ of it. We can indeed achieve this in $\poly(k,\log(d/\delta))$ time as shown below.
\begin{lemma}\label{lem:dtft_freqrecovery}(Informal version, formal version in section \ref{sec:dtft_recovery}) Consider the input of problem definition \ref{def:problem_definition}.
Suppose we are given $\delta>0$ and assume $\|g\|_d^2 \leq c\|x^*\|_d^2$ for a small absolute constant $c>0$. Then in time and sample complexity $\poly(k,\log(d/\delta))$ one can find a list $L$ of $\poly(k)$ frequencies that satisfies the following with probability at least $0.99$ - Let $$S(L)=\{f\in supp(\wh{x^*}): \exists f'\in L \text{ s.t. } |f-f'|_{\circ}\leq \poly(k,\log(d/\delta)/d\},$$ and let $x^*_{S(L)}=\sum_{f\in S(L)}a_je^{2\pi i f t}$. Then $$\|x^*-x^*_{S(L)}\|_d^2 \lsim \|g\|_d^2 +\delta \|x^*\|_d^2.$$ Here $|\cdot|_{\circ}$ is the wrap-around distance (see Defn. \ref{wraparounddefn})
\end{lemma}
\cite{chen2016fourier} prove a similar version of this lemma in Lemma 7.23 in \cite{chen2016fourier} when one has sample access at all real numbers $t\in [0,d]$. We now discuss the algorithm of \cite{chen2016fourier}, why it does not work in our setting and how we fix it. Overall, the algorithm of \cite{chen2016fourier} first works by considering the \emph{clustered} case. This case is when most of the energy of $z = x\cdot H$ in Fourier domain is concentrated around some $f_0\in [0,1]$; they show how to recover an $f'$ satisfying $|f'-f_0|_{\circ}\leq \poly(k,\log(d/\delta))/d$ in $\poly(k,\log(d/\delta))$ time in this case. The second part of the algorithm of \cite{chen2016fourier} is to use hashing based techniques to reduce the general case to the clustered case. We first discuss the clustered case.

\textbf{Issue with the One-Cluster case.}
The formal definition of this case is as follows.
\begin{definition}[$(\epsilon,\Delta)$-one clustered signal]\label{def:one_clustered_signal}
	For a $f_0\in [0,1]$,  $z:\mathbb{Z}\to \mathbb{C}$ is $(\epsilon,\Delta)$-one clustered around $f_0$ if 
	\begin{align*}
		\textnormal{ Property I: } & \quad \int_{f_0 - \Delta}^{f_0 + \Delta} |\wh{z}(f)|^2 df \geq  (1 - \eps) \int_{0}^{1} |\wh{z}(f)|^2  df \\
		\textnormal{Property II: } & \quad \|z\|_d^2 \geq  (1 - \eps) \sum_{t \in \Z} |z(t)|^2. 
	\end{align*}
\end{definition}
The goal here is to find an $f'$ such that $|f'-f_0|\lsim \poly(k,\log(d/\delta))/d$. The main subroutine in \cite{chen2016fourier} for this case is given any $\beta$ not too large,  they can output an $\alpha$ such that $ z(\alpha+\beta)/z(\alpha)$ approximates $e^{2\pi i f_0 \beta}$ with high constant probability. It is not hard to ensure that this subroutine outputs an integer $\alpha\in [d]$ for an integer $\beta$. This is presented in section \ref{subsubsec:sampling_the_signal}. However, this does not translate into a highly accurate estimate, i.e., within $\poly(k,\log(d/\delta))/d$, of $f_0$. \cite{chen2016fourier} then repeatedly use this subroutine inside a $t$-ary search for $t\approx \log d$ to iteratively refine and obtain the final approximation to $f_0$ within $\poly(k,\log(d/\delta)/d$. The key component in this $t$-ary search is to choose $\beta$ randomly such that for $f$ that are ``far away'' from $f_0$, $2\pi \beta |f-f_0|_{\circ}$ is almost uniformly distributed on the circle, that is,
\begin{equation}\label{eqn:low_prob_far_candidates}
\Pr[2\pi \beta |f-f_0|_{\circ} \mod 2\pi \in [-3s\pi/2,3s\pi/2]]\leq 10s.    
\end{equation}
for some small constant $s$. This property is used to ensure that all such $f$ that are far away from $f_0$ get successfully discarded in each iteration of the $t$-ary search and we make progress. \cite{chen2016fourier} show that in each iteration of the $t$-ary search, if $\beta$ is chosen to be a uniformly random \emph{real} number in a carefully chosen range then equation \ref{eqn:low_prob_far_candidates} is satisfied for all $f$ not too close to $f_0$, thus they get discarded in the search and the search space is reduced by a factor $t$. We need $\beta$ to be an integer as we will be querying $z$ at time $\alpha+\beta$ for some integer $\alpha$ as discussed in the previous paragraph. Sampling $\beta$ to be uniformly random \emph{integer} in the same range cannot guarantee equation \ref{eqn:low_prob_far_candidates} as is because for eg. if $|f-f_0|_{\circ}=1/2$ then $2\pi \beta |f-f_0|_{\circ} = \pi \beta = 0 \mod 2\pi $ for every even $\beta$. Keeping this issue in mind we now state the next issue when adapting \cite{chen2016fourier} to the discrete time setting

%\textbf{alternative:} \cite{chen2016fourier} show that in iteration $i$, if $\beta$ is sampled uniformly from roughly $[0.5(\log(d))^i, (\log(d))^i)]$ then equation \ref{eqn:low_prob_far_candidates} is satisfied for all $f$ such that $|f-f_0|\gsim 1/(0.25\log(d))^i$. We need $\beta$ to be an integer as we will be querying $z(\alpha+\beta)$ for some integer $\alpha$. Sampling $\beta$ to be uniformly random \emph{integer} in the same range $[0.5(\log(d))^i, (\log(d))^i)]$ cannot guarantee equation \ref{eqn:low_prob_far_candidates} as is because for eg. if $|f-f_0|=1/2$ then $2\pi \beta |f-f_0| = \pi \beta = 0 \mod 2\pi $ for every even $\beta$. Keeping this issue in mind we now state the next issue when adapting \cite{chen2016fourier} to the discrete time setting.

\textbf{Issue with the Multi-Cluster case.} 
The final part of the algorithm of \cite{chen2016fourier} is to reduce a general instance to a one-cluster instance as per Definition \ref{def:one_clustered_signal}. They acheive this reduction using hashing techniques. Consider the following hash function $h_{\sigma,b}:[0,1]\rightarrow \{0,\ldots,B-1\}$,
\begin{align}\label{eqn:hash_fn}
    \pi_{\sigma,b}(f) &= 2\pi \sigma (f-b) \mod 2\pi\\
    h_{\sigma,b}(f) &= \text{round}(\frac{B}{2\pi}\pi_{\sigma,b}(f))
\end{align}
where $\sigma\in \mathbb{R},b\in [0,1]$, $B$ is the number of hash buckets, and the round$(.)$ function rounds real numbers to the nearest integer. The crucial claim that \cite{chen2016fourier} show is that if we let $\sigma$ to be a uniformly random real number in an appropriate range, then we have that for any $f_1,f_2$ not too close,
\begin{equation}\label{eqn:low_collision_prob}
    \Pr [h_{\sigma,b}(f_1)=h_{\sigma,b}(f_2)]=\Pr [2\pi \sigma (f_1-f_2)\mod 2\pi \in [-2\pi/B,2\pi/B]]\lsim 1/B,
\end{equation}
implying $f_1,f_2$ collide with low probability. Furthermore, \cite{chen2016fourier} also design a filter function $G^{(j)}_{\sigma,b}$ for every $j\in [B]$ which when convolved with essentially gives access to the function only containing frequencies that hashed to bin $j$. Then \cite{chen2016fourier} use equation \ref{eqn:low_collision_prob} to show that for any recoverable $f$, i.e., satisfying the condition of Lemma \ref{lem:dtft_freqrecovery}, the bound \ref{eqn:low_collision_prob} with a union bound implies that no other frequency in $supp(\wh{x^*})$ collides with $f$. These facts can then be used to argue that bins containing isolated heavy frequencies with low SNR are essentially one-clustered, thus allowing us to recover the isolated frequency approximately. \cite{chen2016fourier} design an algorithm \hyperref[alg:hashtobins]{\textsc{HashToBins}} \kstodo{Do we discuss differences in new analysis compared to CKPS?}to compute the value of the signal containing frequencies only from a single hash bucket at any desired time instant as required by the one-cluster recovery algorithm. However to use this algorithm in our context, $\sigma$ must be an \emph{integer}, this is formally presented in Lemma \ref{lem:hashtobins}. Instead if we try to choose $\sigma$ to be a uniformly random integer in the same range needed by equation \ref{eqn:low_collision_prob}, we face the same issue as in the one-cluster case. More specifically consider any $f_1,f_2$ such that $|f_1-f_2|_{\circ} = 1/2$, then for $2\pi \sigma |f_1-f_2| = \pi \sigma = 0 \mod 2\pi$ for every even $\sigma$. Thus we cannot hope to prove equation \ref{eqn:low_collision_prob} with any probability smaller than $1/2$.\\
\textbf{Recovery for Bounded Instances.}
The source of the issues in the one-cluster and the multi-cluster case is identical upto different parameter settings. We now discribe our fix. We call an input \emph{bounded} (see Definition \ref{def:bounded_freq_case} for the formal definition) if essentially $supp(\wh{x^*})$ lives in an interval of size $1/B$ and the energy of the noise outside this interval is bounded. Consider any $f_1,f_2$ such that $F:=|f_1-f_2|_{\circ}\leq 1/B$. Then if we consider $\sigma$ to be a random \emph{integer} number in the same range as needed by equation \ref{eqn:low_collision_prob}, $2\pi \sigma |f_1-f_2|_{\circ}=2\pi \sigma F$ is distributed on a grid with uniform spacing, with the spacing at most $2\pi/B$. Thus we can hope that for every value of $\sigma$ such that $2\pi \sigma F \mod 2\pi \in [-2\pi/B,2\pi/B]$, there are $\gsim B$ values of $\sigma$ for which $2\pi \sigma F \mod 2\pi \notin [-2\pi/B,2\pi/B]$, since the grid on which $2\pi \sigma F$ lies is fine enough. We are able to formally show that this is enough to ensure equation \ref{eqn:low_collision_prob} holds for frequencies in a bounded instance. This claim when applied more generally also fixes the issue appearing in the one-cluster case when proving equation \ref{eqn:low_prob_far_candidates}.


The final part is to actually reduce a general instance to a bounded instance. To do this, we first state an observation. Consider the hash function as per equation \ref{eqn:hash_fn} for $\sigma =1$ and any $b\in [0,1]$. Then one can observe that the hash buckets are simply the intervals $$[b-1/2B,b+1/2B],[b+1/2B,b+3/2B],\ldots,[b-3/2B,b-1/2B]$$ where each interval is modulo 1. Essentially the hash function $h_{1,b}$ chops up $[0,1]$ into $B$ intervals of length $1/B$. Thus $G^{(j)}_{1,b}$ is (almost) the indicator function of the $j^{th}$ interval/bucket, and convolving the input with it gives access to the input only containing frequencies in the $j^{th}$ interval/bucket, which will thus be \emph{bounded}. Since $\sigma=1$ we can compute the convolution of the input with $G^{(j)}_{1,b}$ by simply running \hyperref[alg:hashtobins]{\textsc{HashToBins}}.  Overall with this additional layer of hashing on top, we can reduce a general instance into $B$ bounded instances. The proofs are in general have complicated details, which we defer to section \ref{subsubsection:multi_cluster_reduce}, and we also present the proof of Lemma \ref{lem:dtft_freqrecovery} in section \ref{subsubsection:multi_cluster_reduce}. Then for each of the $B$ bounded instances we apply the again apply the hashing based reduction to reduce a multi cluster bounded instance to a one cluster instance as discussed before in section \ref{subsubsection:multi_cluster_bounded_freqs}, and state the main claim and algorithm of recovering frequencies from a bounded instance in \ref{subsection:recovering_all_freqs_by_boosting}. Finally, we present the algorithm to find the central frequency of a one-cluster instance obtained from a bounded instance in section \ref{subsection:one_cluster}.\
\subsection{Sublinear Time Algorithms for Toeplitz Matrices}\label{sec:sublinear_toeplitz_recovery}
%\Cam{This section needs to be organized. Theorems 1-3 should already be stated and discussed in the intro. So you should not have an intro to this section stating them again without proof. You can maybe move some of this content to the intro. The section should simply first prove Theorem 1 via the heavy light decomposition. And then have a subsection which proves Theorem 2 as an immediate consequence and Theorem 3 as well.}
Equipped with our sublinear time off-grid sparse recovery scheme of Lemma \ref{lem:dtft_freqrecovery} and the existence result of Theorem \ref{frobeniusexistence}, we now describe the proof of our main result on sublinear time Toeplitz matrix approximation, Theorem \ref{thm:sublinear_time_recovery}. \Cam{Should remind reader in a few words what this Lemma actually is. Also should say you are using Theorem 8 as well I think}. We then apply Theorem \ref{thm:sublinear_time_recovery} to prove the result on computing a Toeplitz low-rank approximation in sublinear time Theorem \ref{thm:sublinear_time_lowrankapprox}, and learning the Toeplitz covariance matrix of a Gaussian distribution using sublinear sample complexity and running time Theorem \ref{thm:sublinear_time_covariance_estimation}. \Cam{Should reminder reader what these theorems are in words. Like I did with Theorem 1 above.}%We first restate Theorem \ref{thm:sublinear_time_recovery} before giving its proof.

%\Cam{I updates some wording in the theorem statement. Please update in intro as well. I also removed the variable $r = |S|$ as it was no neccesary in the statement. So if you use it later make sure to define it-Done}
%\begin{reptheorem}{thm:sublinear_time_recovery}
	%Let $T\in \mathbb{R}^{d\times d}$ be a PSD Toeplitz matrix, $E\in \mathbb{R}^{d\times d}$ be arbitrary noise, $\delta>0$ be an error parameter, and $k$ be a positive integer rank parameter. Given query access to the entries of $T+E$, in time $\poly(k,\log(1/\delta))$ we can find $S'\subset  [0,1]$ of size $|S'|=\poly(k,\log(1/\delta))$ and diagonal $D'\in \mathbb{R}^{|S'|\times |S'|}$  such that the symmetric Toeplitz matrix $T' = F_{S'}D' F_{S'}^*$ \Cam{$F_{S'}$ is not defined here.} satisfies, with probability at least $0.9$,
	%\begin{equation*}
	%	\|T- T'\|_F \lsim \max\{\|E\|_F,\|T-T_k\|_F\} + \delta \|T\|_F.
	%\end{equation*}
	%where $T_k = \argmin_{B: rk(B)\leq k}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm.
%\end{reptheorem}
\textbf{Heavy Light decomposition.} To prove Theorem \ref{thm:sublinear_time_recovery}, we consider the first column $\wt T_1=\wt T_{[0:d,0]}$ \Cam{Well it is a sparse Fourier function. We don't just interpret it that way.} of $\wt T=F_{\wt S}\wt D F_{\wt S}^*$ as guaranteed to exist by Theorem \ref{frobeniusexistence} for a small constant $\epsilon$, say $\epsilon=0.1$. From Theorem \ref{frobeniusexistence}, it can be seen that $\wt T_1$ is a $\wt O(k)$-Fourier sparse function, whose support in Fourier domain is exactly the frequencies $\wt S$ in the Vandermonde decomposition of $\wt T =F_{\wt S}\wt D F_{\wt S}^*$. Thus we can hope to apply Lemma \ref{lem:dtft_freqrecovery} to $\wt T_1$ to approximately recover frequencies in the Vandermonde decomposition of $\wt T$. \Cam{This is confusing. These are the heavy frequencies in the function right? Should be more clear about how the sparse function relates to the Vandermonde decomp.}. After this step, we can then hope to regress onto these heavy frequencies as returned by Lemma \ref{lem:dtft_freqrecovery} and recover a good approximation to $\wt T$ in the Frobenius norm. \Cam{Needs more context. Low rank approx to what? Constant factor in what metric?} There are several challenges on the way to implement this ideal plan. First, if we denote the noise on $\wt T$ to be $E^k=T+E-\wt T$ we can only assume that $\|E^k\|_F$ is small compared to $\|\wt T\|_F$ (the other case is handled easily and is described later in this overview). However the noise may very well concentrate on the first column $\wt T_1$. More formally, we can assume $\|E^k\|_F\leq c\|\wt T\|_F$ for a small enough constant $c>0$, however it could be that $\|E^{k}_{[0:d,0]}\|_2 \gg c\|\wt T_{[0:d,0]}\|_2$ thus barring us from applying Lemma \ref{lem:dtft_freqrecovery} on $\wt T_1$. We can instead consider picking a random column $i\sim [d]$, and can argue by Markov's inequality that $\|E^k_{[0:d,i]}\|_2 \leq 10 \|E^k\|_F/\sqrt{d}\leq 10 c\|\wt T\|_F/\sqrt{d}$, with probability $0.9$. However if the $\ell_2$ norm $\|\wt T_{[0;d,i]}\|_2$ is extremely small compared to $\|\wt T\|_F/\sqrt{d}$ then we still cannot conclude that $\|E^k_{[0:d,i]}\|_2\lsim c \|\wt T_{[0:d,i]}\|_2$ which is required for Lemma \ref{lem:dtft_freqrecovery}. This can happen for example when the bottom left entry $\wt T_{[d,0]}$ is extremely large and the rest of the entries of $\wt T$ are very small and thus $\|\wt T_{[0:d,i]}\|_2$ is extremely small compared to $\|\wt T\|_F$ for all $i$ except $i=0,d$. However we show that this cannot happen when 
$\wt T$ is (almost) PSD and Toeplitz, which is guaranteed for us from Theorem \ref{frobeniusexistence}. Formally we show the following lemma.
\begin{lemma}\label{lem:smallnoisefirstcol}
	Let $\wt T$ be a $d\times d$ symmetric Toeplitz matrix, and suppose that there exists a PSD Toeplitz matrix $T$ satisfying $\|\wt T- T\|_F \leq 0.001 \|T\|_F$. 
    Then the following holds,
	\begin{equation*}
		\|\wt T_{[0:d/2,0]}\|_2\geq \frac{0.49}{\sqrt{d}} \|\wt T\|_F.
	\end{equation*}
\end{lemma}
The proof of this lemma relies on a norm compression inequality of Audenaert \cite{audenaert2006norm}. The previous lemma says that if $\wt T$ has large Frobenius norm, then any $i^{th}$ column for $i\in [d/2]$ has large $\ell_2$ norm as well, because any such $i^{th}$ column has its $d/2$ entries $\wt T_{[i:i+d/2,i]}=\wt T_{[0:d/2,0]}$ (since $\wt T$ is Toeplitz) so its norm $\|\wt T_{0:d,i}\|_2$ is atleast $\|\wt T_{[i:i+d/2,i]}\|_2=\|\wt T_{[0:d/2,0]}\|_2\gsim \|\wt T\|_F/\sqrt{d}$.
%  %Morever $\wt T_i$'s Fourier transform is identical to $\wt T_1$ upto a time shift, thus we can still hope to run Lemma \ref{lem:dtft_freqrecovery} on it.

We now describe the second issue, which is that even if we could run Lemma \ref{lem:dtft_freqrecovery} on $\wt T_{[0:d,i]}$, we can only guarantee that the $\ell_2$ norm of the signal corresponding to the unrecoverable ``light'' frequencies in the Fourier spectrum of $\wt T_{[0:d,i]}$(i.e., those not satisfying the requirement of Lemma \ref{lem:dtft_freqrecovery}) is small. This implies that the $\ell_2$ norm of the $i^{th}$ column of the matrix $\wt T^{light}$ defined to be the Toeplitz matrix whose Vandermonde decomposition only contains these ``light'' frequencies is small. However, to recover a good approximation to the whole matrix $\wt T$, we need to ensure that the Frobenius norm of $\wt T^{light}$ is small. We are able to show that $\wt T^{light}$ is also almost PSD. Thus invoking Lemma \ref{lem:smallnoisefirstcol} we can argue that $\|\wt T^{light}\|_F\lsim \sqrt{d}\|\wt T^{light}_{[0:d/2,0]}\|_2\leq \sqrt{d}\|\wt T^{light}_{[0:d,i]}\|_2$ for any $i\in [d/2]$, where the last inequality follows from the fact that $\wt T^{light}$ is symmetric Toeplitz thus $\|\wt T^{light}_{[0:d/2,0]}\|_2=\|\wt T^{light}_{[i:i+d/2,i]}\|_2\leq \|\wt T^{light}_{[0:d,i]}\|_2$.

\begin{comment}
This suggests the following strategy. We sample a random column $i\sim [d/2]$. We want to apply Lemma \ref{lem:dtft_freqrecovery} to $\wt T_{[0:d,i]}$. A small caveat is that this column is identical to $\wt T_{[0:d,0]}$ upto a time-shift, and thus their Fourier spectrum is different. To simplify this we only work with the $d/2$ sized chunk $\wt T_{[i:i+d/2,i]}$ of the $i^{th}$ column, which by the virtue of $\wt T$ being Toeplitz is equal to $\wt T_{[0:d/2,0]}$. Using Markov's inequality we can show that the noise on this chunk of the $i^{th}$ column is small, i.e., $\|E^{k}_{[i:i+d/2,i]}\|_2 \lsim \|E^k\|_F/\sqrt{d}\leq c\|\wt T\|_F/\sqrt{d}$. Moreover from Lemma \ref{lem:smallnoisefirstcol} $\|\wt T_{[i:i+d/2,i]}\|_2=\|\wt T_{[0:d/2,0]}\|_2\gsim \|\wt T\|_F/\sqrt{d}$. Thus we get that $\|E^{k}_{[i:i+d/2,i]}\|_2 \lsim c\|\wt T_{[i:i+d/2,i]}\|_2$ with probability at least $0.9$, enabling us to apply Lemma \ref{lem:dtft_freqrecovery} to this length $d/2$ signal. Let $\wt T^{light}$ be the Toeplitz matrix corresponding to unrecoverable light frequencies in the spectrum of $\wt T_{[i:i+d/2,i]}=\wt T_{[0:d/2,0]}$, i.e., those not satisfying the condition of Lemma \ref{lem:dtft_freqrecovery} for noise $E^{k}_{[i:i+d/2,i]}$. We can then bound the $\ell_2$ norm of the length $d/2$ signal $\wt T^{light}_{[i:i+d/2,i]}=\wt T^{light}_{[0:d/2,0]}$ using the properties of the $H$ function as per equations \ref{eqn:H_properties_summary} and also show using the existence result of Theorem \ref{frobeniusexistence} that $\wt T^{light}$ is almost PSD (in the sense of Lemma \ref{lem:smallnoisefirstcol}). Combining these with Lemma \ref{lem:smallnoisefirstcol} we can show that $\wt T^{light}$ thus has small Frobenius mass. 
\end{comment}
This gives us a ``heavy-light'' decomposition of $\wt T=\wt T^{heavy}+\wt T^{light}$ where the Fourier sparse spectrum of $\wt T^{heavy}$ is approximately recoverable and $\wt T^{light}$ has low Frobenius mass. This is formalized below.
\begin{lemma}\label{lem:heavy_freq_recovery}
Consider the input setup of Theorem \ref{thm:sublinear_time_recovery}. Let $\wt T = F_{\wt S} \wt D F_{\wt S}^*$ be as guaranteed to exist by Theorem \ref{frobeniusexistence} for $T$, $\epsilon=0.1$, $\delta$ and $k$. \Cam{I don't love the notation $E^k$. It implies it is rank-k or something like that.} Let $E^k= E+T-\wt T$. Assume $\|E^k\|_F \leq c\|\wt T\|_F$ for some small enough constant $c>0$. Then in $\poly(k,\log(d/\delta))$ time we can find a list of frequencies $L \subseteq [0,1]$ of size $|L| = \poly(k,\log d)$ satisfying the following with probability 0.9 - Let $S_{heavy}\subseteq \wt S$ defined as follows, $$S_{heavy}= \{f\in \wt S: \exists f'\in L \text{ s.t. } |f-f'|_{\circ}\leq \poly(k,\log(d/\delta))/d \}.$$ Let $D^{heavy}$ containing the entries of $\wt D$ corresponding to $S_{heavy}$, and $\wt T^{heavy} = F_{S^{heavy}} D^{heavy}F_{S^{heavy}}^{*}$. Then $\wt T^{light} = \wt T - \wt T^{heavy}$ satisfies  $$\|\wt T^{light}\|_F \lsim \|E^k\|_F + \delta \|T\|_F.$$
\end{lemma}
The proof of Lemma \ref{lem:smallnoisefirstcol} and Lemma \ref{lem:heavy_freq_recovery} are presented in Section \ref{subsection:heavy_light_decomp}.
\\

\textbf{Noisy Toeplitz Recovery.} Equipped with the previous heavy-light decomposition of Lemma \ref{lem:heavy_freq_recovery}, we can hope to use the set of recovered frequencies $L$ to find an approximation to $\wt T^{heavy}$ and thus to $\wt T$ with low error in the Frobenius norm using a sublinear time approximate regression primitive and prove Theorem \ref{thm:sublinear_time_recovery}. This needs to be done carefully and we now describe the key ideas behind the proof. Theorem \ref{frobeniusexistence} guarantees that the frequencies $\wt S$ in the Vandermonde decomposition of $\wt T$ and thus in $\wt T^{heavy}$ have a certain structure. In particular, every $f\in S^{heavy}\subseteq \wt S$ is of the form $f=(2i-1)/2d + \gamma j$ for some integers $i\in [d]$ and $j\in [-\wt O(\log(1/\delta)),\wt O(\log(1/\delta))]$. Here $\gamma$ is a fixed number per Theorem \ref{frobeniusexistence}. Also assuming $\|E^k\|_F\leq c\|\wt T\|_F$, from Lemma \ref{lem:heavy_freq_recovery} we know that we have approximately recovered every $f\in S^{heavy}$, that is for every such $f$ there exists an $f'\in L $ such that $|f-f'|_{\circ}\leq \poly(k,\log(1/\delta))/d$. Thus we can set up intervals of size $ \poly(k,\log(1/\delta))/d$ around each $f'\in L$ and let $S(L)$ be the set of all $f$ in these intervals of the form $f=(2i-1)/2d + \gamma j$ for some integers $i\in [d]$ and $j\in [-\wt O(\log(1/\delta)),\wt O(\log(1/\delta))]$. Then we know that $S^{heavy}\subseteq S(L)$ and by definition of $S(L)$, $|S(L)|\leq \poly(k,\log(1/\delta))$. This implies that if study the following regression problem $\min_{D:D \text{ is diagonal }}\|T+E- F_{S(L)}DF_{S(L)}^*\|_F$, then it satisfies the following.
\begin{align*}
	\min_{D:D \text{ is diagonal }}\|T+E- F_{S(L)}DF_{S(L)}^*\|_F &\leq \|T+E-\wt T^{heavy}\|_F\\
 &\leq \|E\|_F+ \|T-\wt T\|_F + \|\wt T- \wt T^{heavy}\|_F\\
 &=\|E\|_F+ \|T-\wt T\|_F + \|\wt T^{light}\|_F\\
 &\lsim \|E\|_F + \|T-T_k\|_F +\delta \|T\|_F
\end{align*}
where the last line followed by upper bounding $\|\wt T^{light}\|_F$ from point 2. of Lemma \ref{lem:heavy_freq_recovery} and upper bounding $\|T-\wt T\|_F$ from point 1. of Theorem \ref{frobeniusexistence}. However we need to worry about the case when $\|E^k\|_F\geq c \|\wt T\|_F$, that is when the noise is noticeably larger than the input and the output of Lemma \ref{lem:heavy_freq_recovery} does not approximate the frequencies of $S^{heavy}$. However in this case the above regression problem might as well output $D=0$ as the noise is very high, and one can still show $$\min_{D:D \text{ is diagonal }}\|T+E- F_{S(L')}DF_{S(L')}^*\|_F\lsim \|E\|_F + \|T-T_k\|_F +\delta \|T\|_F.$$
Finally using techniques based on leverage score sampling for Fourier sparse functions from \cite{kapralov2022toeplitz} and \cite{eldar2020toeplitz}, we can solve this regression problem upto constant factor accuracy in $\poly(k,\log(1/\delta))$ time. The output of this approximate regression problem will be a symmetric Toeplitz matrix (since it is of the form $F_{S(L)}DF_{S(L)}^*$) and this then finishes the proof of Theorem \ref{thm:sublinear_time_recovery}. The details are presented in Section \ref{subsection:noisy_toeplitz_recovery}. Finally, equipped with the robust low-rank approximation result of Theorem \ref{thm:sublinear_time_recovery}, the proofs of Theorem \ref{thm:sublinear_time_lowrankapprox} and \ref{thm:sublinear_time_covariance_estimation} are presented in Section \ref{subsection:toeplitz_applications}.
\\
\begin{comment}
\subsection{\Cam{This should be removed.}}
\Cam{I would like to remove this section entirely. Let's discuss in person.}
\textbf{Low-rank approximation and Covariance estimation.}
Now we move on to giving the main ideas behind the sublinear time low rank approximation and covariance estimation results of Theorems \ref{thm:sublinear_time_lowrankapprox} and \ref{thm:sublinear_time_covariance_estimation} respectively. Firstly, equipped with Theorem \ref{thm:sublinear_time_recovery} Theorem \ref{thm:sublinear_time_lowrankapprox} follows easily by setting $E=0$. 

\Cam{This is out of place. This should be in the part where you prove Theorem 3.}
Now recall the setting of Theorem \ref{thm:sublinear_time_covariance_estimation}. In this setting we do not have direct access to the entries of $T$. Instead, we are given samples $x_1,x_2,\ldots, x_s \sim \mathcal{N}(0,T)$, where the covariance $T$ is a $d\times d$ PSD Toeplitz matrix. The goal here is to learn $T$ approximately from having access to $x_1,\ldots, x_s$, while minimizing the number of samples $s$ (this is referred to as the Vector Sample Complexity) \Cam{This should be defined in the intro, not here.} and the number of entries read from each sample $x_i$ (this is referred to as the Entry Sample Complexity).  Applying Theorem \ref{thm:sublinear_time_recovery} to this setting therefore will require more care.
The first claim of this section stated below essentially argues that $s=\poly(k)$ samples suffices to learn the top-$k$ eigenspace of the covariance $T$ approximately, thus being a more general robust version of the fact that $\poly(d)$ samples are necessary and sufficient to learn the full covariance $T$. This allows us to control how far the empirical covariance matrix is from the true covariance matrix in Frobenius norm, allowing us to then instantiate Theorem \ref{thm:sublinear_time_recovery}.

\kstodo{need to also highlight improvement over the existence proof of ELLM'20}
To prove this lemma, we use matrix concentration inequalities and tools from randomized numerical linear algebra such as Projection Cost Preserving (PCP) sketch property of the Gaussian distribution \cite{cohen2015dimensionality}. The complete proof is presented in Section 5. \Cam{I'm not sure why we need this. Don't we just need to bound the norm of $E = XX^T - T$ to apply Theorem 1? I don't get where this triangle inequality statement is being used?} An important point here is that this Lemma \ref{lem:low_rank_concentration} combined with the Toeplitz low-rank approximation existence result of Theorem \ref{frobeniusexistence} imply the following by triangle inequality,
\begin{equation}\label{eqn:low_rank_empirical_existence}
    \|XX^T - F_{\wt S}\wt D F_{\wt S}\|_F \lsim \sqrt{\|T-T_k\|_2 \tr(T)+ \frac{\|T-T_k\|_F \tr(T)}{k}}+ \epsilon \|T\|_2
\end{equation}
where $X$ is as per the statement of Lemma \ref{lem:low_rank_concentration} and $F_{\wt S}\wt D F_{\wt S}=\wt T$ is as per the statement of Theorem \ref{frobeniusexistence} applied to $T$ and $\epsilon=O(1)$. This significantly strengthens the analogous result of Lemma 5.6 of \cite{eldar2020toeplitz} who were only able to show $XX^T$ is well approximated by a matrix spanned by some Fourier frequencies, but equation \ref{eqn:low_rank_empirical_existence} by shows that $XX^T$ is infact well approximated by a very structured object - a low rank Toeplitz matrix.

Equipped with the previous lemma, we can instantiate Theorem \ref{thm:sublinear_time_recovery} with $E=XX^T-T$ to prove our sublinear time covariance estimation result of Theorem \ref{thm:sublinear_time_covariance_estimation}. Note that the error guarantees of Theorem \ref{thm:sublinear_time_covariance_estimation} match the guarantees of the algorithm of \cite{eldar2020toeplitz} for this problem as per Theorem 2.10 in \cite{eldar2020toeplitz}, but our algorithm runs in sublinear time thus resolving their main open problem.
\Cam{As in the othe theorems, remove $r$ as it is not needed.}
The details of the proofs of Lemma \ref{lem:low_rank_concentration} and Theorem \ref{thm:sublinear_time_covariance_estimation} are presented in Section \ref{subsection:toeplitz_applications}.
\end{comment}

\subsection{Other related work}\label{sec:prior} 
\kstodo{Mostly taken from previous soda paper!}
A large body of work in numerical linear algebra, applied mathematics, theoretical computer science, and signal processing  has studied the problem of computing low-rank approximations of Toeplitz and Hankel matrices \cite{Luk:1996ur,Park:1999ta,Ishteva:2014wm,Cai:2016wh,Ongie:2017us,Krim:1996wm,Shi:2019ud}. In many applied signal processing settings, Toeplitz matrices arise as PSD covariance matrices, motivating our focus on the PSD case.
%Using the FFT, any $d \times d$ Toeplitz matrix can be multiplied by a vector in  $O(d \log d)$ time. \cite{Shi:2019ud} show how to use this  primitive to give a near-linear time, near-optimal low-rank approximation algorithm for Toeplitz matrices. In particular, their algorithm outputs $\wt T$ with rank $k$ satisfying $\norm{T-\wt T}_F \le (1+\epsilon) \norm{T-\tilde T}_F$ in $\tilde O(d + \poly(k/\epsilon))$ time. Note that $\wt T$ here may not be Toeplitz.
Significant prior work has also studied the problem of computing an optimal \emph{structure-preserving} Toeplitz low-rank approximation, where the low-rank approximation $\wt T$ is itself required to be Toeplitz. However, no simple characterization of the optimal solution to this problem is known \cite{chu2003structured} and polynomial time algorithms  are only known in the special cases of $k= 1$ and $k = d-1$ \cite{chu2003structured,Knirsch:2021ve}. On the practical side a range of heuristics are known, based on techniques such as convex relaxation \cite{Fazel:2013vw,Cai:2016wh,Ongie:2017us}, alternating minimization \cite{chu2003structured,Wen:2020ub}, and sparse Fourier transform \cite{Krim:1996wm}. 

%\cite{Park:1999ta,Ishteva:2014wm}. %Many works focus on computationally efficient, but not sublinear algorithms that output a good Toeplitz low-rank approximation to the input. 
%\cite{Wen:2020ub} matrix comlpetion alternatiing svd typo algorithm.

Many results in the signal processing literature study sublinear query algorithms for Toeplitz matrices, these are referred to as \emph{sparse array methods} which proceed by querying a small principal submatrix to obtain an approximation to the whole matrix \cite{Abramovich:1999vs,Chen:2015wz,Qiao:2017tp,Lawrence:2020ut}. The work of \cite{eldar2020toeplitz} and \cite{kapralov2022toeplitz} on sublinear query PSD Toeplitz low-rank approximation and Toeplitz covariance estimation is closely related to this literature. %give sublinear query algorithms for various problems on Toeplitz matrices as discussed in the introduction.
%
%
%Several of these works focus on algorithms with sublinear query complexity \cite{Lawrence:2020ut} \cite{Qiao:2017tp}
%
%%\cite{Ongie:2017us} convex relaxation
%
%%\cite{Park:1999ta} -- not really sure the method
%
%%\cite{Knirsch:2021ve} -- optimal rank-1 paper.
%
%
%%Structured low rank approximation \cite{chu2003structured}.
%%\begin{itemize}
%%%\item \url{https://www.cas.mcmaster.ca/~qiao/publications/LQV02.pdf}
%%%\item \url{http://www.cas.mcmaster.ca/~qiao/publications/LQ96b.pdf}
%%%\item \url{https://journalofinequalitiesandapplications.springeropen.com/track/pdf/10.1186/s13660-020-02340-w.pdf}
%%%\item \url{https://ieeexplore.ieee.org/document/8715594}
%%%\item \url{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC5999344/}
%%%\item \url{https://conservancy.umn.edu/handle/11299/215327}
%%%\item \url{https://www.math.colostate.edu/~king/codex/slides/Plonka_2020_11_03.pdf} lots of good refs. Optimal rank-1 solution. Also optimal solution in infinite operator case.
%%\item \url{https://mtchu.math.ncsu.edu/Research/Lectures/Iep/chapter8.pdf} states that optimal Toeplitz low-rank approximation is open.
%%\end{itemize}
%

Beyond Toeplitz matrices, significant recent work has focused on  sublinear time low-rank approximation algorithms for other structured matrix classes. This includes positive semidefinite matrices \cite{musco2017recursive,Bakshi:2020tl}, distance matrices \cite{Bakshi:2018ul,Indyk:2019vy}, and kernel matrices \cite{musco2017recursive,Yasuda:2019vf,Ahle:2020vj}.

%Our techniques also rely on sublinear time algorithms for sparse Fourier recovery problems. There is a large body of work on sparse discrete fourier transforms, that are concerned with computing $k$-Fourier sparse approximations to discrete time signals of period $d$ in $\wt O(k)$ time \cite{hassanieh2012nearly,indyk2014sample,indyk2014nearly,kapralov2016sparse,chen2016fourier}. Most relevant to our work is the work of \cite{chen2016fourier}, which obtained $\poly(k,\log d)$-Fourier sparse approximations on a bounded interval $[0,d]$ to $k$-Fourier sparse functions with arbitrary frequencies, thus not necessarily periodic, in $\poly(k,\log d)$ time given access to the input on the entire interval $[0,d]$.














==> last_intro_checkpoint.tex <==
% !TEX root = ./main.tex

%\Cam{Captialization of section titles should be made consistent. One some of them we use caps for all words, on some for just the first word.}

\section{Introduction}

%\Cam{We need more citation in this first paragraph. They can be drawn from prior work}
A Toeplitz matrix $T\in \mathbb{R}^{d\times d}$ is constant along each of its diagonals. I.e., $T_{i,j}=T_{k,l}$ for all $i,j,k,l$ with $i-j=k-l$. These highly structured  matrices arise in many fields, including signal processing, scientific computing, control theory, approximation theory, and machine learning -- see \cite{Bunch:1985ti} for a survey. In particular, Toeplitz matrices often arise as the covariance matrices of stationary signals, when the covariance structure is shift invariant. I.e., when the covariance between measurements only depends on their distance in space or time \cite{Gray:2006ta}. A row-reversed Toeplitz matrix is known as a Hankel matrix. Such matrices also find broad applications \cite{Fazel:2013vw,Munkhammar:2017ud,Ghadiri:2023tv}. %Toeplitz matrices also arise in control theory, approximation theory, the study of orthogonal polynomials and partial differential equations \cite{Bunch:1985ti}.

Given their importance, significant work has studied fast algorithms for basic linear algebraic tasks on Toeplitz matrices. A $d \times d$ Toeplitz matrix can be multiplied by a vector in just  $O(d\log d)$ time using the fast Fourier transform. Toeplitz linear systems can be solved in $O(d^2)$ time exactly using Levinson recursion \cite{Golub:2013wp}, and to high-precision in $O(d\cdot \polylog d)$ time using randomization  \cite{XiXiaCauley:2014,XiaXiGu:2012}. A full eigendecomposition can be computed in $O(d^2\cdot \polylog d)$ time \cite{pan1999complexity}. 

\subsection{Sublinear query algorithms for Toeplitz matrices} 

Recent work has focused on algorithms for Toeplitz matrices with complexity scaling \emph{sublinearly} in the dimension $d$ \cite{Abramovich:1999vs,Chen:2015wz,Qiao:2017tp,Wu:2017ub,Lawrence:2020ut,eldar2020toeplitz,kapralov2022toeplitz}. Kapralov et al. \cite{kapralov2022toeplitz} study low-rank approximation of positive semidefinite (PSD) Toeplitz matrices. They show that by accessing just $\poly(k,\log(d/\delta),1/\epsilon)$ entries of a PSD Toeplitz matrix $T \in \R^{d \times d}$, one can compute a symmetric Toeplitz matrix $\wt T$ with rank $\tilde O(k \log(1/\delta)/\epsilon)$ such that:\footnote{Throughout we use $\tilde O(\cdot)$ to hide polylogarithmic factors in the dimension $d$ and in the argument.}  
\begin{align}\label{eq:nearRelative}
\|T-\wt{T}\|_F \leq (1+\eps)\|T-T_k\|_F + \delta\|T\|_F,
\end{align}
where $\norm{M}_F = \sqrt{\sum_{i=1}^d \sum_{j=1}^d M_{ij}^2}$ is the Frobenius norm and $T_k = \underset{B:\rank(B)\leq k}{\argmin}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm, given by projecting $T_k$ onto its top $k$ eigenvectors. %$\wt T$ gives a near-optimal \emph{structure preserving} low-rank approximation of $T$. %Observe that since the dependence on $\delta$ is logarithmic, the optimality guarantee is near relative error.

Observe that $T_k$ may not itself be Toeplitz and it is not a priori clear that Toeplitz $\wt T$ satisfying \eqref{eq:nearRelative} even exists. The key technical contribution of \cite{kapralov2022toeplitz} is to prove that it does, and further that $\wt T$ can be recovered using sample efficient off-grid sparse Fourier transform techniques. Unfortunately, despite its sample efficiency, the algorithm of \cite{kapralov2022toeplitz} is computationally inefficient, with runtime that is  exponential in $\tilde O(k \polylog(d)/\epsilon)$  --  i.e., at least $d^{\tilde O(k/\epsilon)}$. The main open question left by their work is if this runtime can be improved, giving a sublinear time, not just a sublinear query, algorithm. %Roughly, the columns of $\wt T$ are spanned by $\tilde O(k/\epsilon)$ off grid frequencies, and the algorithm must perform a brute-force-search to identify these frequencies.

Eldar et al. \cite{eldar2020toeplitz} study the related problem of recovering an (approximately) low-rank Toeplitz covariance matrix $T \in \R^{d \times d}$ given independent samples from the $d$-dimensional Gaussian $\mathcal{N}(0,T)$. Low-rank Toeplitz covariance estimation is widely applied in signal processing, including in  direction of arrival (DOA) estimation  \cite{krim1996two}, spectrum sensing for cognitive radio \cite{ma2009signal,cohen2018analog}, and medical and radar image processing \cite{snyder1989use,ruf1988interferometric,fuhrmann1991application,brookes2008optimising,asl2012low,cohen2018sparse}. 
%
%We now turn to the work of \cite{eldar2020toeplitz} who also developed sublinear query algorithms in the context of Toeplitz matrices. The work of \cite{eldar2020toeplitz} is concerned with the following problem - given $s$ i.i.d. samples $x^1,x^2,\ldots, x^s$ from a $d$ dimensional Gaussian $\mathcal{N}(0,T)$ with covariance $T$ that is Toeplitz, estimate $T$ upto some error threshold. This problem statement is not only more realistic since the algorithm only has \emph{noisy} implicit access to $T$ via the i.i.d. samples as opposed to the setup of Theorem \ref{thm:sublinear_lra_soda2023}, but also it is directly relevant to practical applications. Toeplitz covariance structure emerges for example when the random measurement vector corresponds to measurements on a spatial or temporal grid, and the covariance between two coordinates just depends on the difference between them. Fast algorithms for this problem of estimating Toeplitz covariance matrices have many applications ranging from Direction of Arrival (DOA) estimation for signals received from antenna arrays \cite{krim1996two}, spectrum sensing for cognitive radio \cite{ma2009signal,cohen2018analog}, medical and radar image processing \cite{snyder1989use,ruf1988interferometric,fuhrmann1991application,brookes2008optimising,asl2012low,cohen2018sparse}. 
Motivated by these applications, \cite{eldar2020toeplitz} consider two relevant sample complexity measures: the vector sample complexity (VSC), which is the number of samples (each a vector in $\R^d$) taken from the distribution $\mathcal{N}(0,T)$, and the entry sample complexity (ESC), which is the number of entries read from each vector sample. % and runtime. We encapsulate the definitions of these complexity measures in the following definition, which we will refer to recurringly in the paper. 
%\begin{definition}\label{def:vsc_and_esc}
%Given $s$ i.i.d. samples $s$ of the form $x^1,x^2,\ldots,x^s \sim \mathcal{N}(0,T)$ consider any algorithm which estimates $T$ upto some specified error tolerance using these samples. The Vector sample complexity (VSC) is the number of i.i.d. samples $s$ of the form $x^1,x^2,\ldots,x^s \sim \mathcal{N}(0,T)$ an algorithm uses and the Entry sample complexity (ESC) is the number of entries the algorithm reads from each sample $x^i$ for $i\in [s]$.  
%\end{definition}
\cite{eldar2020toeplitz} show that with $\poly(k,\log d,1/\epsilon)$ VSC and ESC, it is possible to return $\wt T$ satisfying with high probability:\footnote{Throughout, we let $f(\cdot) \lsim g(\cdot)$ denote that $f(\cdot) \le c \cdot g(\cdot)$ for some fixed constant $c$.}
%The main result of \cite{eldar2020toeplitz} is to achieve a sublinear, i.e. $o(d)$, VSC and ESC, this is formalized below.
%\begin{theorem}[Theorem 2.10 in \cite{eldar2020toeplitz}]\label{thm:elmm_soda20}
%There is an algorithm such given i.i.d samples $x^1,x^2,\ldots, x^s\sim \mathcal{N}(0,T)$ for PSD Toeplitz $T\in \mathbb{R}^{d\times d}$ and parameters $k,\epsilon>0$, it has VSC $s=\wt O(k+1/\epsilon^2)$, ESC $\wt O(k^2\log(1/\epsilon))$ and returns a Toeplitz $\wt T$ satisfying the following with probability $0.9$,
\begin{equation}\label{eq:sampleBound}
    \|T-\wt T\|_2 \lsim \sqrt{\|T-T_k\|_2 \cdot  \tr(T)+ \frac{\|T-T_k\|_F \tr(T)}{k}} + \epsilon \|T\|_2,
\end{equation}
where $\tr(T)$ is the trace and $\norm{T}_2$ is the spectral norm.
%\end{theorem}
While the above error bound may seem somewhat non-standard,  \cite{eldar2020toeplitz} show that it implies fairly strong bounds when $T$ has low stable-rank. Observe that when $T$ is exactly rank-$k$, the error bound becomes $\epsilon \norm{T}_2$. As in \cite{kapralov2022toeplitz}, a key drawback is that algorithm of \cite{eldar2020toeplitz} has runtime scaling exponentially in  $\tilde O(k \polylog d)$. Further,   the output matrix $\wt T$ is not itself guaranteed to be low-rank.

%The main drawbacks of this result are that the runtime of the algorithm is $\exp(k)$ and the output Toeplitz $\wt T$ as per the Theorem then is not guaranteed to be low-rank. The error bound may seem non-standard as well, however \cite{eldar2020toeplitz} show that it implies fairly strong bounds when $T$ has low stable-rank.

\subsection{Our contributions}

In this work, we give a \emph{sublinear time} algorithm for computing a near-optimal low-rank approximation of a PSD Toeplitz matrix given noisy access to its entries. Our robust low-rank approximation primitive can be applied in the settings of both \cite{kapralov2022toeplitz} and \cite{eldar2020toeplitz}, yielding the first sublinear time algorithms for both standard PSD Toeplitz low-rank approximation and low-rank Toeplitz covariance estimation. Our main result is as follows:
\begin{theorem}[Robust Sublinear Time Toeplitz Low-Rank Approximation]\label{thm:sublinear_time_recovery}
	Let $T\in \mathbb{R}^{d\times d}$ be a PSD Toeplitz matrix, $E\in \mathbb{R}^{d\times d}$ be an arbitrary noise matrix, $\delta>0$ be an error parameter, and $k$ be an integer rank parameter. There exists an algorithm that, given query access to the entries of $T+E$, runs in $\poly(k,\log(d/\delta))$ time and outputs a representation of symmetric Toeplitz matrix $\wt T$ with rank $\poly(k,\log(d/\delta))$ that satisfies, with probability at least $0.9$,
	\begin{equation*}
		\|T- \wt T\|_F \lsim \max\{\|E\|_F,\|T-T_k\|_F\} + \delta \|T\|_F,
	\end{equation*}
	where $T_k = \argmin_{B: \rank(B)\leq k}\|T-B\|_F$ is the best rank-$k$ approximation to $T$.
\end{theorem}
Observe that given our runtime, which depends just poly-logarithmically on the input dimension $d$, it is not possible to output $\wt T \in \R^{d \times d}$ explicitly. Thus, our algorithm outputs a compressed representation of $\wt T$. To do so, we use the well known Vandermonde decomposition theorem, which states that any Toeplitz matrix can be diagonalized by a Fourier matrix \cite{cybenko1982moment}. We can show that $\wt T$ in particular, which has rank $r = \poly(k,\log(d/\delta))$, can be written as  $FDF^*$ where $F \in \mathbb{C}^{d\times r}$ is a Fourier matrix, with $j^{th}$ column given by $[1, e^{2\pi i \cdot f_j}, e^{2\pi i \cdot 2f_j},\ldots, e^{2\pi i  \cdot (d-1) f_j}]$ for some frequency $f_j$, and $D \in \R^{r \times r}$ is diagonal. Our algorithm outputs the frequencies $f_1,\ldots,f_r$ and diagonal entries $D_{1,1},\ldots,D_{r,r}$, which fully determine $\wt T$.

As an immediate consequence of Theorem \ref{thm:sublinear_time_recovery} applied with $E=0$, we obtain the following sublinear time constant factor low-rank approximation algorithm for PSD Toeplitz matrices, which resolves the main open problem of \cite{kapralov2022toeplitz} for the case of constant factor approximation.
\begin{theorem}[Sublinear Time Toeplitz Low-Rank Approximation]\label{thm:sublinear_time_lowrankapprox}
Let $T\in \mathbb{R}^{d\times d}$ be a PSD Toeplitz matrix, $k$ be an integer rank parameter, and $\delta>0$ be an error parameter. There exists an algorithm that, given query access to entries of $T$, runs in  $\poly(k,\log(d/\delta))$ time and outputs a representation of symmetric Toeplitz matrix $\wt T$ with rank $\poly(k,\log(d/\delta))$ that satisfies with probability at least 0.9,
	\begin{equation*}
		\|T- \wt T\|_F \lsim \|T-T_k\|_F + \delta \|T\|_F.
	\end{equation*}
	%where $T_k = \argmin_{B: \rank(B)\leq k}\|T-B\|_F$ is the best rank-$k$ approximation to $T$.
\end{theorem}
We can further apply Theorem \ref{thm:sublinear_time_recovery} to the Toeplitz covariance estimation setting of \cite{eldar2020toeplitz}. Here, we set $E=\frac{1}{s} \cdot XX^T -T$ where $X \in \R^{d \times s}$ has $s$ columns sampled i.i.d. from the multivariate Gaussian distribution $\mathcal{N}(0,T)$. That is, $E$ is the error between the true covariance matrix $T$ and a sample covariance  matrix $\frac{1}{s} XX^T$ that our algorithm can access. Using similar ideas to \cite{eldar2020toeplitz}, we show that for $s = \tilde O(k^4/\epsilon^2)$, $\norm{E}_F \lsim \sqrt{\|T-T_k\|_2 \tr(T)+ \frac{\|T-T_k\|_F \tr(T)}{k}} + \epsilon \|T\|_2$. Combined with Theorem \ref{thm:sublinear_time_recovery} applied with $\delta = \epsilon/\sqrt{d}$ so that $\delta \norm{T}_F \le \epsilon \norm{T}_2$, this gives:
\begin{theorem}[Sublinear Time Toeplitz Covariance Matrix Estimation]\label{thm:sublinear_time_covariance_estimation}
	Let $T\in \mathbb{R}^{d\times d}$ be a PSD Toeplitz matrix, $k$ be an integer rank parameter, and $\epsilon > 0$ be an error parameter. There is an algorithm that given i.i.d. samples $x^1,\ldots, x^s \sim \mathcal{N}(0,T)$ for $s=\tilde O(k^4/\epsilon^2)$, runs in $\poly(k,\log (d/\epsilon))$ time and outputs a representation of symmetric Toeplitz $\wt T$with rank $\poly(k,\log(d/\epsilon))$ satisfying, with probability at least 0.9,
	\begin{equation*}
		\|T- \wt T\|_F \lsim \sqrt{\|T-T_k\|_2 \tr(T)+ \frac{\|T-T_k\|_F \tr(T)}{k}} + \epsilon \|T\|_2.
	\end{equation*}
	Further, the algorithm has entry sample complexity (ESC) $\poly(k,\log (d/\epsilon))$ --  it reads just  $\poly(k,\log (d/\epsilon))$ entries of each vector sample $x^i$.
\end{theorem}
Observe that the error guarantee of
Theorem \ref{thm:sublinear_time_covariance_estimation} is at least as strong, and can potentially be much stronger, than that of \eqref{eq:sampleBound}, since the bound is on $\norm{T-\wt T}_F$ rather than $\norm{T - \wt T}_2$. At the same time, our algorithms achieves the same vector and entry sample complexities as \cite{eldar2020toeplitz} up to $\poly(k,\log (d/\epsilon))$ factors, while running in sublinear time. Moreover, our output $\wt T$ is guaranteed to be low-rank, while the output of \cite{eldar2020toeplitz} is not.



%At its heart, our algorithm solves the following problem.  Consider a function $x(t)$ where $x:\mathbb{Z}\to \mathbb{C}$, and $x$ is $k$-sparse in Fourier domain. Then, assuming noisy sample access to the function at any $t\in [d]=\{0,1,\ldots,d\}$, recover the $k$ potentially ``off-grid'' frequencies in the support of $\wh x(f) $ approximately in $\poly(k)$ time. The continuous time version of this problem, that is the $k$-Fourier sparse function $x(t)$ is from $x:\mathbb{R}\to \mathbb{C}$ and one has noisy sample access to it for any $t\in [0,d]$, was studied and solved in \cite{chen2016fourier}. The discrete time version we consider poses additional challenges when compared to \cite{chen2016fourier} due to the constraint that we can only access the function at integer points in $[0,d]$. The formal statement of this result is presented in section 4 as Lemma \ref{lem:heavy_freq_recovery}.

\subsection{Our approach}\label{sec:approach}
In this section, we sketch the ideas behind the proof of our main result: the sublinear time robust Toeplitz low-rank approximation algorithm of Theorem \ref{thm:sublinear_time_recovery}. Our starting point is the main result of \cite{kapralov2022toeplitz}, which shows that any PSD Toeplitz matrix has a near optimal low-rank approximation $\wt T$ which is itself Toeplitz. Armed with this existence result,  the key idea behind the algorithm of \cite{kapralov2022toeplitz} is to leverage the well-known sparse Fourier structure of low-rank Toeplitz matrices \cite{cybenko1982moment} to recover $\wt T$ using a sample efficient (but computationally inefficient) algorithm. %In particular, they leverage the well-known Vandermonde decomposition theorem, which shows that any Toeplitz matrix can be diagonalized by an {off-grid} Fourier matrix. Formally,
The  idea behind \cite{eldar2020toeplitz} is similar, except that they rely on a weaker existence statement, where the low-rank approximation $\wt T$ is guaranteed to have sparse Fourier structure, but not necessarily be Toeplitz.
Formally, after defining the notion of a Fourier matrix, we state the main result of \cite{kapralov2022toeplitz}.
\begin{definition}[Fourier matrix]\label{def:symmetric_fourier_matrix}
	For any set of frequencies $S=\{f_1,f_2,\ldots, f_s\}\subset [0,1]$, let the Fourier matrix $F_S\in \mathbb{C}^{d\times s}$ have $j^{th}$ column equal to $v(f_j) \eqdef [1, e^{2\pi i f}, e^{2\pi i (2f)}\ldots, e^{2\pi i  (d-1) f}]$.
	%For every $j\in \{1, 2,\ldots, s\}$ the $j$-th column of $F_{S}$ is the frequency vector $v(f_{j})$. 
\end{definition}


\begin{theorem}[Theorem 2 of \cite{kapralov2022toeplitz}]\label{frobeniusexistence}
        For any PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$, $0<\eps,\delta<1$, and $k\leq d$, there exists symmetric Toeplitz $\wt{T}$ with rank $r = \tilde {O}(k \log(1/\delta)/\eps))$ such that
		$$\|T-\wt{T}\|_F \leq (1+\eps)\|T-T_k\|_F + \delta\|T\|_F.$$ %where $T_k = \underset{B:rank(B)\leq k}{\argmin}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm.
		
		Further, $\wt T$ can be written as $\wt T = F_S D F_S^*$ where $F_S \in \mathbb{C}^{d \times r}$ is a Fourier matrix (Def. \ref{def:symmetric_fourier_matrix}) and $D \in \R^{r \times r}$ is diagonal.
\end{theorem}



%
%\begin{theorem}[Vandermonde Decomposition \cite{cybenko1982moment}]\label{thm:vandermonde}
%	Any PSD Toeplitz matrix $T \in \R^{d\times d}$ of rank $r$ can be written as $T = F_SDF_S^{*}$ where $F_S \in \mathbb{C}^{d\times r}$ is a Fourier matrix with frequencies $S=\{f_1,\ldots,f_r\}\subset [0,1]$ and $D\in \mathbb{R}^{r\times r}$ is a diagonal matrix with $r$ positive entries. Moreover for every $j\in [r]$ there is a $j'\in [r]$ such that $e^{2\pi if_j}=e^{-2\pi i f_{j'}}$ and $D_{jj}=D_{j'j'}$.
%\end{theorem}

%that $\tilde T$ guaranteed to exist by Theorem \ref{frobeniusexistence} admits a BLAH. The work of \cite{eldar2020toeplitz} follows a similar approach, except only is able to show that BLAH.


%\Cam{This can be either removed or moved to the prelims if needed.}
%\begin{definition}[Frequency vector]\label{freqvector}
%	For any frequency $f \in [0,1]$, we define the {\em frequency vector} $v(f) \in \mathbb{C}^d$ as the column vector $[1, e^{2\pi i f}, e^{2\pi i (2f)}\ldots, e^{2\pi i  (d-1) f}]^T$.
%\end{definition}

%Equipped with these basic concepts,
%the main result of \cite{kapralov2022toeplitz} is stated below as promised.
%\begin{theorem}[Informal version of Theorem 2 of \cite{kapralov2022toeplitz}]\label{frobeniusexistence}
%        Given any PSD Toeplitz matrix $T\in \mathbb{R}^{d\times d}$, $0<\eps,\delta<1$ and an integer $k\leq d$, there exists a symmetric Toeplitz matrix $\wt{T}=F_{\wt S}\wt D F_{\wt S}^*$ where $\wt S\subset [0,1]$ of size $|\wt S|=\wt{O}((k/\eps)\log(1/\delta))$, $F_{\wt S}$ as per Definition \ref{def:symmetric_fourier_matrix}, and $\wt D\in \mathbb{R}^{|\wt S| \times |\wt S|}$ is a diagonal matrix such that,
%		$$\|T-\wt{T}\|_F \leq (1+\eps)\|T-T_k\|_F + \delta\|T\|_F,$$ where $T_k = \underset{B:rank(B)\leq k}{\argmin}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm.
%\end{theorem}

To prove Theorem \ref{thm:sublinear_time_recovery}, we apply Theorem \ref{frobeniusexistence} to the input PSD Toeplitz matrix $T$ with $\epsilon = \Theta(1)$. Our algorithm is given access to the entries of the noisy matrix $T+E$, which we will write as $\wt T + \wt E$ for $\wt E = E + T-\wt T$. Observe that by triangle inequality, since $\norm{T-\tilde T}_F \lsim \norm{T-T_k}_F + \delta \norm{T}_F$,
$$\norm{\wt E}_F \lsim \norm{E}_F + \norm{T-T_k}_F + \delta \norm{T}_F \lsim \max\{  \norm{E}_F, \norm{T-T_k}_F\} + \delta \norm{T}_F.$$

Thus, to prove Theorem \ref{thm:sublinear_time_recovery} it suffices to show that we can recover $\wt T$ to within a constant factor of the noise level $\norm{\wt E}_F$. Our key contribution is to improve the runtime of this step from being exponential in the rank $r = \tilde O(k \log(1/\delta))$ to being polynomial, and hence sublinear in $d$ (recall that throughout $\tilde O(\cdot)$ hides poly logarithmic factors in $d$ and the argument).

To approximately recover $\wt T$, as in \cite{kapralov2022toeplitz} and \cite{eldar2020toeplitz}, we will leverage its Fourier structure. In particular, 
Theorem \ref{frobeniusexistence} guarantees that $\wt T$ can be written as $\wt T = F_S D F_S^*$, where $F_{S} \in \mathbb{C}^{d \times r}$ is a Fourier matrix (Def. \ref{def:symmetric_fourier_matrix}) and $D \in \R^{r \times r}$ is diagonal. To find $\wt T$, the algorithm of \cite{kapralov2022toeplitz} brute force searches for a good set of frequencies $S$ and corresponding diagonal matrix $D$. In particular, they consider a large pool of candidate frequency sets drawn from an $\epsilon$-net over $[0,1]^r$. For each set $S$, they solve a regression problem to find a diagonal matrix $D$ that (approximately) minimizes $\norm{T-F_S D F_S^*}_F$. These regression problems can be solved using a sublinear number of queries to $T$ using leverage score based random sampling. One can then return the best approximation given by any of the candidate frequency sets as the final output. 

Unfortunately, the above approach incurs exponential runtime, as the number of frequency sets that must be considered grows exponentially in the rank $r = \tilde O(k \log(1/\delta))$. A similar issue plagues the algorithm of \cite{eldar2020toeplitz}, which also performs a brute force search over frequency sets, but with a different regression step, where $D$ is relaxed to be any $r \times r$ matrix.

\medskip 

\noindent{\textbf{Contribution 1: From Column Recovery to Matrix Recovery.}
To avoid this exponential runtime, we will apply tools from the extensive literature on efficient recovery of Fourier-sparse functions \cite{hassanieh2012nearly,indyk2014sample,indyk2014nearly,Boufounos:2015vj,kapralov2016sparse,chen2016fourier,Jin:2023uc}. Observe that if we expand out the decomposition $\wt T = F_S D F_S^*$,  each column of $\wt T$ is an $r$-Fourier sparse function from $[d] \rightarrow \R$. In particular, letting $\wt T_j$ denote the $j^{th}$ column, for any $t \in [d]$, letting $\{a_f\}_f \in S$ be the diagonal entries of $D$,
$$\wt T_j(t) = \sum_{f\in S}a_f e^{2\pi i f(t-j)}.$$ 

Our algorithm will recover a Fourier-sparse approximation to a single column of $\wt T$ using samples of $T + E = \wt T + \wt E$ in just $\poly(r,\log d)$ time using a sparse Fourier transform algorithm. This Fourier-sparse approximation will give us approximations to the frequencies in $F_S$ and the diagonal entries of $D$, which in turn can be used to form an approximation to $\wt T$.

This approach presents several challenges. First, we must ensure that the column that we apply sparse Fourier transform to does not have too much noise on it, compared to its norm. To do so, we sample a random column, which by Markov's inequality, is corrupted with noise whose $\ell_2$ norm is bounded by $\lsim \norm{\wt E}_F/\sqrt{d}$ with good probability. Further, using the fact that $\wt T$ is close to $T$ and hence nearly PSD, we can apply a norm compression inequality of Audenaert \cite{audenaert2006norm} to show that each column of $\wt T$ must have $\ell_2$ norm $\gsim \norm{\wt T}_F/\sqrt{d}$. In combination, these facts ensure that a random column has a similar signal-to-noise ratio as the full matrix $\wt T$ with good probability. Thus, we can expect to recover a good approximation to $\wt T$ from just this column.

Of course, given the noise $\wt E$, we cannot expect to recover approximations to all frequencies in $S$ given sample access to $\wt T + \wt E$. For example, if a frequency $f$ corresponds to a very small entry $a_f$ in $D$, we may not recover it. We must argue that omitting such  frequencies from our approximation of $\wt T$ does not introduce significant error. Again, to do so we will leverage the fact that $\wt T$ is close to PSD and apply a novel `heavy-light' frequency decomposition for PSD Toeplitz matrices.

We detail our approaches to the above challenges further in Section \ref{sec:sublinear_toeplitz_recovery}.

\medskip

\noindent\textbf{Contribution 2: Sublinear Time Discrete-Time Off-Grid Sparse Fourier Transform.}
After showing that applying a sparse Fourier transform to a random column of $\wt T$ suffices to recover a good approximation to the full matrix, it remains to show that we can implement such a sparse Fourier transform efficiently.

%We can thus hope to recover the first column $\wt T_1$, and in turn $\wt T$ using noise-robust sparse Fourier recovery techniques. % on $\wt T_1(t)$, and then fit $\wt D$ using fast regression primitives. This approach was adopted by \cite{kapralov2022toeplitz} however their sparse Fourier recovery algorithm recovered the frequencies using a brute force search running in $\exp(k)$ time, which resulted in an inefficient running time overall.

If the frequencies in $S$ were integer multiples of $1/d$, i.e., they were ``on-grid'', %then the function $\wt T_j(t)$ would be a periodic function with period $d$, and thus completely determined by its values at the integer points $t\in [d]$. 
then we could apply a discrete sparse Fourier transform algorithm to  recover a Fourier-sparse approximation to a random column $\wt T_j$ of $\wt T$ given samples from the column $[T+E]_j = [\wt T + \wt E]_j$. Such algorithms  have been studied extensively in recent years \cite{hassanieh2012nearly,Hassanieh:2012tq,Gilbert:2014tp}. However, the main difficulty in our case is that the frequencies in $S$ may be ``off-grid'', i.e., arbitrary real numbers in $[0,1]$. % in general and thus $\wt T_1(t)$ may have a period $>>d$ making the problem hard. 
Recent work of \cite{chen2016fourier} solves the off-grid sparse Fourier transform problem given sample access to the function $[\wt T +\wt E]_j$ on the \emph{continuous range $[0,d]$}. However, in our setting, we can only access $[\wt T + \wt E]_j$ at the integer points $\{0,1,\ldots,d-1\}$ -- i.e., at the entries in the $j^{th}$ column of our matrix. We must substantially modify the approach of  \cite{chen2016fourier} to show that, nevertheless, we can well approximate $\wt T_j$ from samples  at these points. In doing so, we give to the best of our knowledge, the first efficient \emph{discrete time off-grid} sparse Fourier transform algorithm, which may be applicable in other settings that involve off-grid frequencies but on grid time samples.

We detail our discrete time off-grid sparse Fourier transform algorithm in Section \ref{section:dtft_recovery_techintro}.

%$Since the frequencies in $S$ lie in $[0,1]$, by the Shannon-Nyquist theorem, the function $T_j$ is completely determined by its values at the integers. 

%The work of \cite{chen2016fourier} solved this problem in more generality when $\wt S \subseteq [-F,F]$ for any bandlimit $F$, given access to the input at all $t\in [0,d]$. This won't work in our setting as is, since we only have access to the input at \emph{integer} $t\in [d]=[0,d]\cap \mathbb{Z}$. It is important to note that since all frequencies in $\wt S$ are in $[0,1]$, by the Shannon-Nyquist theorem $\wt T_1(t)$ is completely determined by its values at all $t\in \mathbb{Z}$. Moreover if one settles for recovering frequencies in $\wt S$ \emph{approximately},  then we can hope to use tools from \cite{chen2016fourier} to deal with the fact that we can only access the input on a bounded interval $[0,d]\cap \mathbb{Z}$ and not the entire $\mathbb{Z}$. It is not trivial how to make the framework of \cite{chen2016fourier} work in this case, and that is our first contribution discussed below.


\section{Technical Overview}\label{sec:overview}

We next describe our main contributions in more detail. We first detail our efficient discrete time off-grid sparse Fourier transform in Section \ref{section:dtft_recovery_techintro}. In Section \ref{sec:sublinear_toeplitz_recovery} we describe how this primitive is used to prove Theorem \ref{thm:sublinear_time_recovery}, by showing how to recover a low-rank Toeplitz approximation $\wt T$ to the input matrix $T$ by applying our sparse Fourier transform to a random  column of the input matrix.

%\Cam{UP TO HERE.}

%\Cam{This was out of place. Move elsewhere. For any function $f:\mathbb{Z}\rightarrow \mathbb{C}$, let $\|f\|_d^2 := \sum_{t\in [d]}|f(t)|^2$. }

\subsection{Discrete Time Off-Grid Sparse Fourier Recovery}\label{section:dtft_recovery_techintro}
A discussed, a key primitive used in our robust Toeplitz low-rank approximation algorithm is an efficient  discrete time off-grid sparse Fourier transform. Informally,  such an algorithm must solve the following sparse Fourier recovery problem:

\Cam{Is the indexing off here? Should $t$ range from $0$ to $d-1$ ? Also here you define $x^*$ only over $[d]$, but later you use it as a function over all of $\mathbb{Z}$ right? (KS-yes, ok so redefined $x^*$ to be over all $\mathbb{Z}$ and then say have access over $[d]$)}

\Cam{I had to change the notation here to have at set of frequencies $S$ rather than indexing the frequencies as $f_j$. Since there were multiple places later where indexing didn't work. E.g. we refs $f \in S(L)$ and then wrote its coefficient as $a_j$ which didn't make sense. Make sure the notation is properly propogated.}
\begin{problem}\label{def:problem_definition}(Off-Grid Sparse DTFT -- Informal)
Let $x^*(t) = \sum_{f \in S} a_f \cdot e^{2\pi i f t}$ for $t\in \mathbb{Z}$ and $S \subset [0,1]$ with $|S| = k$. Let $x(t) = x^*(t)+g(t)$, where $g$ is arbitrary noise. Given sample access to $x(t)$ for any $t\in [d]$, approximately recover all $f \in S$ that contribute significantly to $x$. % in $\poly(k, \log d)$ time. %Remark: Note that since we only have time domain access at points $t\in [d]$, this is a harder problem than the one studied in \cite{chen2016fourier}\kstodo{add footnote formalizing the connection}.
\end{problem}
We will be working with the discrete time Fourier transform (DTFT), which for any function $x:\mathbb{Z}\to \mathbb{C}$ is denoted by $\wh{x^*}:[0,1]\to \mathbb{C}$ and formally defined in Definition \ref{def:dtft}. The work of \cite{chen2016fourier} solves the above problem in the more general case when $S \subset [-F,F]$ for some bandlimit $F$. However, their algorithm critically requires sample access to $x(t)$ for any real  $t\in [0,d]$. Prony's method \cite{Prony:1795wv} can exactly recover all frequencies $f \in S$ and coefficients $a_f$ using any $2k$ time domain samples, including at integers in $[d]$ -- but only in the noiseless setting when $g(t) = 0$.
Observe that in the presence of noise it generally will not be possible to identify all frequencies in $S$ given sample access to $x(t)$ only on $[d]$. For example, if two frequencies $f$ and $f'$ are extremely close to each other, their contributions to the function $x$ could nearly cancel out, making it impossible to identify them in the presence of noise. This is true even if the coefficients $a_{f}$ and $a_{f'}$ are arbitrarily large.

\Cam{But *why* do we even need to filter the time domain to $[d]$? That does not solve the problem of having frequencies that are too close to distinguish right?} 

Furthermore we cannot simply truncate the signal to $[d]$, say by multiplying it with the indicator function of the interval $[d]$, as this hard thresholding operation will spread out the frequencies of $x^*$ a lot. \Cam{What does it mean to `spread out' a frequency and why is it bad to do?} To mitigate this we can use a discrete variant of a \emph{filter function} designed by \cite{chen2016fourier}. This discrete filter function  $H:\mathbb{Z}\rightarrow
\mathbb{R}$ satisfies the following for some given $\delta > 0$ and for any $k$-sparse $x^*(t):\mathbb{Z}\rightarrow \mathbb{C}$,
\begin{align}\label{eqn:H_properties_summary}
		 \sum_{t \in \mathbb{Z}\setminus [d]} |x^*(t) \cdot H(t) |^2 &\leq \delta \|x^*\|_d^2\nonumber\\
		 0.99\|x^*\|_d^2\leq \sum_{t \in [d]} |x^*(t) \cdot H(t) |^2 &\leq \|x^*\|_d^2,
\end{align}
where for any function $f:\mathbb{Z}\rightarrow \mathbb{C}$, we define $\|f\|_d^2 \eqdef \sum_{t\in [d]}|f(t)|^2$. \Cam{Its more like they design a function satisfying a continuous variant of this and we show that it also satisfies the discrete variant right? (KS-yes, fixed)}

Intuitively, $H$ approximates the indicator function of the interval $[d]$ by almost killing off the energy of $x^*(t)$ outside of $[d]$ and preserving the energy inside $[d]$. \Cam{Both $supp$ and the Fourier transform notation are undefined. (KS-fixed)} At the same time, $H$ is designed to be compact in the Fourier domain: $|supp(\wh{H})|\leq \poly(k,\log(d/\delta)/d$, where $supp(f)$ denotes the support of any complex valued function $f$ defined as $supp(f)=\{x\in \text{domain($f$)}:|f(x)|>0\}$. The formal definition and properties of $H$ are in Lemma \ref{lem:H_discrete_properties}. \Cam{Is it a direct import? (KS-not a direct import, fixed)} We now discuss that these properties of $H$ ensure that working with $x\cdot H$ instead of $x$ is sufficient for approximate frequency recovery.\Cam{'Thus' implies that this follows from what you stated above. but it doesn't. You haven't said anything about why $H$ having small support is useful. (KS-ok tried to fix)}

The discrete time Fourier transform of $x^*\cdot H$ is equal to $\wh{x^*\cdot H}=\widehat{x^*}\ast \widehat{H}$ where $\ast$ is the convolution operator. Since $|supp(\wh{H})|\leq \poly(k,\log(d/\delta))/d$,  all of the mass of $\widehat{x^*}\ast \widehat{H}$ is within $\poly(k,\log(d/\delta))/d$ of all the frequencies in $supp(\widehat{x^*})$. \Cam{What does this mean? How can a frequency not be corrupted by noise? The noise is added in the time domain and will effect all frequencies (KS-tried to fix)} Thus we can aim for locating frequencies of $supp(\wh{x^*})$ approximately with an additive error of roughly $\poly(k,\log(d/\delta))/d$. Moreover we can aim for recovering a list of frequencies such that the total mass of frequencies of $\wh{x^*}$ that do not contain any frequency within $\poly(k,\log(d/\delta))/d$ of them in the list is small. We can indeed achieve this in $\poly(k,\log(d/\delta))$ time as shown below. \Cam{Sounds like we *can* achieve this but *why do we want to* achieve this? Why is it good enough to get the frequencies to error $\frac{\poly(k,\log(d,\delta)}{d}$?} See Section \ref{sec:dtft_recovery} for a more formal statement.


\begin{lemma}[Approximate Frequency Recovery -- Informal] \label{lem:dtft_freqrecovery} Consider the setting of Problem \ref{def:problem_definition}. Assume that $\|g\|_d^2 \leq c\|x^*\|_d^2$ for a small absolute constant $c$. Then for any given $\delta>0$, there exists an algorithm that in time and sample complexity $\poly(k,\log(d/\delta))$ outputs a list $L$ of $\poly(k)$ \Cam{This is just $\poly(k)$ with no logs (KS-yes)?} frequencies in $[0,1]$ such that, with probability at least $0.99$, letting $$S(L)=\left \{f\in S: \exists f'\in L \text{ s.t. } |f-f'|_{\circ}\leq \frac{\poly(k,\log(d/\delta)}{d}\right \},$$ and letting $x^*_{S(L)} \eqdef \sum_{f\in S(L)}a_f e^{2\pi i f t}$, we have $$\|x^*-x^*_{S(L)}\|_d^2 \lsim \|g\|_d^2 +\delta \|x^*\|_d^2.$$ Here $|\cdot|_{\circ}$ is the wrap-around distance defined as $|f_1-f_2|_{\circ}=\min\{|f_1-f_2|,|1-(f_1-f_2)|\}$ for any $f_1,f_2\in [0,1]$. \Cam{You have to define it here. In paper is is never ok to forward ref to a definition or theorem.}
\end{lemma}
Lemma \ref{lem:dtft_freqrecovery} mirrors Lemma 7.23 in \cite{chen2016fourier}, but only requires accessing $x(t)$ at the integer $t \in [d]$ rather than at real $t\in [0,d]$. We now discuss how we modify the approach of \cite{chen2016fourier} to work in this more restricted sampling setting.

\medskip

\noindent \textbf{Single Cluster Case.} As in \cite{chen2016fourier}, we first consider the \emph{single cluster} case, when most of the energy of $z = x\cdot H$ in Fourier domain is concentrated around a single frequency $f_0\in [0,1]$. Formally, we define the single cluster case as follows:
\begin{definition}[$(\epsilon,\Delta)$-one clustered signal]\label{def:one_clustered_signal}
	$z:\mathbb{Z}\to \mathbb{C}$ is $(\epsilon,\Delta)$-one clustered around $f_0 \in [0,1]$ if 
	\begin{align*}
		\textnormal{ Property I: } & \quad \int_{f_0 - \Delta}^{f_0 + \Delta} |\wh{z}(f)|^2 df \geq  (1 - \eps) \int_{0}^{1} |\wh{z}(f)|^2  df \\
		\textnormal{Property II: } & \quad \|z\|_d^2 \geq  (1 - \eps) \sum_{t \in \Z} |z(t)|^2. 
	\end{align*}
\end{definition}
In this setting, \cite{chen2016fourier} shows how to recover $f'$ with $|f'-f_0|_{\circ}\leq \frac{\poly(k,\log(d/\delta))}{d}$ in $\poly(k,\log(d/\delta))$ time when $\epsilon$ is a small enough constant and $\Delta=\poly(k,\log(d/\delta))/d$. Later, they use hashing and filtering techniques to reduce the general case to this clustered case for this setting of $\epsilon,\Delta$.
%Observe that Property II is ensured if $z = x \cdot H$ for our filter function $H$ by \eqref{eqn:H_properties_summary}. 
\Cam{I added the prior sentence. Is is true? Also why are we using $\epsilon$ rather than $\delta$ here? And how can our gurantees for both accuracy and runtime not depend on $\epsilon$?}

To find  $f'$ with $|f'-f_0|\lsim \frac{\poly(k,\log(d/\delta))}{d}$, \cite{chen2016fourier} show that given any sufficiently small $\beta$,  they can output an $\alpha$ such that $ z(\alpha+\beta)/z(\alpha)$ approximates $e^{2\pi i f_0 \beta}$ with large constant probability. It is not hard to modify this subroutine to output an integer $\alpha\in [d]$ for an integer $\beta$, so that both $z(\alpha+\beta)$ and $z(\alpha)$ can be queried in our more restricted query setting. \Cam{This needs to be explained more. E.g. explain that if the signal was exactly just the single frequency $e^{2\pi i f_0 t}$ then we would exactly have  $ z(\alpha+\beta)/z(\alpha) = e^{2\pi i f_0 \beta}$. Also you need to explain *why* we care about approximating this. Presumably because we can then back out $f_0$.} We present this modification in Section \ref{subsubsec:sampling_the_signal}. 

The above primitive is used by the algorithm of \cite{chen2016fourier} within a $t$-ary search for $t\approx \log d$  \Cam{not sure what this means? Why are we doing $\log d$-ary search instead of binary search. its very myterious to the reader. ALso the above primitive gives a way of approximating $f_0$. How is it used in this t-ary search? Also we should not use $t$ a variable here since we are already using it to refer to time domain samples. Maybe use $b$?} to iteratively refine an approximation to $f_0$ until achieving the desired accuracy of $\frac{\poly(k,\log(d/\delta)}{d}$. The key component in this $t$-ary search is to choose $\beta$ randomly such that for $f$ that are far from $f_0$, $2\pi \beta |f-f_0|_{\circ}$ is almost uniformly distributed on the circle. That is,
\begin{equation}\label{eqn:low_prob_far_candidates}
\Pr[2\pi \beta |f-f_0|_{\circ} \mod 2\pi \in [-3s\pi/2,3s\pi/2]]\leq 10s.    
\end{equation}
for some small constant $s$. \Cam{Is it for some small constant? Or for any small enough s? I also don't see how this property has anything to do with being uniformly distributed on the circle. It just says that the random variable in unlikely to fall in a range near $0$. Which doesn't relate to the property of being unifomrly distributed} This property is used to ensure that all $f$ that are sufficiently far away from $f_0$ get  discarded in each iteration of the $t$-ary search, and we make progress. \Cam{It is completely unclear why this propoerty allows us to discard $f$. This neesd more explaination. I assume that $f'$ which is close enough to $f_0$ will generally have $2\pi \beta |f-f_0|$ close to $0$. But this can't be determined as we haven't talked about roughly how large $\beta$ is.} \cite{chen2016fourier} show that if $\beta$ is chosen to be a uniformly random \emph{real} number in a carefully chosen range, then \eqref{eqn:low_prob_far_candidates} is satisfied for all $f$ not too close to $f_0$ \Cam{What does not too close mean? The reader needs some intuition for what is going on.}. Thus, these frequencies are discarded in the search and the search space is reduced by a factor $t$. \Cam{Why is it reduced by a factor $t$? Why not by a factor $2$, or $100$?}

In our setting, we need $\beta$ to be an integer, so that we can query the function values $z(\alpha+\beta)$ and $z(\alpha)$. However, letting $\beta$  be a uniformly random {integer} in the same range will not suffice to guarantee that equation \eqref{eqn:low_prob_far_candidates} holds. For example, if $|f-f_0|_{\circ}=1/2$ then $2\pi \beta |f-f_0|_{\circ} = \pi \beta = 0 \mod 2\pi $ for every even $\beta$. 

Keeping the above issue in mind, we now discuss a related issue that arises in the algorithm of \cite{chen2016fourier} when using the single cluster recovery primitive to solve the general sparse recovery problem. We will see that both issues can be resolved with the same modification, discussed below.

 \Cam{I think the discussion above is too vague. It is basically impossible to follow. E.g. you reference a 'carefully chosen range'. What roughly  is this range? And you write out a complex condition (4) but then it is  unclear how this condition relates to the task at hand. It is very non intuitive that somehow having some weird notion of distance be uniformly distributed would allow a frequency to be `thrown out'. Do nearby frequencies  have this distance not uniformly distributed and thus we can identify them? I feel that i understood this primitive when we discussed in person but cna't understand it at all from this paragraph. If you want to keep things simple maybe you can just explain what happens in either the first or the last iteration of the $b$-ary search?}

%\textbf{alternative:} \cite{chen2016fourier} show that in iteration $i$, if $\beta$ is sampled uniformly from roughly $[0.5(\log(d))^i, (\log(d))^i)]$ then equation \ref{eqn:low_prob_far_candidates} is satisfied for all $f$ such that $|f-f_0|\gsim 1/(0.25\log(d))^i$. We need $\beta$ to be an integer as we will be querying $z(\alpha+\beta)$ for some integer $\alpha$. Sampling $\beta$ to be uniformly random \emph{integer} in the same range $[0.5(\log(d))^i, (\log(d))^i)]$ cannot guarantee equation \ref{eqn:low_prob_far_candidates} as is because for eg. if $|f-f_0|=1/2$ then $2\pi \beta |f-f_0| = \pi \beta = 0 \mod 2\pi $ for every even $\beta$. Keeping this issue in mind we now state the next issue when adapting \cite{chen2016fourier} to the discrete time setting.

\medskip

\noindent \textbf{Multi-Cluster Case.} 
The complete algorithm of \cite{chen2016fourier} reduces a general instance of Problem \ref{def:problem_definition} to several one-cluster  instances (Def. \ref{def:one_clustered_signal}). They achieve this reduction using hashing techniques. Let  $\sigma\in \mathbb{R},b\in [0,1]$ and $B$ be the number of hash buckets, and consider the following hash function $h_{\sigma,b}:[0,1]\rightarrow \{0,\ldots,B-1\}$,
\begin{align}
    \pi_{\sigma,b}(f) &= 2\pi \sigma (f-b) \mod 2\pi \nonumber\\
    h_{\sigma,b}(f) &= \text{round}(\frac{B}{2\pi}\pi_{\sigma,b}(f))\label{eqn:hash_fn},
\end{align}
\Cam{IF you have a numbered equation with two lines, and you don't have a lable for both lines, then you should use nonumber to remove the number on one of the lines. There is no need to have two number when you can only reference one of them.}\Cam{This should be stated when $B$ is first used. Actualyl before it is first used.} and the round$(.)$ function rounds real numbers to the nearest integer. The crucial claim that \cite{chen2016fourier} show is that if we let $\sigma$ be a uniformly random real number in an appropriate range \Cam{Again, roughly what range and roughly how close?}, then we have that for any $f_1,f_2$ not too close,
\begin{equation}\label{eqn:low_collision_prob}
    \Pr [h_{\sigma,b}(f_1)=h_{\sigma,b}(f_2)]=\Pr [2\pi \sigma (f_1-f_2)\mod 2\pi \in [-2\pi/B,2\pi/B]]\lsim 1/B,
\end{equation}
implying $h_{\sigma,b}(f_1)=h_{\sigma,b}(f_2)$, i.e. $f_1,f_2$ collide and land in the same bucket, with low probability. \Cam{What does this mean that they collide? That $h_{\sigma,b}(f_1) = h_{\sigma,b}(f_2)$? How is that equvilant to the above event?} Furthermore, \cite{chen2016fourier} also design a filter function $G^{(j)}_{\sigma,b}$ for every $j\in [B]$ which when convolved with essentially gives access to the function only containing frequencies that hashed to bin $j$. \Cam{Need to explain that this results in a one cluster signal if that is the case.} Then \cite{chen2016fourier} use equation \eqref{eqn:low_collision_prob} to show that for any frequency $f$\Cam{I don't think there is a condition stated in this Lemma?}, the bound \eqref{eqn:low_collision_prob} with a union bound over all frequencies in $supp(\wh{x^*})$ implies that no other frequency in $supp(\wh{x^*})$ collides with $f$.\Cam{A union bound over what?} These facts can then be used to argue that bins containing isolated heavy frequencies with low SNR are essentially one-clustered, thus allowing us to recover the isolated frequency approximately. \cite{chen2016fourier} design an algorithm \hyperref[alg:hashtobins]{\textsc{HashToBins}} \kstodo{Do we discuss differences in new analysis compared to CKPS?}to compute the value of the signal containing frequencies only from a single hash bucket at any desired time instant as required by the one-cluster recovery algorithm. However to use this algorithm in our context, $\sigma$ must be an \emph{integer}. The details of \hyperref[alg:hashtobins]{\textsc{HashToBins}} are formally presented in Lemma \ref{lem:hashtobins} \Cam{What is formally presented? The fact that it must be an integer?}. However, if we choose $\sigma$ to be a uniformly random integer in the same range needed by equation \eqref{eqn:low_collision_prob}, we face the same issue as in the one-cluster case. More specifically consider any $f_1,f_2$ such that $|f_1-f_2|_{\circ} = 1/2$, then for any even integer $\sigma$, $2\pi \sigma |f_1-f_2| = \pi \sigma = 0 \mod 2\pi$. Thus we cannot hope to prove equation \eqref{eqn:low_collision_prob} with any probability smaller than $1/2$.

\medskip
\noindent \textbf{Recovery for Bounded Instances.}
The source of the issues in the one-cluster and the multi-cluster case is identical up to different parameter settings. We now describe our fix. We call an input \emph{bounded} (see Definition \ref{def:bounded_freq_case} for the formal definition) if essentially $supp(\wh{x^*})$ is contained in an interval of size $1/B$ and the energy of the noise outside this interval is bounded. Consider any $f_1,f_2$ such that $F:=|f_1-f_2|_{\circ}\leq 1/B$. Then if we consider $\sigma$ to be a random \emph{integer} number in the same range as needed by equation \eqref{eqn:low_collision_prob}, $2\pi \sigma |f_1-f_2|_{\circ}=2\pi \sigma F$ is distributed on a grid with uniform spacing, with the spacing at most $2\pi/B$. Thus we can hope that for every value of $\sigma$ such that $2\pi \sigma F \mod 2\pi \in [-2\pi/B,2\pi/B]$, there are $\gsim B$ values of $\sigma$ for which $2\pi \sigma F \mod 2\pi \notin [-2\pi/B,2\pi/B]$, since the grid on which $2\pi \sigma F$ lies is fine enough. We are able to formally show that this is enough to ensure equation \eqref{eqn:low_collision_prob} holds for frequencies in a bounded instance. This claim when applied more generally also fixes the issue appearing in the one-cluster case when proving equation \eqref{eqn:low_prob_far_candidates}.


The final part is to actually reduce a general instance to a bounded instance. To do this, we first state an observation. Consider the hash function as per equation \eqref{eqn:hash_fn} for $\sigma =1$ and any $b\in [0,1]$. Then one can observe that the hash buckets are simply the intervals $$[b-1/2B,b+1/2B],[b+1/2B,b+3/2B],\ldots,[b-3/2B,b-1/2B]$$ where each interval is modulo 1. Essentially the hash function $h_{1,b}$ chops up $[0,1]$ into $B$ intervals of length $1/B$. Thus $G^{(j)}_{1,b}$ is (almost) the indicator function of the $j^{th}$ interval/bucket, and convolving the input with it gives access to the input only containing frequencies in the $j^{th}$ interval/bucket, which will thus be \emph{bounded}. Since $\sigma=1$ we can compute the convolution of the input with $G^{(j)}_{1,b}$ by simply running \hyperref[alg:hashtobins]{\textsc{HashToBins}}.  Overall with this additional layer of hashing on top, we can reduce a general instance into $B$ bounded instances. The proofs are in general have complicated details, which we defer to section \ref{subsubsection:multi_cluster_reduce}, and we also present the proof of Lemma \ref{lem:dtft_freqrecovery} in section \ref{subsubsection:multi_cluster_reduce}. Then for each of the $B$ bounded instances we apply the again apply the hashing based reduction to reduce a multi cluster bounded instance to a one cluster instance as discussed before in section \ref{subsubsection:multi_cluster_bounded_freqs}, and state the main claim and algorithm of recovering frequencies from a bounded instance in \ref{subsection:recovering_all_freqs_by_boosting}. Finally, we present the algorithm to find the central frequency of a one-cluster instance obtained from a bounded instance in section \ref{subsection:one_cluster}.\
\subsection{Sublinear Time Algorithms for Toeplitz Matrices}\label{sec:sublinear_toeplitz_recovery}
%\Cam{This section needs to be organized. Theorems 1-3 should already be stated and discussed in the intro. So you should not have an intro to this section stating them again without proof. You can maybe move some of this content to the intro. The section should simply first prove Theorem 1 via the heavy light decomposition. And then have a subsection which proves Theorem 2 as an immediate consequence and Theorem 3 as well.}
Equipped with our sublinear time off-grid sparse recovery scheme of Lemma \ref{lem:dtft_freqrecovery} and the existence result of Theorem \ref{frobeniusexistence}, we now describe the proof of our main result on sublinear time Toeplitz low-rank approximation, Theorem \ref{thm:sublinear_time_recovery}. 

%\Cam{I updates some wording in the theorem statement. Please update in intro as well. I also removed the variable $r = |S|$ as it was no neccesary in the statement. So if you use it later make sure to define it-Done}
%\begin{reptheorem}{thm:sublinear_time_recovery}
	%Let $T\in \mathbb{R}^{d\times d}$ be a PSD Toeplitz matrix, $E\in \mathbb{R}^{d\times d}$ be arbitrary noise, $\delta>0$ be an error parameter, and $k$ be a positive integer rank parameter. Given query access to the entries of $T+E$, in time $\poly(k,\log(1/\delta))$ we can find $S'\subset  [0,1]$ of size $|S'|=\poly(k,\log(1/\delta))$ and diagonal $D'\in \mathbb{R}^{|S'|\times |S'|}$  such that the symmetric Toeplitz matrix $T' = F_{S'}D' F_{S'}^*$ \Cam{$F_{S'}$ is not defined here.} satisfies, with probability at least $0.9$,
	%\begin{equation*}
	%	\|T- T'\|_F \lsim \max\{\|E\|_F,\|T-T_k\|_F\} + \delta \|T\|_F.
	%\end{equation*}
	%where $T_k = \argmin_{B: rk(B)\leq k}\|T-B\|_F$ is the best rank-$k$ approximation to $T$ in the Frobenius norm.
%\end{reptheorem}

\medskip

\noindent
\textbf{Heavy-Light decomposition.} To prove Theorem \ref{thm:sublinear_time_recovery}, we consider $\wt T=F_{ S} D F_{ S}^*$ as guaranteed to exist by Theorem \ref{frobeniusexistence} applied with small constant $\epsilon$. Expanding out this decomposition, we see that every column of $\wt T$ is a $\wt O(k)$-Fourier sparse function, whose support in Fourier domain is exactly the frequencies $ S$ in the Vandermonde decomposition of $\wt T$. Thus we can hope to apply Lemma \ref{lem:dtft_freqrecovery} to some column to approximately recover frequencies in the Vandermonde decomposition of $\wt T$. After this step, we can then hope to regress onto these heavy frequencies as returned by Lemma \ref{lem:dtft_freqrecovery} and recover a good approximation to $\wt T$ in the Frobenius norm. 

There are several challenges that we must overcome to implement this plan. Recalling that we denote the noise on $\wt T$ as $\wt E = E + T-\wt T$, we can only assume that $\|\wt E\|_F$ is small compared to $\|\wt T\|_F$ (in the other case noise is high so outputting all zeros matrix works). \Cam{What other case? What do you mean you can 'only assume'? Do you mean we can assume this since otherwise even outputting a trivial approximation like the all zeros matrix works?} However the noise may very well concentrate on the first column of $\wt T$. More formally, we can assume $\|\wt E\|_F\leq c\|\wt T\|_F$ for a small enough constant $c>0$. However it could be that \Cam{Here you have switched notation. Instead of using $\wt E_1$ to denote the first column you are using $\wt E_{[0:d,0]}$.} $\|\wt E_{[0:d,0]}\|_2 \gg c\|\wt T_{[0:d,0]}\|_2$\footnote{For any matrix $A$ we denote $A_{[i:j,k]}$ to be the $i$ to $j^{th}$ entries of the $k^{th}$ column of $A$ for $i,j,k$ within dimension bounds of $A$.}. \Cam{The lemma doesn't state this as being a requirement though?} We can instead consider picking a random column $i\sim [d]$, and can argue by Markov's inequality that $\|\wt E_{[0:d,i]}\|_2 \leq 10 \|\wt E\|_F/\sqrt{d}\leq 10 c\|\wt T\|_F/\sqrt{d}$, with probability $0.9$. However if the $\ell_2$ norm $\|\wt T_{[0;d,i]}\|_2$ is extremely small compared to $\|\wt T\|_F/\sqrt{d}$ then we still cannot conclude that $\|\wt E_{[0:d,i]}\|_2\lsim c \|\wt T_{[0:d,i]}\|_2$. This can happen for example when the bottom left entry $\wt T_{[d,0]}$ is extremely large and the rest of the entries of $\wt T$ are very small and thus $\|\wt T_{[0:d,i]}\|_2$ is extremely small compared to $\|\wt T\|_F$ for all $i$ except $i=0,d$. However we show that this cannot happen when 
$\wt T$ is (almost) PSD and Toeplitz, which is guaranteed for us from Theorem \ref{frobeniusexistence}. Formally we show the following lemma.
\begin{lemma}\label{lem:smallnoisefirstcol}
	Let $\wt T$ be a $d\times d$ symmetric Toeplitz matrix, and suppose that there exists a PSD Toeplitz matrix $T$ satisfying $\|\wt T- T\|_F \leq 0.001 \|T\|_F$. 
    Then the following holds,
	\begin{equation*}
		\|\wt T_{[0:d/2,0]}\|_2\geq \frac{0.49}{\sqrt{d}} \|\wt T\|_F.
	\end{equation*}
\end{lemma}
The proof of this lemma relies on a norm compression inequality of Audenaert \cite{audenaert2006norm}. The previous lemma says that if $\wt T$ has large Frobenius norm, then any $i^{th}$ column for $i\in [d/2]$ has large $\ell_2$ norm as well, because any such $i^{th}$ column has its $d/2$ entries $\wt T_{[i:i+d/2,i]}=\wt T_{[0:d/2,0]}$ (since $\wt T$ is Toeplitz) so its norm $\|\wt T_{0:d,i}\|_2$ is at least $\|\wt T_{[i:i+d/2,i]}\|_2=\|\wt T_{[0:d/2,0]}\|_2\gsim \|\wt T\|_F/\sqrt{d}$.
%  %Morever $\wt T_i$'s Fourier transform is identical to $\wt T_1$ upto a time shift, thus we can still hope to run Lemma \ref{lem:dtft_freqrecovery} on it.

We now describe the second issue, which is that even if we could run Lemma \ref{lem:dtft_freqrecovery} on $\wt T_{[0:d,i]}$, this lemma only guarantees that the $\ell_2$ norm of the signal corresponding to the unrecovered frequencies in the Fourier spectrum of $\wt T_{[0:d,i]}$ is small. Defining $\wt T^{light}$ be the Toeplitz matrix whose Vandermonde decomposition contains these uncrecovered frequencies, the previous discussion implies that the $\ell_2$ norm of the $i^{th}$ column of the matrix $\wt T^{light}$ is small. However, to recover a good approximation to the whole matrix $\wt T$, we need to ensure that the Frobenius norm of $\wt T^{light}$ is small. We are able to show that $\wt T^{light}$ is also almost PSD using the properties of $\wt T$ as per Theorem \ref{frobeniusexistence} \cite{kapralov2022toeplitz}. Thus invoking Lemma \ref{lem:smallnoisefirstcol} we can argue that $\|\wt T^{light}\|_F\lsim \sqrt{d}\|\wt T^{light}_{[0:d/2,0]}\|_2\leq \sqrt{d}\|\wt T^{light}_{[0:d,i]}\|_2$ for any $i\in [d/2]$, where the last inequality follows from the fact that $\wt T^{light}$ is symmetric Toeplitz thus $\|\wt T^{light}_{[0:d/2,0]}\|_2=\|\wt T^{light}_{[i:i+d/2,i]}\|_2\leq \|\wt T^{light}_{[0:d,i]}\|_2$.

\begin{comment}
This suggests the following strategy. We sample a random column $i\sim [d/2]$. We want to apply Lemma \ref{lem:dtft_freqrecovery} to $\wt T_{[0:d,i]}$. A small caveat is that this column is identical to $\wt T_{[0:d,0]}$ upto a time-shift, and thus their Fourier spectrum is different. To simplify this we only work with the $d/2$ sized chunk $\wt T_{[i:i+d/2,i]}$ of the $i^{th}$ column, which by the virtue of $\wt T$ being Toeplitz is equal to $\wt T_{[0:d/2,0]}$. Using Markov's inequality we can show that the noise on this chunk of the $i^{th}$ column is small, i.e., $\|\wt E_{[i:i+d/2,i]}\|_2 \lsim \|\wt E\|_F/\sqrt{d}\leq c\|\wt T\|_F/\sqrt{d}$. \Cam{Havne't we already made this argument earlier in the sectin? We argued that the noise on the whole column norm is small.} Moreover from Lemma \ref{lem:smallnoisefirstcol} $\|\wt T_{[i:i+d/2,i]}\|_2=\|\wt T_{[0:d/2,0]}\|_2\gsim \|\wt T\|_F/\sqrt{d}$. Thus we get that $\|\wt E_{[i:i+d/2,i]}\|_2 \lsim c\|\wt T_{[i:i+d/2,i]}\|_2$ with probability at least $0.9$, enabling us to apply Lemma \ref{lem:dtft_freqrecovery} to this length $d/2$ signal. Let $\wt T^{light}$ be the Toeplitz matrix corresponding to unrecoverable light frequencies in the spectrum of $\wt T_{[i:i+d/2,i]}=\wt T_{[0:d/2,0]}$, i.e., those not satisfying the condition of Lemma \ref{lem:dtft_freqrecovery} for noise $\wt E_{[i:i+d/2,i]}$. We can then bound the $\ell_2$ norm of the length $d/2$ signal $\wt T^{light}_{[i:i+d/2,i]}=\wt T^{light}_{[0:d/2,0]}$ using the properties of the $H$ function as per equations \ref{eqn:H_properties_summary} and also show using the existence result of Theorem \ref{frobeniusexistence} that $\wt T^{light}$ is almost PSD (in the sense of Lemma \ref{lem:smallnoisefirstcol}). Combining these with Lemma \ref{lem:smallnoisefirstcol} we can show that $\wt T^{light}$ thus has small Frobenius mass. 
\end{comment}
This gives us a ``heavy-light'' decomposition of $\wt T=\wt T^{heavy}+\wt T^{light}$ where the Fourier sparse spectrum of $\wt T^{heavy}$ is approximately recoverable and $\wt T^{light}$ has low Frobenius mass. This is formalized below.
\begin{lemma}\label{lem:heavy_freq_recovery}
Consider the input setup of Theorem \ref{thm:sublinear_time_recovery}. Let $\wt T = F_{ S} D F_{S}^*$ be as guaranteed to exist by Theorem \ref{frobeniusexistence} for $T$, $\epsilon=0.1$, $\delta$ and $k$. Let $\wt E= E+T-\wt T$. Assume $\|\wt E\|_F \leq c\|\wt T\|_F$ for some small enough constant $c$. Then in $\poly(k,\log(d/\delta))$ time we can find a list of frequencies $L \subseteq [0,1]$ of size $|L| = \poly(k,\log (d/\delta))$ satisfying, with probability 0.9 - Let $S_{heavy}\subseteq S$ defined as follows, $$S_{heavy}= \{f\in S: \exists f'\in L \text{ s.t. } |f-f'|_{\circ}\leq \poly(k,\log(d/\delta))/d \}.$$ Let $D^{heavy}$ containing the entries of $D$ corresponding to $S_{heavy}$, and $\wt T^{heavy} = F_{S^{heavy}} D^{heavy}F_{S^{heavy}}^{*}$. Then $\wt T^{light} = \wt T - \wt T^{heavy}$ satisfies  $$\|\wt T^{light}\|_F \lsim \|\wt E\|_F + \delta \|T\|_F.$$
\end{lemma}
The proof of Lemma \ref{lem:smallnoisefirstcol} and Lemma \ref{lem:heavy_freq_recovery} are presented in Section \ref{subsection:heavy_light_decomp}.

\medskip

\noindent\textbf{Noisy Toeplitz Recovery.} Equipped with the previous heavy-light decomposition of Lemma \ref{lem:heavy_freq_recovery}, we can hope to use the set of recovered frequencies $L$ to find an approximation to $\wt T^{heavy}$ and thus to $\wt T$ with low error in the Frobenius norm using a sublinear time approximate regression primitive and prove Theorem \ref{thm:sublinear_time_recovery}. This needs to be done carefully and we now describe the key ideas behind the proof. A more formal version of Theorem \ref{frobeniusexistence} (see Section \ref{finalproof}) guarantees that the frequencies $S$ in the Vandermonde decomposition of $\wt T$ and thus in $\wt T^{heavy}$ have a certain grid structure. In particular, every $f\in S^{heavy}\subseteq  S$ is of the form $f=(2i-1)/2d + \gamma j$ for some integers $i\in [d]$ and $j\in [-\wt O(\log(1/\delta)),\wt O(\log(/\delta))]$. Here $\gamma$ is a fixed number per Theorem \ref{frobeniusexistence}. Also assuming $\|\wt E\|_F\leq c\|\wt T\|_F$, from Lemma \ref{lem:heavy_freq_recovery} we know that we have approximately recovered every $f\in S^{heavy}$, that is for every such $f$ there exists an $f'\in L $ such that $|f-f'|_{\circ}\leq \poly(k,\log(d/\delta))/d$. Thus we can set up intervals of size $ \poly(k,\log(d/\delta))/d$ around each $f'\in L$ and let $S(L)$ be the set of all $f$ in these intervals of the form $f=(2i-1)/2d + \gamma j$ for some integers $i\in [d]$ and $j\in [-\wt O(\log(1/\delta)),\wt O(\log(1/\delta))]$. Then we know that $S^{heavy}\subseteq S(L)$ and by definition of $S(L)$, $|S(L)|\leq \poly(k,\log(d/\delta))$. This implies that if study the following regression problem $\min_{D:D \text{ is diagonal }}\|T+E- F_{S(L)}DF_{S(L)}^*\|_F$, then it satisfies the following.
\begin{align*}
	\min_{D:D \text{ is diagonal }}\|T+E- F_{S(L)}DF_{S(L)}^*\|_F &\leq \|T+E-\wt T^{heavy}\|_F\\
 &\leq \|E\|_F+ \|T-\wt T\|_F + \|\wt T- \wt T^{heavy}\|_F\\
 &=\|E\|_F+ \|T-\wt T\|_F + \|\wt T^{light}\|_F\\
 &\lsim \|E\|_F + \|T-T_k\|_F +\delta \|T\|_F
\end{align*}
where the last line followed by upper bounding $\|\wt T^{light}\|_F$ from point 2. of Lemma \ref{lem:heavy_freq_recovery} and upper bounding $\|T-\wt T\|_F$ from point 1. of Theorem \ref{frobeniusexistence}. However we need to worry about the case when $\|\wt E\|_F\geq c \|\wt T\|_F$, that is when the noise is noticeably larger than the input and the output of Lemma \ref{lem:heavy_freq_recovery} does not approximate the frequencies of $S^{heavy}$. However in this case the above regression problem might as well output $D=0$ as the noise is very high, and one can still show $$\min_{D:D \text{ is diagonal }}\|T+E- F_{S(L')}DF_{S(L')}^*\|_F\lsim \|E\|_F + \|T-T_k\|_F +\delta \|T\|_F.$$
Finally using techniques based on leverage score sampling for Fourier sparse functions from \cite{kapralov2022toeplitz} and \cite{eldar2020toeplitz}, we can solve this regression problem upto constant factor accuracy in $\poly(k,\log(d/\delta))$ time. The output of this approximate regression problem will be a symmetric Toeplitz matrix (since it is of the form $F_{S(L)}DF_{S(L)}^*$ for diagonal $D$) and this then finishes the proof of Theorem \ref{thm:sublinear_time_recovery}. The details are presented in Section \ref{subsection:noisy_toeplitz_recovery}. Finally, equipped with the robust low-rank approximation result of Theorem \ref{thm:sublinear_time_recovery}, the proofs of Theorem \ref{thm:sublinear_time_lowrankapprox} and \ref{thm:sublinear_time_covariance_estimation} are presented in Section \ref{subsection:toeplitz_applications}.
\\
\begin{comment}
\subsection{\Cam{This should be removed.}}
\Cam{I would like to remove this section entirely. Let's discuss in person.}
\textbf{Low-rank approximation and Covariance estimation.}
Now we move on to giving the main ideas behind the sublinear time low rank approximation and covariance estimation results of Theorems \ref{thm:sublinear_time_lowrankapprox} and \ref{thm:sublinear_time_covariance_estimation} respectively. Firstly, equipped with Theorem \ref{thm:sublinear_time_recovery} Theorem \ref{thm:sublinear_time_lowrankapprox} follows easily by setting $E=0$. 

\Cam{This is out of place. This should be in the part where you prove Theorem 3.}
Now recall the setting of Theorem \ref{thm:sublinear_time_covariance_estimation}. In this setting we do not have direct access to the entries of $T$. Instead, we are given samples $x_1,x_2,\ldots, x_s \sim \mathcal{N}(0,T)$, where the covariance $T$ is a $d\times d$ PSD Toeplitz matrix. The goal here is to learn $T$ approximately from having access to $x_1,\ldots, x_s$, while minimizing the number of samples $s$ (this is referred to as the Vector Sample Complexity) \Cam{This should be defined in the intro, not here.} and the number of entries read from each sample $x_i$ (this is referred to as the Entry Sample Complexity).  Applying Theorem \ref{thm:sublinear_time_recovery} to this setting therefore will require more care.
The first claim of this section stated below essentially argues that $s=\poly(k)$ samples suffices to learn the top-$k$ eigenspace of the covariance $T$ approximately, thus being a more general robust version of the fact that $\poly(d)$ samples are necessary and sufficient to learn the full covariance $T$. This allows us to control how far the empirical covariance matrix is from the true covariance matrix in Frobenius norm, allowing us to then instantiate Theorem \ref{thm:sublinear_time_recovery}.

\kstodo{need to also highlight improvement over the existence proof of ELLM'20}
To prove this lemma, we use matrix concentration inequalities and tools from randomized numerical linear algebra such as Projection Cost Preserving (PCP) sketch property of the Gaussian distribution \cite{cohen2015dimensionality}. The complete proof is presented in Section 5. \Cam{I'm not sure why we need this. Don't we just need to bound the norm of $E = XX^T - T$ to apply Theorem 1? I don't get where this triangle inequality statement is being used?} An important point here is that this Lemma \ref{lem:low_rank_concentration} combined with the Toeplitz low-rank approximation existence result of Theorem \ref{frobeniusexistence} imply the following by triangle inequality,
\begin{equation}\label{eqn:low_rank_empirical_existence}
    \|XX^T - F_{ S} D F_{ S}\|_F \lsim \sqrt{\|T-T_k\|_2 \tr(T)+ \frac{\|T-T_k\|_F \tr(T)}{k}}+ \epsilon \|T\|_2
\end{equation}
where $X$ is as per the statement of Lemma \ref{lem:low_rank_concentration} and $F_{ S} D F_{ S}=\wt T$ is as per the statement of Theorem \ref{frobeniusexistence} applied to $T$ and $\epsilon=O(1)$. This significantly strengthens the analogous result of Lemma 5.6 of \cite{eldar2020toeplitz} who were only able to show $XX^T$ is well approximated by a matrix spanned by some Fourier frequencies, but equation \eqref{eqn:low_rank_empirical_existence} by shows that $XX^T$ is infact well approximated by a very structured object - a low rank Toeplitz matrix.

Equipped with the previous lemma, we can instantiate Theorem \ref{thm:sublinear_time_recovery} with $E=XX^T-T$ to prove our sublinear time covariance estimation result of Theorem \ref{thm:sublinear_time_covariance_estimation}. Note that the error guarantees of Theorem \ref{thm:sublinear_time_covariance_estimation} match the guarantees of the algorithm of \cite{eldar2020toeplitz} for this problem as per Theorem 2.10 in \cite{eldar2020toeplitz}, but our algorithm runs in sublinear time thus resolving their main open problem.
\Cam{As in the othe theorems, remove $r$ as it is not needed.}
The details of the proofs of Lemma \ref{lem:low_rank_concentration} and Theorem \ref{thm:sublinear_time_covariance_estimation} are presented in Section \ref{subsection:toeplitz_applications}.
\end{comment}

\subsection{Other related work}\label{sec:prior} 
\kstodo{Mostly taken from previous soda paper!}
A large body of work in numerical linear algebra, applied mathematics, theoretical computer science, and signal processing  has studied the problem of computing low-rank approximations of Toeplitz and Hankel matrices \cite{Luk:1996ur,Park:1999ta,Ishteva:2014wm,Cai:2016wh,Ongie:2017us,Krim:1996wm,Shi:2019ud}. In many applied signal processing settings, Toeplitz matrices arise as PSD covariance matrices, motivating our focus on the PSD case.
%Using the FFT, any $d \times d$ Toeplitz matrix can be multiplied by a vector in  $O(d \log d)$ time. \cite{Shi:2019ud} show how to use this  primitive to give a near-linear time, near-optimal low-rank approximation algorithm for Toeplitz matrices. In particular, their algorithm outputs $\wt T$ with rank $k$ satisfying $\norm{T-\wt T}_F \le (1+\epsilon) \norm{T-\tilde T}_F$ in $\tilde O(d + \poly(k/\epsilon))$ time. Note that $\wt T$ here may not be Toeplitz.
Significant prior work has also studied the problem of computing an optimal \emph{structure-preserving} Toeplitz low-rank approximation, where the low-rank approximation $\wt T$ is itself required to be Toeplitz. However, no simple characterization of the optimal solution to this problem is known \cite{chu2003structured} and polynomial time algorithms  are only known in the special cases of $k= 1$ and $k = d-1$ \cite{chu2003structured,Knirsch:2021ve}. On the practical side a range of heuristics are known, based on techniques such as convex relaxation \cite{Fazel:2013vw,Cai:2016wh,Ongie:2017us}, alternating minimization \cite{chu2003structured,Wen:2020ub}, and sparse Fourier transform \cite{Krim:1996wm}. 

%\cite{Park:1999ta,Ishteva:2014wm}. %Many works focus on computationally efficient, but not sublinear algorithms that output a good Toeplitz low-rank approximation to the input. 
%\cite{Wen:2020ub} matrix comlpetion alternatiing svd typo algorithm.

Many results in the signal processing literature study sublinear query algorithms for Toeplitz matrices, these are referred to as \emph{sparse array methods} which proceed by querying a small principal submatrix to obtain an approximation to the whole matrix \cite{Abramovich:1999vs,Chen:2015wz,Qiao:2017tp,Lawrence:2020ut}. The work of \cite{eldar2020toeplitz} and \cite{kapralov2022toeplitz} on sublinear query PSD Toeplitz low-rank approximation and Toeplitz covariance estimation is closely related to this literature. %give sublinear query algorithms for various problems on Toeplitz matrices as discussed in the introduction.
%
%
%Several of these works focus on algorithms with sublinear query complexity \cite{Lawrence:2020ut} \cite{Qiao:2017tp}
%
%%\cite{Ongie:2017us} convex relaxation
%
%%\cite{Park:1999ta} -- not really sure the method
%
%%\cite{Knirsch:2021ve} -- optimal rank-1 paper.
%
%
%%Structured low rank approximation \cite{chu2003structured}.
%%\begin{itemize}
%%%\item \url{https://www.cas.mcmaster.ca/~qiao/publications/LQV02.pdf}
%%%\item \url{http://www.cas.mcmaster.ca/~qiao/publications/LQ96b.pdf}
%%%\item \url{https://journalofinequalitiesandapplications.springeropen.com/track/pdf/10.1186/s13660-020-02340-w.pdf}
%%%\item \url{https://ieeexplore.ieee.org/document/8715594}
%%%\item \url{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC5999344/}
%%%\item \url{https://conservancy.umn.edu/handle/11299/215327}
%%%\item \url{https://www.math.colostate.edu/~king/codex/slides/Plonka_2020_11_03.pdf} lots of good refs. Optimal rank-1 solution. Also optimal solution in infinite operator case.
%%\item \url{https://mtchu.math.ncsu.edu/Research/Lectures/Iep/chapter8.pdf} states that optimal Toeplitz low-rank approximation is open.
%%\end{itemize}
%

Beyond Toeplitz matrices, significant recent work has focused on  sublinear time low-rank approximation algorithms for other structured matrix classes. This includes positive semidefinite matrices \cite{musco2017recursive,Bakshi:2020tl}, distance matrices \cite{Bakshi:2018ul,Indyk:2019vy}, and kernel matrices \cite{musco2017recursive,Yasuda:2019vf,Ahle:2020vj}.

%Our techniques also rely on sublinear time algorithms for sparse Fourier recovery problems. There is a large body of work on sparse discrete fourier transforms, that are concerned with computing $k$-Fourier sparse approximations to discrete time signals of period $d$ in $\wt O(k)$ time \cite{hassanieh2012nearly,indyk2014sample,indyk2014nearly,kapralov2016sparse,chen2016fourier}. Most relevant to our work is the work of \cite{chen2016fourier}, which obtained $\poly(k,\log d)$-Fourier sparse approximations on a bounded interval $[0,d]$ to $k$-Fourier sparse functions with arbitrary frequencies, thus not necessarily periodic, in $\poly(k,\log d)$ time given access to the input on the entire interval $[0,d]$.













